Parameter-Efficient Multi-Task Fine-Tuning in Code-Related Tasks

Large Language Models (LLMs) have proven highly effective in automating software engineering tasks, bridging natural language and code semantics to achieve notable results in code generation and summarization. However, their scale incurs substantial computational costs, making full fine-tuning impractical. Parameter-Efficient Fine-Tuning (PEFT) methods like QLoRA enable efficient specialization with lower resource demands. Recent studies show QLoRA-optimized Large Code Models (LCMs) perform strongly across diverse tasks, yet it remains unclear whether this effectiveness persists when a single model is QLoRA fine-tuned for multiple code-related tasks. The interaction between Multi-task fine-tuning and QLoRA optimization, and how transfer learning affects correctness and quality of generated artifacts, remains largely unexplored. We investigate Multi-task QLoRA fine-tuning --- a representative parameter-efficient method from the LoRA family --- across three representative tasks: code generation, translation, and summarization. We evaluate functional correctness through execution-based and similarity-based metrics, complemented by comprehensive code quality analysis--an aspect largely overlooked in prior work. Our findings show that Multi-task QLoRA effectively leverages transfer learning, achieving competitive or superior performance at the 1.5B, 3B, and 7B configurations relative to both Single-task QLoRA and Multi-task full fine-tuning. Larger models demonstrate more consistent balance between correctness and quality, whereas smaller models preserve functionality but exhibit a higher incidence of quality-related issues.

==> sections/qualitative-old.tex <==
% !TEX root = ../main.tex
\subsection{Qualitative Analysis: Model Capacity Effects Across Code-Related Tasks}
\label{sec:qualitative_analysis}

To illustrate the practical implications of our quantitative findings, we present qualitative examples demonstrating how model capacity influences output quality across all three code-related tasks. These examples reveal consistent patterns: larger models systematically produce outputs with better structure, reduced errors, and more sophisticated understanding of task requirements, even when functional correctness varies across configurations.

\subsubsection{Code Generation}

\figref{fig:qualitative_example_cg} displays three implementations of the \texttt{verifyClass} function from the \texttt{zope.interface} library, generated by 0.5B, 1.5B, and 3B models, respectively. This example demonstrates how model capacity influences both code structure and quality characteristics measurable through static analysis, even when functional correctness remains unachieved across all configurations.

\begin{figure*}[t]
\centering
\includegraphics[width=0.95\textwidth]{images/qualitative-example-CG.pdf}
\caption{Comparison of code generated by \MT QLoRA across three model scales (0.5B, 1.5B, 3B) for the same programming task. The task requires implementing the \texttt{verifyClass} function that validates whether a candidate class correctly provides a specified interface. Code quality--measured by Pylint and SonarCloud violations--improves systematically with model capacity: 0.5B generates verbose, repetitive code with 29 Pylint violations; 1.5B produces more structured code with proper control flow and 25 violations; 3B generates concise, logically sound code with only 23 violations. Ellipsis (\texttt{...}) indicates abbreviated content for space constraints.}
\label{fig:qualitative_example_cg}
\end{figure*}

The qualitative issues panel summarizes static analysis violations. The 0.5B model generates 29 Pylint violations (0 Errors, 20 Warnings, 9 Convention, 0 Refactor) and 2 SonarCloud issues (0 Security, 0 Reliability, 2 Maintainability). The 1.5B model reduces total violations to 25 (2 Errors, 18 Warnings, 4 Convention, 1 Refactor) with 2 SonarCloud issues. The 3B model further reduces violations to 23 (4 Errors, 15 Warnings, 4 Convention, 0 Refactor) with only 1 SonarCloud issue.

Examining the implementations reveals distinct quality patterns. The 0.5B model produces verbose, repetitive code with fundamental logical errors. Lines 5--8 perform basic validation checking for \texttt{None} values, but line 11 misuses \texttt{isinstance(candidate, iface)}--this function tests object instances against types, not class-interface compliance as required. Lines 15--29 demonstrate severe code redundancy: the implementation repeats nearly identical validation blocks four times, checking \texttt{iface.methods()} and \texttt{iface.interfaces()} with duplicate \texttt{hasattr} calls and error messages. This violates the DRY (Don't Repeat Yourself) principle and suggests the model fails to abstract common patterns. Additionally, the function never returns a success value, implicitly returning \texttt{None} instead of \texttt{True}. The 20 warnings (primarily indentation issues W0311) and 9 convention violations (including formatting C0304 and string formatting C0209) indicate struggles with basic code structure.

The 1.5B model demonstrates substantial improvement in logical organization. It correctly implements interface and class validation through \texttt{isInterface(iface)} and \texttt{isClass(candidate)} checks (lines 6--7), returning \texttt{False} for invalid inputs. Lines 9--14 properly iterate over \texttt{iface.\_\_bases\_\_} to verify inheritance relationships, using appropriate control flow with \texttt{break}, \texttt{continue}, and \texttt{return False}. The tentative parameter handling (lines 16--17) correctly shortcuts validation when appropriate. Lines 19--22 include exception handling with \texttt{try-except TypeError}, attempting to instantiate the candidate class to verify it is callable. The final \texttt{return True} (line 24) properly indicates success. While the implementation eliminates redundancy and reduces warnings to 18 and convention violations to 4, it introduces 2 undefined variable errors (E0602) in the \texttt{isInterface} and \texttt{isClass} calls, indicating missing imports. The 1 refactor suggestion (R1723) likely addresses the \texttt{if-return} pattern that could be simplified.

The 3B model produces concise, well-structured code demonstrating sophisticated understanding of the verification logic. Lines 5--7 implement proper interface validation using \texttt{isInterface(iface)} with a descriptive \texttt{TypeError} message. Lines 8--9 validate the candidate is a class rather than an instance. Lines 11--12 efficiently check interface caching using \texttt{\_classCache}, returning the cached result immediately if available. Lines 14--15 verify the candidate has the required \texttt{\_\_implements\_\_} attribute, returning \texttt{False} if absent--this correctly identifies that classes declare interface implementation through this attribute. Lines 17--18 handle the tentative parameter, while lines 20--22 iterate through \texttt{candidate.\_\_implements\_\_} using \texttt{issubclass} to verify interface inheritance relationships. The final \texttt{return False} (line 24) handles cases where verification fails. This implementation demonstrates understanding of interface implementation patterns, caching mechanisms, and efficient validation logic. The 23 total violations represent the lowest count, with only 1 SonarCloud maintainability issue versus 2 for smaller models. The 4 errors (E0602) again stem from missing imports for helper functions rather than logical flaws, while the 15 warnings and 4 convention violations indicate superior code structure compared to smaller models.

\subsubsection{Code Translation}

\figref{fig:qualitative_example_ct} presents C\#-to-Java translations of the \texttt{getLong()} method across three model scales. Unlike code generation, translation operates within tighter constraints: the source code provides explicit guidance for structure and logic, yet models must adapt language-specific idioms while maintaining semantic equivalence.

\begin{figure*}[t]
\centering
\includegraphics[width=0.95\textwidth]{images/qualitative-example-CT.pdf}
\caption{Comparison of C\#$\rightarrow$Java translations by \MT QLoRA across three model scales. All models produce functionally equivalent implementations that preserve the source logic. However, quality differences emerge in language-specific details: 0.5B introduces non-standard constant references (\texttt{LIBCORE\_IO\_SIZEOF.LONG}); 1.5B adds unnecessary \texttt{final} modifiers; 3B produces the most idiomatic Java translation matching standard conventions. Quality metrics show consistent patterns: 0.5B and 3B each generate 6 PMD violations and 1 SonarCloud issue, while 1.5B achieves slight improvement with 5 PMD violations.}
\label{fig:qualitative_example_ct}
\end{figure*}

All three models successfully translate the core logic, producing syntactically valid Java implementations with identical control flow. However, subtle quality differences emerge in language-specific conventions and style adherence. The 0.5B model introduces \texttt{LIBCORE\_IO\_SIZEOF.LONG} (line 2), a non-standard constant reference that deviates from typical Java conventions--the reference implementation uses \texttt{SizeOf.LONG}. This generates 6 PMD violations (0 Best Practices, 5 Code Style, 1 Design, 0 Error Prone, 0 Multi-threading, 0 Performance) and 1 SonarCloud maintainability issue, primarily reflecting naming and formatting inconsistencies.

The 1.5B model produces a more conventional translation using \texttt{SizeOf.LONG} and adding the \texttt{final} modifier to both the method declaration and the \texttt{newPosition} variable (lines 1--2). While \texttt{final} enhances immutability guarantees, its application here may be considered overly defensive for local variables in straightforward accessor methods. This configuration achieves 5 PMD violations (0 Best Practices, 4 Code Style, 1 Design, 0 Error Prone, 0 Multi-threading, 0 Performance) and 1 SonarCloud issue, representing marginal improvement over the 0.5B model.

The 3B model generates the most idiomatic translation, using \texttt{SizeOf.LONG} without extraneous modifiers. The resulting code (lines 1--17) mirrors the reference implementation's structure and style conventions. Quality metrics show 6 PMD violations (matching 0.5B) and 1 SonarCloud issue, indicating that even the largest model produces outputs with detectable style violations--though these violations reflect standard Java formatting preferences rather than logical defects.

This example illustrates that translation quality improvements with increased capacity are more subtle than in code generation. All models successfully preserve semantic equivalence, but larger models demonstrate better understanding of target language idioms and conventions. The 3B model's output most closely approximates human-written Java code in terms of naming conventions and modifier usage, even though static analysis metrics show comparable violation counts across scales.

\subsubsection{Code Summarization}

\figref{fig:qualitative_example_cs} presents summaries generated for the \texttt{getLong()} method across three model scales, evaluated using LLM-as-a-judge methodology. This example demonstrates how model capacity affects semantic accuracy and linguistic quality in natural language generation.

\begin{figure*}[t]
\centering
\includegraphics[width=0.95\textwidth]{images/qualitative-example-CS.pdf}
\caption{Comparison of code summaries generated by \MT QLoRA across three model scales for the \texttt{getLong()} method. The 0.5B model produces an incorrect summary describing boolean array conversion (Content Adequacy: 1.0), while 1.5B and 3B generate semantically accurate summaries with progressive quality improvements. LLM-as-judge scores show consistent improvement: 0.5B achieves mean quality of 2.67, 1.5B reaches 3.93, and 3B attains 4.13 across Content Adequacy (CA), Conciseness (Conc), and Fluency (Fl) dimensions.}
\label{fig:qualitative_example_cs}
\end{figure*}

The quality progression across model scales is stark. The 0.5B model generates: \textit{``Converts a primitive array of booleans into a wrapper array.''} This summary is factually incorrect--the method extracts a long integer from a byte buffer, not converting boolean arrays. The LLM-as-judge evaluation reflects this fundamental error: Content Adequacy scores 1.0 (indicating minimal alignment with actual functionality), Conciseness scores 4.8 (the summary is appropriately brief), and Fluency scores 2.2 (grammatically correct but semantically misleading), yielding a mean quality of 2.67.

The 1.5B model produces: \textit{``Convert a Boolean array to primitive boolean array.''} While this remains semantically incorrect (still referencing boolean arrays rather than long integers), the phrasing demonstrates improved grammatical structure. Quality scores improve accordingly: Content Adequacy reaches 2.0, Conciseness achieves 5.0 (maximal), and Fluency improves to 4.8, producing a mean quality of 3.93. The substantial fluency improvement suggests the model has developed better natural language generation capabilities, though the semantic understanding of the code remains flawed.

The 3B model generates: \textit{``Converts a Boolean array into a primitive boolean array.''} Remarkably, this summary remains semantically incorrect despite improved linguistic quality, achieving Content Adequacy of 2.4, Conciseness of 5.0, and Fluency of 5.0 (maximal), yielding a mean quality of 4.13. The perfect fluency score indicates the model produces well-formed, grammatically correct English, yet the persistent semantic error reveals that even the largest model fails to accurately capture the method's true functionality in this instance.

This example highlights a critical insight: increased model capacity consistently improves linguistic quality (fluency, grammatical correctness, and naturalness of expression) but does not guarantee semantic accuracy. While our aggregate results in RQ$_1$ show that 3B models achieve substantially higher BLEU and BERTScore across the full evaluation set, individual cases demonstrate that capacity-driven improvements in surface-level quality do not eliminate all semantic errors. This underscores the importance of comprehensive evaluation across large test sets rather than relying on individual examples to characterize model behavior.

%\subsubsection{Synthesis Across Tasks}

These qualitative examples reinforce our quantitative findings: model capacity systematically improves output quality across all tasks, though improvement patterns vary by task. Code generation benefits from better logical structure and reduced redundancy. Code translation shows improved adherence to target language idioms while maintaining functional correctness. Code summarization achieves higher fluency and grammatical correctness, though semantic accuracy remains variable at the instance level.

The 3B model consistently demonstrates superior understanding of domain-specific patterns--interface implementation conventions, language-specific naming standards, and natural language generation principles--even under parameter-efficient constraints. These capacity-driven quality improvements underpin the aggregate performance advantages observed in RQ$_1$ and RQ$_2$, establishing that larger models better leverage \MT QLoRA's constrained parameter space to balance multiple objectives.




% \subsection{Qualitative Analysis: Model Capacity Effects on Code Quality}
% \label{sec:qualitative_analysis}

% To illustrate the practical implications of our quantitative findings, we present a qualitative example of code generated by \MT QLoRA configurations across different model scales for the same programming task. \figref{fig:qualitative_example_cg} displays three implementations of the \texttt{verifyClass} function from the \texttt{zope.interface} library, generated by 0.5B, 1.5B, and 3B models respectively. This example demonstrates how model capacity influences both code structure and quality characteristics measurable through static analysis, even when functional correctness remains unachieved across all configurations.

% \begin{figure*}[t]
% \centering
% \includegraphics[width=0.95\textwidth]{images/qualitative-example.pdf}
% \caption{Comparison of code generated by \MT QLoRA across three model scales (0.5B, 1.5B, 3B) for the same programming task. The task requires implementing the \texttt{verifyClass} function that validates whether a candidate class correctly provides a specified interface. Code quality--measured by Pylint and SonarCloud violations--improves systematically with model capacity: 0.5B generates verbose, repetitive code with 29 Pylint violations; 1.5B produces more structured code with proper control flow and 25 violations; 3B generates concise, logically sound code with only 23 violations. Ellipsis (\texttt{...}) indicates abbreviated content for space constraints.}
% \label{fig:qualitative_example_cg}
% \end{figure*}

% The qualitative issues panel in \figref{fig:qualitative_example} summarizes static analysis violations. The 0.5B model generates 29 Pylint violations (0 Errors, 20 Warnings, 9 Convention, 0 Refactor) and 2 SonarCloud issues (0 Security, 0 Reliability, 2 Maintainability). The 1.5B model reduces total violations to 25 (2 Errors, 18 Warnings, 4 Convention, 1 Refactor) with 2 SonarCloud issues. The 3B model further reduces violations to 23 (4 Errors, 15 Warnings, 4 Convention, 0 Refactor) with only 1 SonarCloud issue.

% Examining the implementations reveals distinct quality patterns. The 0.5B model produces verbose, repetitive code with fundamental logical errors. Lines 5--8 perform basic validation checking for \texttt{None} values, but line 11 misuses \texttt{isinstance(candidate, iface)}--this function tests object instances against types, not class-interface compliance as required. Lines 15--29 demonstrate severe code redundancy: the implementation repeats nearly identical validation blocks four times, checking \texttt{iface.methods()} and \texttt{iface.interfaces()} with duplicate \texttt{hasattr} calls and error messages. This violates the DRY (Don't Repeat Yourself) principle and suggests the model fails to abstract common patterns. Additionally, the function never returns a success value, implicitly returning \texttt{None} instead of \texttt{True}. The 20 warnings (primarily indentation issues W0311) and 9 convention violations (including formatting C0304 and string formatting C0209) indicate struggles with basic code structure.

% The 1.5B model demonstrates substantial improvement in logical organization. It correctly implements interface and class validation through \texttt{isInterface(iface)} and \texttt{isClass(candidate)} checks (lines 6--7), returning \texttt{False} for invalid inputs. Lines 9--14 properly iterate over \texttt{iface.\_\_bases\_\_} to verify inheritance relationships, using appropriate control flow with \texttt{break}, \texttt{continue}, and \texttt{return False}. The tentative parameter handling (lines 16--17) correctly shortcuts validation when appropriate. Lines 19--22 include exception handling with \texttt{try-except TypeError}, attempting to instantiate the candidate class to verify it is callable. The final \texttt{return True} (line 24) properly indicates success. While the implementation eliminates redundancy and reduces warnings to 18 and convention violations to 4, it introduces 2 undefined variable errors (E0602) in the \texttt{isInterface} and \texttt{isClass} calls, indicating missing imports. The 1 refactor suggestion (R1723) likely addresses the \texttt{if-return} pattern that could be simplified.

% The 3B model produces concise, well-structured code demonstrating sophisticated understanding of the verification logic. Lines 5--7 implement proper interface validation using \texttt{isInterface(iface)} with a descriptive \texttt{TypeError} message. Lines 8--9 validate the candidate is a class rather than an instance. Lines 11--12 efficiently check interface caching using \texttt{\_classCache}, returning the cached result immediately if available. Lines 14--15 verify the candidate has the required \texttt{\_\_implements\_\_} attribute, returning \texttt{False} if absent--this correctly identifies that classes declare interface implementation through this attribute. Lines 17--18 handle the tentative parameter, while lines 20--22 iterate through \texttt{candidate.\_\_implements\_\_} using \texttt{issubclass} to verify interface inheritance relationships. The final \texttt{return False} (line 24) handles cases where verification fails. This implementation demonstrates understanding of interface implementation patterns, caching mechanisms, and efficient validation logic. The 23 total violations represent the lowest count, with only 1 SonarCloud maintainability issue versus 2 for smaller models. The 4 errors (E0602) again stem from missing imports for helper functions rather than logical flaws, while the 15 warnings and 4 convention violations indicate superior code structure compared to smaller models.

% This qualitative analysis reinforces our quantitative findings from RQ$_1$ and RQ$_2$: while increased model capacity does not guarantee functional correctness, it systematically produces code with better logical structure, reduced redundancy, and more sophisticated implementation patterns. The 3B model's understanding of caching mechanisms and interface implementation conventions demonstrates that larger models develop stronger comprehension of library-specific patterns and software engineering principles, even under parameter-efficient fine-tuning constraints. These quality improvements contribute to the aggregate advantages observed across our large-scale evaluation.

==> sections/results-ext.tex <==
% !TEX root = ../main.tex
%%%%%%%%%%% EXTENDED STUDY %%%%%%%%%%%


\subsection{Exploring the Capacity-Training Trade-off}
\label{sec:capacity_training}

Across RQ$_1$--RQ$_3$, we observed that the performance advantages of \MT QLoRA become increasingly pronounced as model scale increases. To determine whether these gains are primarily driven by base model capacity or by the number of trainable adapter parameters, we conduct capacity-matched experiments in which smaller backbone models are equipped with adapter configurations that match the trainable parameter counts of larger models. This design enables us to disentangle the effects of architectural capacity from those of parameter-efficient adaptation in \MT learning.

\tabref{tab:param_configs} summarizes the experimental configurations. Specifically, we train (i) Qwen-0.5B models with 9.3M trainable parameters (\MTqlora$_{9.3M}$, matching the standard 1.5B configuration) and 14.8M parameters (\MTqlora$_{15M}$, matching the standard 3B configuration), (ii) a Qwen-1.5B model with 15.0M trainable parameters (matching the standard 3B configuration), and (iii) a Qwen-3B model with 9.4M trainable parameters (matching the standard 1.5B configuration). These settings allow direct comparison between models with equivalent numbers of trainable parameters but different backbone capacities. All capacity-matched variants are evaluated on code generation, code translation, and code summarization, using the same functional correctness and quality metrics as in prior sections.

\begin{table}[h]
\centering
\caption{Parameter configurations for capacity-training experiments.}
\label{tab:param_configs}
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{llcccc}
\toprule
\textbf{Model} & \textbf{Configuration} & \textbf{r} & \textbf{$\alpha$} & \textbf{Trainable} & \textbf{\%} \\
\midrule
\multicolumn{6}{l}{\textit{Default configurations}} \\
Qwen-0.5B & Standard & 8 & 16 & 4.4M & 0.88\% \\
Qwen-1.5B & Standard & 8 & 16 & 9.3M & 0.59\% \\
Qwen-3B & Standard & 8 & 16 & 15.0M & 0.48\% \\
\midrule
\multicolumn{6}{l}{\textit{Capacity-matched experiments}} \\
Qwen-0.5B & \MTqlora$_{9.3M}$ ($\rightarrow$1.5B match) & 17 & 32 & 9.3M & 1.86\% \\
Qwen-0.5B & \MTqlora$_{15M}$ ($\rightarrow$3B match) & 27 & 54 & 14.8M & 2.92\% \\
Qwen-1.5B & \MTqlora$_{15M}$ ($\rightarrow$3B match) & 13 & 26 & 15.0M & 0.96\% \\
Qwen-3B & \MTqlora$_{9.3M}$ ($\rightarrow$1.5B match) & 5 & 10 & 9.4M & 0.30\% \\
\bottomrule
\end{tabular}
}
\end{table}

\subsubsection{Code Generation}

Results from the capacity-matched experiments indicate that increasing the number of trainable parameters alone is insufficient to replicate the performance of larger backbone models. For Python (\tabref{tab:ext_codegen_python}), \MTqlora$_{9.3M}$ on Qwen-0.5B achieves 16.84\% \passatone compared to standard \MTqlora on Qwen-1.5B at 18.95\% ($-2.11$ points), while \MTqlora$_{15M}$ on Qwen-0.5B reaches only 14.74\% relative to the standard Qwen-3B configuration at 21.05\% ($-6.31$ points). A similar pattern holds for \java (\tabref{tab:ext_codegen_java}), where \MTqlora$_{15M}$ on Qwen-0.5B achieves 20.65\% versus 32.07\% for standard Qwen-3B ($-11.42$ points), and \MTqlora$_{15M}$ on Qwen-1.5B reaches 27.17\% ($-4.90$ points). 

In contrast, reducing the number of trainable parameters on a larger backbone does not substantially degrade performance. \MTqlora$_{9.3M}$ on Qwen-3B achieves 20.53\% \passatone for Python and 34.78\% for \java, exceeding the corresponding standard Qwen-1.5B configurations despite using fewer trainable parameters. These results underscore that backbone capacity, rather than adapter size, is the primary driver of code generation performance.

\input{tables/ext-cg-py}
\input{tables/ext-cg-java}

Quality metrics further reinforce the dominance of base model capacity. For Python, \MTqlora$_{9.3M}$ on Qwen-0.5B produces 913 Cyclomatic Complexity issues compared to 882 for standard Qwen-1.5B (+3.5\%), while \MTqlora$_{15M}$ on Qwen-0.5B generates 975 issues versus 677 for standard Qwen-3B (+44.0\%). SonarCloud maintainability issues show a similar pattern, increasing from 72 under standard Qwen-1.5B to 89 under \MTqlora$_{9.3M}$ on Qwen-0.5B (+23.6\%). For \java, \MTqlora$_{9.3M}$ on Qwen-0.5B produces 710 Cyclomatic Complexity issues versus 589 for standard Qwen-1.5B (+20.5\%), while \MTqlora$_{15M}$ on Qwen-0.5B yields 613 issues relative to 558 for standard Qwen-3B (+9.9\%).

Code size analysis yields consistent conclusions. \MTqlora$_{15M}$ on Qwen-0.5B generates substantially longer Python code (2,467 LoC vs.\ 1,759 for standard Qwen-3B, +40.3\%) with higher token counts (15,486 vs.\ 11,773, +31.5\%). Conversely, \MTqlora$_{9.3M}$ on Qwen-3B produces compact implementations (1,845 LoC for Python and 1,573 LoC for \java), comparable to standard configurations, indicating that larger backbone models enable concise solutions even under constrained adaptation.

\subsubsection{Code Translation}

For code translation, the capacity--training trade-off reveals sharper thresholds for maintaining output validity. In the Java$\rightarrow$C\# direction (\tabref{tab:ext_codetrans_java2csharp}), \MTqlora$_{15M}$ on Qwen-0.5B achieves 71.79\% CodeBLEU, exceeding the standard Qwen-3B configuration at 62.88\%. In contrast, \MTqlora$_{9.3M}$ on Qwen-0.5B drops to 60.98\% relative to 73.08\% for standard Qwen-1.5B ($-12.10$ points). 

The C\#$\rightarrow$Java direction (\tabref{tab:ext_codetrans_csharp2java}) is substantially more sensitive to parameter constraints. \MTqlora$_{9.3M}$ on Qwen-0.5B achieves only 51.14\% CodeBLEU compared to 70.72\% for standard Qwen-1.5B ($-19.58$ points), while \MTqlora$_{15M}$ on Qwen-0.5B reaches 59.45\%, trailing standard Qwen-3B by 11.77 points. Most critically, \MTqlora$_{9.3M}$ on Qwen-3B exhibits catastrophic degradation at 47.43\% CodeBLEU with a detection rate of 78.6\%, indicating that insufficient trainable parameters can compromise translation validity even when backbone capacity is high.

\input{tables/ext-ct-java-csharp}
\input{tables/ext-ct-sharp-java}

Quality diagnostics corroborate these findings. For Java$\rightarrow$C\#, Roslyn analysis shows that \MTqlora$_{9.3M}$ on Qwen-0.5B generates few syntax errors (11) but accumulates 1,476 maintainability issues, representing a 149\% increase over standard Qwen-1.5B (592). For C\#$\rightarrow$Java, \MTqlora$_{9.3M}$ on Qwen-3B yields anomalous outputs with most PMD categories unreported (N/A), reflecting fundamental translation failures. Even when translations remain valid, quality degrades sharply: \MTqlora$_{15M}$ on Qwen-0.5B produces 3,324 PMD issues versus 1,171 under standard Qwen-3B, including pronounced increases in Code Style (2,858 vs.\ 1,072, +166.6\%) and Design violations (181 vs.\ 45, +302.2\%).

Taken together, these results indicate that code translation requires a balanced combination of backbone capacity and sufficient trainable parameters. An approximate threshold of 15M trainable parameters emerges as critical, below which even large backbone models fail to consistently produce valid translations. This sensitivity reflects the bidirectional and structurally constrained nature of code-to-code transformation.

\subsubsection{Code Summarization}

For code summarization, capacity effects dominate for Python, whereas \java remains largely invariant to both backbone size and adapter configuration. For Python (\tabref{tab:ext_codesum}), \MTqlora$_{9.3M}$ on Qwen-0.5B achieves 7.55\% BLEU compared to 12.60\% for standard Qwen-1.5B ($-40.1$\% relative), while \MTqlora$_{15M}$ on Qwen-0.5B reaches 7.78\% relative to 24.33\% for standard Qwen-3B ($-68.0$\% relative). In contrast, \MTqlora$_{9.3M}$ on Qwen-3B attains 25.13\% BLEU, surpassing the standard 3B configuration (24.33\%) while using 37\% fewer trainable parameters. Similarly, \MTqlora$_{15M}$ on Qwen-1.5B achieves 13.99\%, exceeding its standard counterpart at 12.60\% (+11.0\%).

\input{tables/ext-cs}

For \java, summarization performance remains clustered around 1.1--1.5\% BLEU across all configurations. \MTqlora$_{9.3M}$ on Qwen-0.5B achieves 1.18\% compared to 1.28\% for standard Qwen-1.5B, while \MTqlora$_{15M}$ on Qwen-1.5B reaches 1.50\%, and \MTqlora$_{9.3M}$ on Qwen-3B maintains 1.33\%. These marginal variations indicate that neither backbone capacity nor adapter size substantially influences \java summarization.

LLM-as-a-judge evaluation (Appendix~\ref{appendix:llm_judge}) provides additional insight beyond similarity metrics. For Python, Content Adequacy decreases only slightly for \MTqlora$_{9.3M}$ on Qwen-0.5B (1.802 vs.\ 1.862 for standard Qwen-1.5B, $-3.2$\%) despite a 40.1\% BLEU gap, suggesting that smaller models retain core semantic content while struggling with reference-aligned phrasing. For \java, quality metrics remain stable across configurations: Content Adequacy ranges from 2.154 to 2.339 (73--79\% of the human baseline), Conciseness approaches ceiling values (4.925--4.990), and Fluency consistently exceeds the human baseline (4.226--4.408 vs.\ 4.079).

Overall, these results demonstrate that Python summarization benefits primarily from increased backbone capacity, while \java summarization remains largely invariant to both capacity and trainable parameter count. This contrast suggests that improvements to Java summarization may require alternative modeling or representation strategies beyond scaling or adapter reconfiguration.

\begin{tcolorbox}[
    colback=gray!10, 
    colframe=black, 
    arc=5mm, 
    colupper=black, 
    boxrule=1pt,
    title={\textbf{Summary of Extended Study: Exploring the Capacity-Training Trade-off}}, 
    coltitle=white,
    colbacktitle=black,
    toptitle=1mm,
    bottomtitle=1mm,
    left=6pt, 
    right=6pt, 
    top=6pt, 
    bottom=6pt
]
\justifying
We investigate whether \MT QLoRA performance stems from base model capacity or trainable adapter parameters through capacity-matched experiments adjusting LoRA rank and alpha to match parameter counts across backbone sizes.

For \textit{code generation}, base model capacity dominates. Smaller backbones with increased adapters fail to match larger models with standard configurations despite identical trainable parameters, while larger backbones with reduced adapters exceed smaller models despite fewer parameters. Quality metrics reinforce this: smaller backbones produce higher complexity and maintainability issues regardless of adapter size.
For \textit{code translation}, a critical 15M trainable parameter threshold emerges. Below this threshold, even large backbones exhibit catastrophic failures with detection rates below 21\%, indicating translation requires minimum adapter capacity regardless of backbone size.
For \textit{code summarization}, Python performance depends on backbone capacity (smaller backbones underperform despite increased adapters), while \java remains invariant across all configurations. LLM-as-judge evaluation shows smaller backbones retain semantic content despite reference similarity gaps.

Code size patterns reveal larger backbones with constrained adapters produce more compact implementations, while capacity-matched smaller models generate longer code with more quality violations.
Base model capacity, not adapter parameter count, primarily drives \MT QLoRA performance. Smaller backbones cannot replicate larger models even with matching adapters, while larger backbones maintain effectiveness with reduced adapters. Exception: translation requires minimum 15M trainable parameters regardless of backbone. Practitioners should prioritize larger backbones with minimal adapters over compensating small models with extensive adapters.
\end{tcolorbox}



\begin{comment}
\subsection{Exploring the Capacity-Training Trade-off}

Across RQ1-RQ3, we observed that \MT QLoRA's performance improvements become increasingly pronounced as model size increases. To investigate whether this advantage stems from model capacity or trainable parameter configuration, we conduct capacity-matched experiments where smaller models are trained with adapter configurations that match the trainable parameter counts of larger models.

Table~\ref{tab:param_configs} presents the experimental configurations. We train Qwen-0.5B with 9.3M trainable parameters (matching 1.5B's standard configuration) and 14.8M parameters (matching 3B), train Qwen-1.5B with 15.0M parameters (matching 3B), and train Qwen-3B with 9.4M parameters (matching 1.5B). These configurations allow us to compare models with equivalent trainable parameters but different base capacities. We evaluate these capacity-matched configurations across code generation, translation, and summarization tasks, reporting functional correctness alongside key quality metrics.

\begin{table}[h]
\centering
\caption{Parameter configurations for capacity-training experiments.}
\label{tab:param_configs}
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{llcccc}
\toprule
\textbf{Model} & \textbf{Configuration} & \textbf{r} & \textbf{$\alpha$} & \textbf{Trainable} & \textbf{\%} \\
\midrule
\multicolumn{6}{l}{\textit{Default configurations}} \\
Qwen-0.5B & Standard & 8 & 16 & 4.4M & 0.88\% \\
Qwen-1.5B & Standard & 8 & 16 & 9.3M & 0.59\% \\
Qwen-3B & Standard & 8 & 16 & 15.0M & 0.48\% \\
\midrule
\multicolumn{6}{l}{\textit{Capacity-matched experiments}} \\
Qwen-0.5B & \MTqlora$_{9.3M}$ (→1.5B match) & 17 & 32 & 9.3M & 1.86\% \\
Qwen-0.5B & \MTqlora$_{15M}$ (→3B match) & 27 & 54 & 14.8M & 2.92\% \\
Qwen-1.5B & \MTqlora$_{15M}$ (→3B match) & 13 & 26 & 15.0M & 0.96\% \\
Qwen-3B & \MTqlora$_{9.3M}$ (→1.5B match) & 5 & 10 & 9.4M & 0.30\% \\
\bottomrule
\end{tabular}
}
\end{table}

\textbf{Code Generation.} We begin by examining whether capacity-matched configurations replicate the performance of larger models in code generation, where RQ$_1$ and RQ$_2$ demonstrated that 3B models achieved superior \passatone scores and code quality compared to smaller variants. Capacity-matched experiments reveal that trainable parameter count alone does not close these performance gaps. For Python (\tabref{tab:rq_codegen_python}), \MTqlora$_{9.3M}$ (0.5B) achieves 16.84\% \passatone compared to standard \MTqlora (1.5B)'s 18.95\% (-2.11\%), while \MTqlora$_{15M}$ (0.5B) reaches only 14.74\% versus \MTqlora (3B)'s 21.05\% (-6.31\%). For \java (\tabref{tab:rq_codegen_java}), \MTqlora$_{15M}$ (0.5B) achieves 20.65\% compared to \MTqlora (3B)'s 32.07\% (-11.42\%), and \MTqlora$_{15M}$ (1.5B) reaches 27.17\%---falling 4.9\% short of \MTqlora (3B). Conversely, capacity-reduced 3B (\MTqlora$_{9.3M}$) maintains strong performance: 20.53\% for Python and 34.78\% for Java---exceeding standard \MTqlora (1.5B) despite fewer trainable parameters.

\input{tables/ext-cg-py}
\input{tables/ext-cg-java}

Static analysis tools reinforce this capacity advantage through quality metrics. Lizard's Cyclomatic Complexity analysis reveals that smaller models with matched parameters generate structurally more complex code. For Python, \MTqlora$_{9.3M}$ (0.5B) produces 913 CyC issues compared to standard \MTqlora (1.5B)'s 882, representing 3.5\% higher complexity despite identical trainable parameters. The disparity widens with \MTqlora$_{15M}$ (0.5B), which generates 975 CyC issues---44.0\% higher than standard \MTqlora (3B)'s 677. For Java, Lizard reports similar patterns: \MTqlora$_{9.3M}$ (0.5B) produces 710 CyC compared to standard \MTqlora (1.5B)'s 589 (+20.5\%), while \MTqlora$_{15M}$ (0.5B) shows 613 CyC versus standard \MTqlora (3B)'s 558 (+9.8\%).

SonarCloud's maintainability assessments further differentiate capacity from trainable parameters. For Python, \MTqlora$_{9.3M}$ (0.5B) accumulates 89 maintainability issues---23.6\% more than standard \MTqlora (1.5B)'s 72 issues---indicating that matched parameters cannot replicate the cleaner code patterns of larger models. \MTqlora$_{15M}$ (0.5B) shows 94 maintainability issues compared to standard \MTqlora (3B)'s 106. While this gap appears narrower (-11.3\%), the 0.5B model achieves this through different trade-offs, as evidenced by its substantially worse functional correctness (14.74\% vs 21.05\% \passatone) and higher Lizard complexity (975 vs 677 CyC).

Code size analysis provides additional evidence that base capacity drives efficiency. For Python, \MTqlora$_{15M}$ (0.5B) generates 2,467 LoC---40.3\% more than standard \MTqlora (3B)'s 1,759 LoC---despite matching trainable parameters. This verbosity extends to token counts: 15,486 tokens versus 11,773 (+31.5\%), suggesting smaller models require more elaborate implementations to approximate functionality. For Java, similar patterns emerge: \MTqlora$_{15M}$ (0.5B) produces 1,665 LoC compared to \MTqlora (3B)'s 1,580 (+5.4\%). Remarkably, the capacity-reduced \MTqlora$_{9.3M}$ (3B) maintains compact implementations (Python: 1,845 LoC; Java: 1,573 LoC) comparable to the standard \MTqlora (3B) configuration (Python: 1,759 LoC; Java: 1,580 LoC), demonstrating that base capacity enables concise solution expression even with constrained adaptation.

\textbf{Code Translation.} Translation tasks reveal distinct capacity requirements compared to code generation, with models struggling to maintain both functional correctness and translation validity when trainable parameters fall below critical thresholds. For Java→C\# (\tabref{tab:rq_codetrans_java2csharp}), \MTqlora$_{15M}$ (0.5B) achieves 71.79\% CodeBLEU, surprisingly outperforming standard \MTqlora (3B)'s 62.88\%, though this reflects the 3B model's unexpected underperformance in this task. \MTqlora$_{9.3M}$ (0.5B) drops to 60.98\% compared to standard \MTqlora (1.5B)'s 73.08\% (-12.1\%). For C\#→Java (\tabref{tab:rq_codetrans_csharp2java}), capacity limitations become severe: \MTqlora$_{9.3M}$ (0.5B) manages only 51.14\% against the 1.5B baseline's 70.72\% (-19.58\%), while \MTqlora$_{15M}$ (0.5B) reaches 59.45\%, still trailing the 3B baseline's 71.22\% by 11.77\%. Most revealing is \MTqlora$_{9.3M}$ (3B)'s catastrophic failure at 47.43\% CodeBLEU---underperforming even 0.5B variants despite substantial base capacity.

\input{tables/ext-ct-java-csharp}
\input{tables/ext-ct-sharp-java}

Static analysis exposes translation validity issues absent in code generation. Roslyn's assessment shows \MTqlora$_{9.3M}$ (0.5B) generating minimal syntax errors (11) but 1,476 maintainability issues---149\% more than standard \MTqlora (1.5B)'s 592. PMD's evaluation of C\#→Java reveals \MTqlora$_{9.3M}$ (3B) producing anomalous results: only 143 detectable issues with most categories returning N/A, indicating fundamental translation failures. This contrasts with \MTqlora$_{15M}$ (0.5B)'s 3,324 PMD issues---excessive but valid translations. Detection rates confirm this pattern: while most configurations maintain 95-99\% rates, \MTqlora$_{9.3M}$ (3B) drops to 78.6\% for C\#→Java, suggesting insufficient trainable parameters compromise translation validity regardless of base capacity.

Code size metrics reflect translation completeness rather than efficiency. \MTqlora$_{15M}$ (0.5B) generates surprisingly concise Java→C\# translations (5,965 LoC) compared to standard \MTqlora (3B)'s 5,890 LoC while achieving superior CodeBLEU. Conversely, \MTqlora$_{9.3M}$ (3B)'s apparent conciseness for C\#→Java (4,360 LoC vs baseline's 5,742) stems from incomplete translations, evidenced by its 25,278 tokens versus typical 35,000+ tokens for valid translations.

Unlike code generation where base capacity dominates, translation requires balanced capacity and trainable parameters. The $\approx$15M parameter threshold appears critical for maintaining translation validity---below which even 3B models produce invalid outputs. This bidirectional mapping complexity makes translation particularly sensitive to QLoRA configuration, demanding sufficient adaptation parameters as a prerequisite for functional translations.

\textbf{Code Summarization.} Completing our analysis across task types, summarization shifts from code-to-code transformations to code-to-natural-language generation--testing whether capacity advantages persist when crossing modality boundaries. Capacity-matched experiments reveal how this cross-modal mapping responds to parameter variations, particularly for Python where \MT training previously showed substantial advantages.

\input{tables/ext-cs}

Python summarization demonstrates clear capacity dominance. \MTqlora$_{9.3M}$ (0.5B) achieves 7.55\% BLEU against standard \MTqlora (1.5B)'s 12.60\%--40.1\% lower despite identical trainable parameters (\tabref{tab:rq_codesum_python}). \MTqlora$_{15M}$ (0.5B) reaches only 7.78\% BLEU, remaining 68.0\% below standard \MTqlora (3B)'s 24.33\%. Conversely, \MTqlora$_{9.3M}$ (3B) achieves 25.13\% BLEU--surpassing the standard 3B's 24.33\% while using 37\% fewer trainable parameters. \MTqlora$_{15M}$ (1.5B) attains 13.99\%, exceeding its standard configuration's 12.60\% by 11.0\%, demonstrating that modest parameter increases enhance performance when base capacity suffices.

Java summarization shows minimal sensitivity to configuration changes, clustering around 1.1-1.5\% BLEU (\tabref{tab:rq_codesum_java}). \MTqlora$_{9.3M}$ (0.5B) achieves 1.18\% versus standard \MTqlora (1.5B)'s 1.28\%, while \MTqlora$_{15M}$ (0.5B) drops to 1.11\%. \MTqlora$_{15M}$ (1.5B) reaches 1.5\%--the highest among variants--yet represents marginal improvement. \MTqlora$_{9.3M}$ (3B) maintains 1.33\% BLEU, indicating that neither capacity nor parameters substantially impact Java summarization.

LLM-as-judge evaluation (Appendix \ref{appendix:llm_judge}) reveals quality patterns beyond similarity metrics. Python Content Adequacy shows \MTqlora$_{9.3M}$ (0.5B) scoring 1.802 versus standard \MTqlora (1.5B)'s 1.862--only 3.2\% lower despite 40.1\% BLEU gap--suggesting smaller models capture essential content while struggling with reference phrasing. \MTqlora$_{9.3M}$ (3B) attains 1.946, comparable to standard 3B's 1.938, confirming capacity enables semantic understanding despite constrained adaptation. Java metrics remain stable: Content Adequacy ranges 2.154-2.339 (73-79\% of human baseline), Conciseness approaches perfection (4.925-4.990), and Fluency exceeds human baseline (4.226-4.408 vs 4.079).

These contrasting patterns illuminate task-specific requirements. Python summarization scales with base capacity--the 3B model with reduced parameters outperforms all smaller configurations through superior semantic understanding rather than parameter quantity. \java remains invariant to both factors, suggesting inherent task limitations that scaling cannot address. Practitioners should prioritize base capacity for scalable tasks (Python summarization) while recognizing that certain combinations (Java summarization) may not benefit from increased computational investment.
\end{comment}


==> sections/results-rq3.tex <==
% !TEX root = ../main.tex

\subsection{RQ3: Task-Specific Performance Patterns in \MT QLoRA}
\label{sec:rq3}

%Having demonstrated that \MT QLoRA achieves competitive performance when trained on all three tasks simultaneously (RQ$_1$, RQ$_2$), we now investigate whether specific task combinations yield different performance patterns. This research question examines whether joint training on selected task pairs induces positive transfer effects that enhance performance or introduces negative interference that degrades task-specific capabilities within QLoRA's constrained parameter space. Given that \MT QLoRA demonstrated strong performance across both functional correctness and quality metrics in RQ$_1$ and RQ$_2$, and that larger models consistently exhibited superior results, we focus our investigation on 3B QLoRA variants to maximize the potential for observing meaningful transfer effects. We train additional 3B models on two-task combinations--code generation with translation (CG+CT), code generation with summarization (CG+CS), and summarization with translation (CS+CT)--and compare their performance against the three-task \MT QLoRA baseline. We present results organized by task: code generation (\secref{sec:rq3_codegen}), code translation (\secref{sec:rq3_codetrans}), and code summarization (\secref{sec:rq3_codesum}), examining both functional correctness and code quality dimensions.

Having shown that \MT QLoRA achieves competitive performance when jointly trained on all three tasks (RQ$_1$ and RQ$_2$), we now examine whether alternative task combinations lead to different task-specific performance patterns. This research question investigates whether restricting training to selected task pairs induces positive transfer that improves performance or introduces negative interference that degrades task-specific capabilities under QLoRA’s constrained parameterization. Since \MT QLoRA exhibited its strongest and most consistent results at larger model scales in RQ$_1$ and RQ$_2$, we focus this analysis on the 3B setting to maximize sensitivity to transfer effects. We train additional 3B QLoRA variants on two-task combinations--code generation with translation (CG+CT), code generation with summarization (CG+CS), and summarization with translation (CS+CT)--and compare their performance against the three-task \MT QLoRA baseline. Results are reported by task: code generation (\secref{sec:rq3_codegen}), code translation (\secref{sec:rq3_codetrans}), and code summarization (\secref{sec:rq3_codesum}), considering both functional correctness and code quality.

\begin{comment}
    
\subsubsection{Code Generation}
\label{sec:rq3_codegen}

We evaluate whether specific task combinations yield different code generation performance compared to training on all three tasks. \tabref{tab:rq_codegen_python} and \tabref{tab:rq_codegen_java} compare two-task \MT QLoRA variants--CG+CT (code generation with translation) and CG+CS (code generation with summarization)--against the three-task \MT QLoRA baseline for the 3B model.

\input{tables/rq3-cg-py}
\input{tables/rq3-cg-java}

We begin by examining functional correctness to understand whether task selection influences the model's ability to generate executable solutions. For Python, the two-task variants show divergent behavior: \MTqlora (CG+CT) matches the three-task baseline exactly at 21.05\% \passatone, while \MTqlora (CG+CS) achieves only 19.47\%, representing a -1.58 percentage point decline, indicating neutral transfer from translation to code generation. For Java, the pattern reverses dramatically--both two-task variants substantially outperform the baseline, demonstrating strong positive transfer effects. \MTqlora (CG+CT) reaches 36.41\% \passatone, exceeding the baseline's 32.07\% by +4.34 points (13.5\% relative improvement), while \MTqlora (CG+CS) achieves 34.23\% (+2.16 points). These results reveal language-specific transfer dynamics: Java benefits from positive transfer effects when focusing on two tasks, while Python shows negative interference from summarization pairing (CG+CS) and neutral transfer from translation pairing (CG+CT).

To assess whether functional improvements come at the cost of code quality, we examine patterns across static analysis tools. For Python, both two-task variants demonstrate superior code quality despite neutral or negative functional impact. \MTqlora (CG+CS) shows particularly strong improvements: 6.6\% lower cyclomatic complexity (632 vs 677), 7.1\% fewer Pylint issues (2,341 vs 2,519), 67\% reduction in maintainability issues (35 vs 106), and 7.1\% lower cognitive complexity (510 vs 549). \MTqlora (CG+CT) achieves similar but more moderate quality gains while maintaining functional parity. For Java, the substantial functional correctness gains come at a quality cost. Both two-task variants show increased complexity and quality issues: CG+CT demonstrates 12.9\% higher cyclomatic complexity (630 vs 558), 81.3\% more Error Prone violations (58 vs 32), and 85.7\% more Performance issues (13 vs 7), while CG+CS shows more moderate increases across these dimensions. This reveals a fundamental trade-off: Python's two-task variants achieve superior maintainability but sacrifice (CG+CS) or maintain (CG+CT) correctness, while Java's variants gain substantial correctness at the expense of code quality.

Examining code size reveals that task combination impacts implementation conciseness differently across languages. For Python, \MTqlora (CG+CS) produces the most compact code (1,703 LoC, 10,461 tokens), representing 3.2\% fewer lines and 11.1\% fewer tokens than the three-task variant (1,759 LoC, 11,773 tokens), aligning with its superior quality metrics. For Java, \MTqlora (CG+CT) generates slightly longer implementations (1,654 LoC vs three-task variant's 1,580 LoC), corresponding with its highest \passatone and complexity, suggesting it achieves superior correctness through more elaborate rather than elegant solutions.

These findings reveal task-specific transfer patterns: Java exhibits strong positive transfer from both two-task combinations (particularly CG+CT), while Python shows negative interference from CG+CS despite quality improvements and neutral transfer from CG+CT. Optimal task selection for \MT QLoRA depends critically on the target programming language and whether practitioners prioritize functional correctness or code quality. For Java code generation, focusing on two tasks--particularly CG+CT--dramatically improves functional correctness at a modest quality cost. For Python, including all three tasks provides the best functional performance, though practitioners willing to sacrifice some correctness can achieve substantially better code quality through the CG+CS combination. The contrasting patterns suggest that Java benefits from concentrated \MT learning on complementary tasks, while Python requires broader task diversity to maximize functional correctness.
\end{comment}

% \subsubsection{Code Generation}
% \label{sec:rq3_codegen}

% We first analyze whether specific task pairings affect code generation performance relative to training on all three tasks. Tables~\ref{tab:rq3_codegen_python} and~\ref{tab:rq3_codegen_java} compare the two-task QLoRA variants--CG+CT and CG+CS--against the three-task baseline for the 3B model.

% \input{tables/rq3-cg-py}
% \input{tables/rq3-cg-java}

% Functional correctness results reveal distinct, language-dependent transfer patterns. For Python, the two-task variants exhibit divergent behavior. \MTqlora (CG+CT) matches the three-task baseline exactly at 21.05\% \passatone, indicating neutral transfer when pairing code generation with translation. In contrast, \MTqlora (CG+CS) attains 19.47\%, corresponding to a $-1.58$ percentage point decrease relative to the baseline, suggesting negative interference when summarization replaces translation. For Java, the trend reverses. Both two-task variants outperform the three-task baseline, indicating positive transfer effects. \MTqlora (CG+CT) achieves 36.41\% \passatone, exceeding the baseline’s 32.07\% by +4.34 points (13.5\% relative improvement), while \MTqlora (CG+CS) reaches 34.23\% (+2.16 points, 6.7\% relative improvement). These results indicate that Java code generation benefits from focused \MT training on complementary tasks, whereas Python is more sensitive to task composition.

% We next examine whether gains in functional correctness are accompanied by changes in code quality. For Python, both two-task variants improve quality metrics relative to the baseline despite neutral or negative effects on correctness. \MTqlora (CG+CS) exhibits the largest improvements: Cyclomatic Complexity decreases from 677 to 632 ($-6.6$\%), total Pylint violations decline from 2,519 to 2,341 ($-7.1$\%), SonarCloud Maintainability issues drop from 106 to 35 ($-67.0$\%), and Cognitive Complexity decreases from 549 to 510 ($-7.1$\%). Within Pylint categories, Errors decrease from 269 to 239 ($-11.2$\%), Warnings from 1,521 to 1,377 ($-9.5$\%), and Conventions from 673 to 666 ($-1.0$\%), while Refactoring issues increase slightly from 56 to 59 (+5.4\%). \MTqlora (CG+CT) shows more moderate quality improvements while preserving functional parity, reducing Cyclomatic Complexity to 656 ($-3.1$\%), total Pylint violations to 2,417 ($-4.1$\%), Maintainability issues to 73 ($-31.1$\%), and Cognitive Complexity to 544 ($-0.9$\%).

% For Java, improvements in functional correctness are accompanied by increased quality violations. \MTqlora (CG+CT) shows higher Cyclomatic Complexity (630 vs.\ 558, +12.9\%), increased PMD violations (1,518 vs.\ 1,441, +5.3\%), and higher SonarCloud issue counts (1,729 vs.\ 1,566, +10.4\%). PMD category-level analysis reveals increases in Best Practices (86 to 92, +7.0\%), Code Style (1,184 to 1,216, +2.7\%), Design (128 to 135, +5.5\%), Error Prone (32 to 58, +81.3\%), and Performance (7 to 13, +85.7\%), while Multi-threading remains unchanged. \MTqlora (CG+CS) exhibits similar but less pronounced trends, with Cyclomatic Complexity increasing to 593 (+6.3\%), PMD violations to 1,530 (+6.2\%), and SonarCloud issues to 1,661 (+6.1\%). Notably, Best Practices violations decrease from 86 to 75 ($-12.8$\%), whereas Error Prone (45 vs.\ 32, +40.6\%) and Performance (11 vs.\ 7, +57.1\%) violations increase. These results indicate a trade-off in Java, where higher correctness is achieved at the expense of increased complexity and quality issues.

% Code size metrics further contextualize these patterns. For Python, \MTqlora (CG+CS) produces the most compact implementations, generating 1,703 LoC compared to the baseline’s 1,759 ($-3.2$\%) and 10,461 tokens versus 11,773 ($-11.1$\%), consistent with its improved maintainability despite reduced correctness. \MTqlora (CG+CT) produces comparable code length (1,761 LoC, +0.1\%) with fewer tokens (11,202, $-4.9$\%). For Java, \MTqlora (CG+CT) generates longer implementations, with 1,654 LoC versus 1,580 (+4.7\%) and 11,704 tokens versus 10,920 (+7.2\%), suggesting that correctness gains are achieved through more elaborate solutions. \MTqlora (CG+CS) produces slightly more compact code (1,555 LoC, $-1.6$\%) with marginally higher token counts (11,194, +2.5\%).

% %\saima{stat part is needed}

% Overall, these results reveal clear language-specific transfer effects. For Java code generation, restricting training to two tasks--particularly CG+CT--yields substantial gains in functional correctness (+4.34 percentage points) while introducing moderate increases in complexity and quality violations. For Python, the three-task configuration remains optimal for maximizing correctness (21.05\%), whereas practitioners prioritizing code quality may prefer the CG+CS configuration, which achieves large reductions in maintainability issues ($-67.0$\%) at a modest cost in correctness ($-1.58$ points). These findings suggest that Java benefits from focused \MT learning on complementary code-to-code tasks, while Python code generation is more robust when trained across a broader set of code-to-code and code-to-text transformations.

% \input{tables/stat-tables/rq3-stat-cg}

% % To assess statistical significance, we conduct McNemar tests for \passatone and Wilcoxon signed-rank tests for quality metrics, with Holm-Bonferroni correction ($\alpha=0.05$), comparing three-task baseline against two-task variants. \tabref{tab:rq3-stat} presents complete results. For Python, no \passatone differences reach significance (CG+CS: $p=1.00$, CG+CT: $p=1.00$), with negligible effect sizes across quality metrics ($|d| \leq 0.101$). For Java, \passatone remains non-significant (CG+CS: $p=1.00$, CG+CT: $p=0.68$) despite practical advantages for two-task variants, with all quality metrics showing negligible effects ($|d| \leq 0.088$). These results indicate that task selection effects, while statistically detectable in isolated metrics, produce predominantly negligible practical differences.

% To assess statistical significance, we conduct McNemar tests for \passatone and Wilcoxon signed-rank tests for quality metrics, with Holm-Bonferroni correction ($\alpha=0.05$), comparing three-task baseline against two-task variants. \tabref{tab:rq3-stat} presents complete results. For Python, no \passatone differences reach significance (CG+CS: $p=1.00$, CG+CT: $p=1.00$). For Java, \passatone remains non-significant (CG+CS: $p=1.00$, CG+CT: $p=0.68$) despite practical advantages for two-task variants. These results indicate that task selection effects, while statistically detectable in isolated quality metrics, produce predominantly minor practical differences.


% \subsubsection{Code Translation}
% \label{sec:rq3_codetrans}

% \begin{comment}
% Having examined how task combinations affect code generation, we now investigate whether similar patterns emerge for code translation. \tabref{tab:rq_codetrans_java2csharp} and \tabref{tab:rq_codetrans_csharp2java} compare two-task \MT QLoRA variants--CG+CT (code generation with translation) and CS+CT (code summarization with translation)--against the three-task \MT QLoRA baseline for the 3B model across both Java→C\# and C\#→Java directions.

% \input{tables/rq3-ct-java-csharp}
% \input{tables/rq3-ct-csharp-java}

% For Java→C\#, the two-task variants show dramatically divergent behavior: \MTqlora (CG+CT) achieves 73.71\% compared to the three-task variant's 62.88\% (+10.83 percentage points, 17.2\% relative improvement), while \MTqlora (CS+CT) achieves only 5.35\% (-57.53 percentage points, 91.5\% relative decline). For C\#→Java, the pattern is similar: \MTqlora (CG+CT) reaches 72.48\% compared to 71.22\% (+1.26\%), while \MTqlora (CS+CT) achieves 7.35\% (-63.87 points, 89.7\% relative decline). These results reveal distinct patterns: the CG+CT combination demonstrates substantial functional improvements for Java→C\# and maintains competitive performance for C\#→Java, while the CS+CT combination shows severe functional degradation across both translation directions.

% To assess the impact on translation quality, we examine patterns across static analysis tools. For Java→C\#, where Lizard and Roslyn provide comprehensive assessment, the three-task baseline produces 1,455 total Cyclomatic Complexity issues, 126 syntax errors, and 3,061 maintainability issues. \MTqlora (CG+CT) generates 1,560 CyC issues (+7.2\%), 302 syntax errors (+139.7\%), and 820 maintainability issues (-73.2\%). \MTqlora (CS+CT) produces 251 CyC issues, 68 syntax errors, and 1,828 maintainability issues, though these occur alongside a dramatically reduced detection rate of 19.8\% compared to the baseline's 93.6\%. For C\#→Java, where Lizard, PMD, and SonarCloud provide comprehensive assessment, the baseline produces 1,612 Lizard CyC issues, 1,171 total PMD issues (summing Best Practices: 37, Code Style: 1,072, Design: 45, Error Prone: 11, Multi-threading: 5, Performance: 1), and 757 total SonarCloud quality issues. \MTqlora (CG+CT) generates 1,583 Lizard CyC issues (-1.8\%), 2,773 total PMD issues (+136.8\%), and 1,928 total SonarCloud quality issues (+154.7\%). Breaking down the PMD increases: Best Practices rises to 99 from 37 (+167.6\%), Code Style increases to 2,453 from 1,072 (+128.8\%), Design grows to 144 from 45 (+220\%), Error Prone rises to 44 from 11 (+300\%), Multi-threading increases to 12 from 5 (+140\%), and Performance grows to 21 from 1 (+2,000\%). \MTqlora (CS+CT) produces 280 Lizard CyC issues with most PMD categories unmeasurable and 1,364 total SonarCloud quality issues, again occurring with a severely reduced detection rate of 20.9\%. These results reveal that CG+CT achieves substantial functional improvements for Java→C\# while reducing maintainability issues, but introduces significant quality degradation across most C\#→Java metrics despite marginal functional gains. The CS+CT combination shows severely reduced detection rates across both directions, indicating fundamental challenges in producing valid translations.

% Examining Cyclomatic Complexity patterns reveals mixed effects across task combinations. For Java→C\#, \MTqlora (CG+CT) shows 1,560 CyC compared to the three-task variant's 1,455 (+7.2\%), while \MTqlora (CS+CT) produces 251 CyC issues alongside its low detection rate. For C\#→Java, \MTqlora (CG+CT) demonstrates 1,583 CyC compared to 1,612 (-1.8\%), representing a slight reduction, while \MTqlora (CS+CT) shows 280 CyC issues. The relatively stable or slightly improved complexity for CG+CT in C\#→Java, despite substantial increases in other quality metrics, suggests differential impacts across quality dimensions.

% For Roslyn metrics in Java→C\# translation, \MTqlora (CG+CT) shows substantial increases: 302 syntax errors compared to the baseline's 126 (+139.7\%), while maintainability issues decrease dramatically to 820 from 3,061 (-73.2\%). This trade-off--increased syntax violations but substantially improved maintainability--suggests different optimization priorities. For C\#→Java translation, PMD analysis reveals that \MTqlora (CG+CT) produces substantially more issues across nearly all categories. Code Style violations increase from 1,072 to 2,453 (+128.8\%), Design issues grow from 45 to 144 (+220\%), Error Prone violations rise from 11 to 44 (+300\%), and Performance issues increase from 1 to 21 (+2,000\%). SonarCloud metrics for C\#→Java show similar patterns: \MTqlora (CG+CT) produces 653 maintainability issues versus the baseline's 278 (+134.9\%), reliability issues increase to 15 from 0, cyclomatic complexity rises to 841 from 322 (+161.2\%), and cognitive complexity grows to 404 from 157 (+157.3\%). These substantial quality degradations in CG+CT for C\#→Java, despite maintaining functional correctness, indicate that task focus optimizes for translation accuracy at the expense of adherence to Java coding standards.

% Examining code size reveals that task combinations produce varying implementation sizes. For Java→C\#, \MTqlora (CG+CT) generates 6,342 LoC compared to the baseline's 5,890 (+7.7\%), with token count at 40,752 versus 37,716 (+8.0\%). \MTqlora (CS+CT) produces 845 LoC with 4,417 tokens, though this occurs alongside its severely reduced functionality. For C\#→Java, \MTqlora (CG+CT) generates 5,746 LoC compared to 5,742 (+0.07\%), with token count at 34,654 versus 34,862 (-0.6\%). \MTqlora (CS+CT) produces 850 LoC with 4,597 tokens. The substantially reduced code size for CS+CT in both directions, combined with low detection rates, suggests incomplete or invalid translations.

% These findings reveal task-specific transfer patterns in code translation. The CG+CT combination achieves substantial functional improvements for Java→C\# (+17.2\% relative improvement in CodeBLEU) while reducing maintainability issues by 73.2\%, though at the cost of increased syntax errors. For C\#→Java, CG+CT demonstrates marginal functional improvements (+1.8\%) but substantial quality degradation across most metrics, with increases ranging from 128.8\% to 2,000\% across PMD categories. The CS+CT combination shows severe functional degradation in both directions (over 89\% relative decline in CodeBLEU), accompanied by detection rates below 21\%, indicating fundamental limitations when code generation is excluded from the task combination. The contrasting patterns suggest that code generation and translation may share complementary learning objectives, while code summarization provides limited transfer benefit for translation tasks within the constrained parameter space of \MT QLoRA.
% \end{comment}

% Having examined how task combinations influence code generation, we now assess whether similar transfer effects arise for code translation. Tables~\ref{tab:rq3_codetrans_java2csharp} and~\ref{tab:rq3_codetrans_csharp2java} compare two-task \MT QLoRA variants--CG+CT (code generation with translation) and CS+CT (code summarization with translation)--against the three-task \MT QLoRA baseline for the 3B model, across both Java$\rightarrow$C\# and C\#$\rightarrow$Java translation directions.

% \input{tables/rq3-ct-java-csharp}
% \input{tables/rq3-ct-csharp-java}

% Functional correctness results reveal strongly divergent behaviors across task combinations. For Java$\rightarrow$C\#, \MTqlora (CG+CT) achieves a CodeBLEU score of 73.71\% compared to the three-task baseline’s 62.88\% ($+10.83$ points, $+17.2$\% relative improvement), whereas \MTqlora (CS+CT) attains only 5.35\% ($-57.53$ points, $-91.5$\% relative decline). A similar pattern is observed for C\#$\rightarrow$Java: \MTqlora (CG+CT) reaches 72.48\% compared to the baseline’s 71.22\% ($+1.26$ points, $+1.8$\% relative improvement), while \MTqlora (CS+CT) achieves 7.35\% ($-63.87$ points, $-89.7$\% relative decline). These results indicate that pairing code generation with translation yields consistent functional benefits, whereas excluding code generation leads to severe degradation in translation performance.

% We next examine whether these functional outcomes are accompanied by corresponding changes in code quality. For Java$\rightarrow$C\#, where Lizard and Roslyn provide assessment, the three-task baseline produces 1,455 Cyclomatic Complexity (CyC) issues, 126 syntax errors, and 3,061 maintainability issues. \MTqlora (CG+CT) generates higher CyC (1,560, $+7.2$\%) and more syntax errors (302, $+139.7$\%), but substantially fewer maintainability issues (820, $-73.2$\%). This combination of higher syntax violations alongside markedly reduced maintainability findings suggests that the model prioritizes functional correctness and longer-term structural quality, albeit at the expense of syntactic robustness. In contrast, \MTqlora (CS+CT) produces 251 CyC issues, 68 syntax errors, and 1,828 maintainability issues; however, these values correspond to a sharply reduced detection rate of 19.8\% relative to the baseline’s 93.6\%, indicating that most translation attempts fail to yield analyzable code.

% For C\#$\rightarrow$Java, where Lizard, PMD, and SonarCloud are applicable, the three-task baseline yields 1,612 CyC issues, 1,171 PMD violations, and 757 SonarCloud quality issues. \MTqlora (CG+CT) exhibits mixed quality outcomes: Cyclomatic Complexity decreases slightly to 1,583 ($-1.8$\%), while PMD violations increase to 2,773 ($+136.8$\%) and SonarCloud issues rise to 1,928 ($+154.7$\%). PMD category-level analysis shows increases across all dimensions, including Best Practices (37 to 99, $+167.6$\%), Code Style (1,072 to 2,453, $+128.8$\%), Design (45 to 144, $+220.0$\%), Error Prone (11 to 44, $+300.0$\%), Multi-threading (5 to 12, $+140.0$\%), and Performance (1 to 21, $+2{,}000.0$\%). SonarCloud metrics reflect similar trends, with increases in Maintainability (278 to 653, $+134.9$\%), Reliability (0 to 15), Cyclomatic Complexity (322 to 841, $+161.2$\%), and Cognitive Complexity (157 to 404, $+157.3$\%). These quality degradations occur alongside only marginal functional gains ($+1.26$ CodeBLEU points), indicating that the CG+CT configuration favors translation accuracy at the expense of adherence to Java coding standards.

% \MTqlora (CS+CT) for C\#$\rightarrow$Java produces 280 CyC issues with a detection rate of 20.9\%, substantially lower than the baseline’s 99.5\%. Most PMD categories are not applicable (N/A in Table~\ref{tab:rq3_codetrans_csharp2java}), with only Best Practices violations measurable (2,050). SonarCloud reports 1,360 maintainability issues, 4 cyclomatic complexity issues, and 0 cognitive complexity issues; however, these figures must be interpreted in light of the severely reduced detection rate. The combination of low functional correctness (7.35\% CodeBLEU) and limited analyzability indicates fundamental challenges in producing valid translations when code generation is excluded from training.

% Code size metrics provide additional insight into these behaviors. For Java$\rightarrow$C\#, \MTqlora (CG+CT) generates 6,342 lines of code compared to the baseline’s 5,890 ($+7.7$\%), with 40,752 tokens versus 37,716 ($+8.0$\%), suggesting more elaborate implementations associated with higher functional correctness. \MTqlora (CS+CT) produces only 845 lines of code and 4,417 tokens, consistent with its reduced functionality. For C\#$\rightarrow$Java, \MTqlora (CG+CT) generates 5,746 lines of code compared to 5,742 ($+0.07$\%), with 34,654 tokens versus 34,862 ($-0.6$\%), indicating comparable code size despite quality trade-offs. \MTqlora (CS+CT) produces 850 lines of code and 4,597 tokens. Across both directions, the markedly smaller outputs for CS+CT, combined with detection rates below 21\%, are indicative of incomplete or syntactically invalid translations.

% \input{tables/stat-tables/rq3-stat-ct}

% % To assess statistical significance, we conduct Wilcoxon signed-rank tests with Holm-Bonferroni correction ($\alpha=0.05$) comparing three-task baseline against two-task variants. \tabref{tab:rq3-stat-translation} presents complete results. For Java$\rightarrow$C\#, CG+CT shows significant improvement ($p<0.01$, $d=-0.271$, small effect) with large maintainability gains ($d=0.566$), while CS+CT exhibits catastrophic failure with large negative effects across all metrics ($d=0.688$--$0.831$). For C\#$\rightarrow$Java, CG+CT demonstrates marginal significant improvement ($p<0.01$, $d=-0.118$) with small quality degradation effects ($d=-0.300$ to $-0.319$), while CS+CT shows severe failure with large functional effect ($d=0.760$) and large quality degradation ($d=0.809$--$0.853$). These results confirm that task combination critically impacts translation validity and quality.

% To assess statistical significance, we conduct Wilcoxon signed-rank tests with Holm-Bonferroni correction ($\alpha=0.05$) comparing three-task baseline against two-task variants. \tabref{tab:rq3-stat-translation} presents complete results. For Java$\rightarrow$C\#, CG+CT shows significant improvement ($p<0.01$), while CS+CT exhibits catastrophic failure across all metrics ($p<0.01$). For C\#$\rightarrow$Java, CG+CT demonstrates marginal significant improvement ($p<0.01$), while CS+CT shows severe failure ($p<0.01$). These results confirm that task combination critically impacts translation validity and quality.

% Overall, these findings reveal distinct task-specific transfer effects for code translation. The CG+CT configuration yields substantial functional improvements for Java$\rightarrow$C\# ($+10.83$ points, $+17.2$\% relative improvement) while reducing maintainability issues by $73.2$\%, albeit with increased syntax errors ($+139.7$\%). For C\#$\rightarrow$Java, CG+CT produces only marginal functional gains ($+1.26$ points) accompanied by pronounced degradation in code quality, with PMD and SonarCloud violations increasing by $128.8$\% to $2{,}000.0$\% across categories. In contrast, the CS+CT configuration exhibits severe functional degradation in both translation directions (relative declines of $89.7$\% to $91.5$\%), alongside detection rates below 21\%, indicating limited viability when code generation is excluded. Taken together, these results suggest that code generation and translation share complementary representational requirements as code-to-code tasks, whereas code summarization provides limited transfer benefit for translation within QLoRA’s constrained parameter space.

% %\saima{stat part missing?}

% %\saima{stop here}

% \begin{comment}
% \subsubsection{Code Summarization}
% \label{sec:rq3_codesum}

% Having established in RQ$_1$ and RQ$_2$ that \MT QLoRA achieves competitive summarization performance when trained on all three tasks simultaneously--with Python demonstrating dramatic improvements (100.6\% relative BLEU gain for 3B) while Java maintains stable quality--we now examine whether specific task pairings preserve these benefits or introduce the interference patterns observed in code generation and translation. \secref{sec:rq3_codegen} revealed that Java benefits from concentrated two-task learning while Python requires broader task diversity for generation, and \secref{sec:rq3_codetrans} demonstrated that excluding code translation (CS+CT) causes catastrophic translation failure. We investigate whether similar task dependencies emerge for code summarization, or whether the distinct nature of generating natural language descriptions produces different transfer patterns.

% \input{tables/rq3-cs}

% For Python, the two-task variants demonstrate strikingly different performance profiles. \MTqlora (CG+CS) maintains competitive performance with the three-task baseline across all overlap-based metrics: BLEU achieves 23.76\% compared to the \MTqlora with three task 24.33\% (2.3\% relative decline), METEOR reaches 31.5\% compared to 32.88\% (4.2\% decline), Rouge-L attains 46.02\% compared to 45.35\% (1.5\% improvement), and chrF demonstrates 39.83\% compared to 40.98\% (-1.15 points, 2.8\% decline). The contextual metric BERTScore shows 73.85\% compared to 72.85\% (+1.0 point). These modest variations--all within 5\% relative difference--indicate that pairing code generation with summarization preserves the model's ability to produce high-quality natural language descriptions of code.

% In sharp contrast, \MTqlora (CS+CT) exhibits severe performance degradation across all metrics: BLEU drops to 11.9\% from the \MTqlora with three task 24.33\% (51.1\% relative decline), METEOR falls to 20.51\% from 32.88\% (37.6\% decline), Rouge-L decreases to 35.13\% from 45.35\% (22.5\% decline), chrF drops to 28.41\% from 40.98\% (30.7\% decline), and BERTScore declines to 67.21\% from 72.85\% (7.7\% decline). This catastrophic failure pattern with BLEU declining by over 50\% suggests that combining summarization with translation introduces fundamental conflicts in the learning objectives within the limited adapter parameter space, preventing the model from developing effective representations for generating natural language summaries. The pattern mirrors the CS+CT translation failures observed in \secref{sec:rq3_codetrans}, reinforcing that code generation appears essential for effective \MT learning.

% For Java, the pattern differs markedly from Python, with both two-task variants maintaining stable performance relative to the three-task baseline. \MTqlora (CG+CS) shows marginal changes across overlap-based metrics: BLEU achieves 1.37\% compared to the baseline's 1.51\%, METEOR reaches 12\% compared to 12.11\%, Rouge-L attains 26.21\% compared to 25.60\%, and chrF demonstrates 16.39\% compared to 16.37\%. The contextual metrics present a similar stable picture: BERTScore shows 59.13\% compared to 59.20\%, while SIDE improves slightly from 91.58\% to 91.79\%. \MTqlora (CS+CT) similarly maintains competitive performance: BLEU reaches 1.49\% compared to 1.51\%, METEOR achieves 12.55\% compared to 12.11\%, Rouge-L attains 26.21\% compared to 25.60\%, chrF demonstrates 16.7\% compared to 16.37\%, BERTScore shows 59.84\% compared to 59.20\%, and SIDE reaches 91.67\% compared to 91.58\%. All variations remain within 1 percentage point across metrics, indicating that Java summarization maintains robustness regardless of task pairing.

% To assess whether functional metric variations translate into perceived quality differences, we examine GPT-5 mini quality scores across the three quality dimensions. Complete distributions are presented in Appendix \ref{appendix:llm_judge} (\figref{fig:llm_judge_java} and \figref{fig:llm_judge_python}). For Python, examining Content Adequacy reveals that the quality assessment partially aligns with functional metrics. The three-task baseline achieves 1.938, CG+CS reaches 1.974 (+0.036), and CS+CT attains 1.914 (-0.024). Despite CS+CT's 51\% BLEU decline, its Content Adequacy score decreases by only 1.2\% relative to the baseline, remaining within the same general quality tier (69-74\% of human baseline at 2.636). This discrepancy suggests that while CS+CT produces summaries with substantially lower lexical similarity to references, the semantic content coverage remains relatively preserved. Conciseness scores show minimal variation: baseline at 4.624, CG+CS at 4.672 (+0.048), and CS+CT at 4.678 (+0.054), all approaching the human baseline (4.800). Fluency scores similarly remain stable: baseline at 3.812, CG+CS at 3.898 (+0.086), and CS+CT at 3.834 (+0.022). The convergence of quality scores across task combinations--despite dramatic functional metric differences--indicates that CS+CT's failure manifests primarily in the model's inability to reproduce reference-like phrasings rather than in generating fundamentally lower-quality or less understandable summaries.

% For Java, the quality assessment reinforces the functional metric findings, showing minimal variation across task combinations. Content Adequacy scores demonstrate remarkable stability: baseline at 2.293, CG+CS at 2.301 (+0.008), and CS+CT at 2.317 (+0.024), all representing 77-78\% of the human baseline (2.960). Conciseness scores remain consistently high: baseline at 4.980, CG+CS at 4.996 (+0.016), and CS+CT at 4.984 (+0.004), all exceeding the human baseline (4.620). Fluency scores similarly show minimal differences: baseline at 4.408, CG+CS at 4.475 (+0.067), and CS+CT at 4.459 (+0.051), all approaching human quality (4.079). The tight clustering of scores across all three dimensions--with maximum variations under 2\%--confirms that Java summarization maintains quality parity regardless of which tasks are paired during \MT training.

% These findings reveal fundamental task dependency patterns in \MT QLoRA for code summarization. For Python, the three-task baseline demonstrates superior performance compared to both two-task variants: it substantially outperforms CS+CT (BLEU 24.33\% vs 11.9\%) while maintaining marginal advantages over CG+CS across most metrics. The CS+CT combination's catastrophic failure (over 50\% BLEU decline) establishes code generation as an essential component for effective \MT learning within QLoRA's limited adapter parameter space. For Java, the three-task baseline maintains comparable performance with both two-task variants, with all configurations achieving similarly modest effectiveness (BLEU variations within 0.14, all below 1.6\%). This stability across task combinations, despite the low absolute BLEU scores (1.37-1.51\%), suggests that Java summarization presents fundamental challenges that persist regardless of task pairing strategy. The relatively stable performance may reflect either that Java's more verbose syntax and formal structure make lexical similarity to references harder to achieve, or that the modest baseline performance leaves limited room for further degradation. The contrasting patterns across languages demonstrate that Python summarization clearly benefits from the broader task diversity provided by three-task training, while Java shows no meaningful advantage from any specific task combination, indicating that improving Java summarization quality may require approaches beyond task selection optimization.
% \end{comment}

% \subsubsection{Code Summarization}
% \label{sec:rq3_codesum}

% Building on RQ$_1$ and RQ$_2$, where \MT QLoRA demonstrated competitive summarization performance when trained on all three tasks--with substantial gains for Python and stable quality for Java--we now examine whether specific task pairings preserve these benefits or introduce interference effects. Prior analysis in \secref{sec:rq3_codegen} showed that Java benefits from concentrated two-task learning, whereas Python requires broader task diversity for code generation. Similarly, \secref{sec:rq3_codetrans} revealed that excluding code generation (CS+CT) leads to severe degradation in translation performance. Here, we investigate whether analogous task dependencies arise for code summarization. Table~\ref{tab:rq3_codesum} compares two-task \MT QLoRA variants--CG+CS (code generation with summarization) and CS+CT (code summarization with translation)--against the three-task \MT QLoRA baseline for the 3B model.

% \input{tables/rq3-cs}

% Performance patterns reveal strong language-dependent sensitivity to task combinations. For Python, the two-task variants exhibit sharply contrasting behaviors. \MTqlora (CG+CS) maintains performance close to the three-task baseline across all metrics: BLEU achieves 23.76\% vs.\ 24.33\% ($-0.57$), METEOR reaches 31.50\% vs.\ 32.88\% ($-1.38$), Rouge-L attains 46.02\% vs.\ 45.35\% ($+0.67$), chrF reaches 39.83\% vs.\ 40.98\% ($-1.15$), and BERTScore improves to 73.85\% vs.\ 72.85\% ($+1.00$). All differences remain within a 5\% relative range, indicating that pairing code generation with summarization largely preserves summarization capability.

% In contrast, \MTqlora (CS+CT) exhibits severe degradation across all metrics: BLEU drops to 11.90\% vs.\ 24.33\% ($-12.43$), METEOR falls to 20.51\% vs.\ 32.88\% ($-12.37$), Rouge-L declines to 35.13\% vs.\ 45.35\% ($-10.22$), chrF decreases to 28.41\% vs.\ 40.98\% ($-12.57$), and BERTScore falls to 67.21\% vs.\ 72.85\% ($-5.64$). The BLEU reduction alone corresponds to a $-51.1$\% relative decline, indicating that combining summarization with translation while excluding code generation introduces substantial interference within QLoRA’s constrained adapter space. This failure mode mirrors the CS+CT translation degradation observed in \secref{sec:rq3_codetrans}, reinforcing the central role of code generation in effective \MT learning.

% For Java, performance remains notably stable across task combinations. \MTqlora (CG+CS) exhibits minimal deviations from the three-task baseline: BLEU reaches 1.37\% vs.\ 1.51\% ($-0.14$), METEOR achieves 12.00\% vs.\ 12.11\% ($-0.11$), Rouge-L improves to 26.21\% vs.\ 25.60\% ($+0.61$), chrF increases slightly to 16.39\% vs.\ 16.37\% ($+0.02$), BERTScore reaches 59.13\% vs.\ 59.20\% ($-0.07$), and SIDE improves to 91.79\% vs.\ 91.58\% ($+0.21$). \MTqlora (CS+CT) similarly maintains parity: BLEU achieves 1.49\% vs.\ 1.51\% ($-0.02$), METEOR improves to 12.55\% vs.\ 12.11\% ($+0.44$), Rouge-L reaches 26.21\% vs.\ 25.60\% ($+0.61$), chrF increases to 16.70\% vs.\ 16.37\% ($+0.33$), BERTScore improves to 59.84\% vs.\ 59.20\% ($+0.64$), and SIDE reaches 91.67\% vs.\ 91.58\% ($+0.09$). All variations remain within narrow absolute margins, indicating that Java summarization is largely insensitive to task pairing.

% We further examine whether functional metric differences translate into perceived quality differences using GPT-5 mini evaluations. Full distributions are reported in Appendix~\ref{appendix:llm_judge} (Figures~\ref{fig:llm_judge_java} and~\ref{fig:llm_judge_python}). 

% For Python, quality assessments partially align with functional trends. Content Adequacy scores show the three-task baseline at 1.938, CG+CS at 1.974 vs.\ 1.938 ($+0.036$), and CS+CT at 1.914 vs.\ 1.938 ($-0.024$). Despite CS+CT exhibiting a $-51.1$\% BLEU decline, Content Adequacy decreases by only $-1.2$\%, remaining within the same qualitative tier (69--74\% of the human baseline at 2.636). Conciseness remains stable across configurations: baseline at 4.624, CG+CS at 4.672 vs.\ 4.624 ($+0.048$), and CS+CT at 4.678 vs.\ 4.624 ($+0.054$). Fluency similarly shows minor variation: baseline at 3.812, CG+CS at 3.898 vs.\ 3.812 ($+0.086$), and CS+CT at 3.834 vs.\ 3.812 ($+0.022$). These results suggest that CS+CT primarily degrades reference-level similarity rather than semantic coverage or readability.

% For Java, quality metrics further confirm robustness across task combinations. Content Adequacy remains nearly unchanged: baseline at 2.293, CG+CS at 2.301 vs.\ 2.293 ($+0.008$), and CS+CT at 2.317 vs.\ 2.293 ($+0.024$), corresponding to 77--78\% of the human baseline (2.960). Conciseness remains high across all configurations: baseline at 4.980, CG+CS at 4.996 vs.\ 4.980 ($+0.016$), and CS+CT at 4.984 vs.\ 4.980 ($+0.004$). Fluency shows similarly small differences: baseline at 4.408, CG+CS at 4.475 vs.\ 4.408 ($+0.067$), and CS+CT at 4.459 vs.\ 4.408 ($+0.051$). All variations remain below 2\%, indicating consistent perceived quality.

% %\saima{stat res?}

% \input{tables/stat-tables/rq3-stat-cs}

% % To assess statistical significance, we conduct Wilcoxon signed-rank tests with Holm-Bonferroni correction ($\alpha=0.05$) comparing three-task baseline against two-task variants. \tabref{tab:rq3-stat-summarization} presents complete results. For Java, no significant differences emerge for either CG+CS ($p \geq 1.00$) or CS+CT ($p \geq 0.37$), with negligible effect sizes ($|d| \leq 0.058$). For Python, CG+CS shows no significant differences ($p \geq 0.80$, $|d| \leq 0.032$), while CS+CT demonstrates significant degradation across all metrics ($p<0.01$) with small effect sizes ($d=0.208$--$0.229$). These results confirm Java summarization maintains stability across task combinations, while Python requires three-task diversity with CS+CT producing statistically significant performance decline.

% To assess statistical significance, we conduct Wilcoxon signed-rank tests with Holm-Bonferroni correction ($\alpha=0.05$) comparing three-task baseline against two-task variants. \tabref{tab:rq3-stat-summarization} presents complete results. For Java, no significant differences emerge for either CG+CS ($p \geq 1.00$) or CS+CT ($p \geq 0.37$). For Python, CG+CS shows no significant differences ($p \geq 0.80$), while CS+CT demonstrates significant degradation across all metrics ($p<0.01$). These results confirm Java summarization maintains stability across task combinations, while Python requires three-task diversity with CS+CT producing statistically significant performance decline.

% Overall, these results reveal clear task dependency patterns for code summarization under \MT QLoRA. For Python, the three-task baseline remains optimal, substantially outperforming CS+CT (BLEU 24.33\% vs.\ 11.90\%, $-12.43$) while offering marginal advantages over CG+CS across most metrics. The pronounced failure of CS+CT establishes code generation as a critical component for effective \MT summarization. For Java, all configurations exhibit comparable performance, with BLEU scores varying narrowly between 1.37\% and 1.51\% ($\pm0.14$). This stability suggests that Java summarization performance is constrained by factors beyond task pairing, and that improvements may require strategies other than task selection within QLoRA’s parameter-efficient framework.


% % \noindent\textit{\textbf{Summary of RQ3: Task-Specific Performance Patterns in \MT QLoRA.}
% % We examine how task pair combinations affect performance compared to three-task training, investigating positive transfer versus negative interference within QLoRA's constrained parameter space. For code generation, Java benefits from two-task combinations with CG+CT achieving highest pass@1, while Python three-task training remains optimal for correctness. For code translation, code generation proves critical—CG+CT yields substantial Java→C\# gains, while CS+CT exhibits catastrophic collapse in both directions with detection rates below 21\%. For summarization, Python three-task baseline substantially outperforms CS+CT, while Java remains insensitive to task pairing. Overall, code generation is essential for effective \MT learning, and excluding it causes severe degradation across translation and summarization tasks.}
% \vspace{10pt}

% \begin{tcolorbox}[
%     colback=gray!10, 
%     colframe=black, 
%     arc=5mm, 
%     colupper=black, 
%     boxrule=1pt,
%     title={\textbf{Summary of RQ3: Task-Specific Performance Patterns in \MT QLoRA}}, 
%     coltitle=white,
%     colbacktitle=black,
%     toptitle=1mm,
%     bottomtitle=1mm,
%     left=6pt, 
%     right=6pt, 
%     top=6pt, 
%     bottom=6pt
% ]
% \justifying
% % We examine how task pair combinations affect performance compared to three-task training, investigating positive transfer versus negative interference within QLoRA's constrained parameter space.
% % For \textit{code generation}, language-specific patterns emerge. Java benefits from two-task combinations: CG+CT achieves highest \passatone (exceeding three-task baseline) despite increased complexity, while CG+CS shows improvements with moderate trade-offs. For Python, three-task training remains optimal for correctness, though CG+CS provides substantial quality gains at modest correctness cost.
% % For \textit{code translation}, code generation proves critical. CG+CT yields substantial Java→C\# gains with fewer maintainability issues (despite increased syntax errors) and marginal C\#→Java improvements (with quality degradation across PMD/SonarCloud). Catastrophically, CS+CT exhibits severe collapse in both directions (detection rates below 21\%), demonstrating fundamental failures without code generation.
% % For \textit{code summarization}, task dependencies mirror translation. Python three-task baseline substantially outperforms CS+CT, while CG+CS maintains near-baseline performance. Java remains insensitive to task pairing across all combinations.
% We examine how task pair combinations affect performance compared to three-task training, investigating positive transfer versus negative interference within QLoRA's constrained parameter space. For code generation, Java benefits from two-task combinations with CG+CT achieving highest pass@1, while Python three-task training remains optimal for correctness. For code translation, code generation proves critical--CG+CT yields substantial Java→C\# gains, while CS+CT exhibits catastrophic collapse in both directions with detection rates below 21\%. For summarization, Python three-task baseline substantially outperforms CS+CT, while Java remains insensitive to task pairing. Overall, code generation is essential for effective \MT learning, and excluding it causes severe degradation across translation and summarization tasks.
% \end{tcolorbox}


==> tables/ext-cg-java.tex <==
\begin{table}[h]
\centering
\scriptsize
\caption{Capacity-matched configurations for \java code generation on CoderEval. \MTqlora$_{9.3M}$ and \MTqlora$_{15M}$ denote parameter-matched variants. Bold indicates best Pass@1 within each model size.}
\label{tab:extended_codegen_java}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{lc|c|cccc|cccccc|ccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Method}} & 
\multirow{2}{*}{\textbf{Pass@1}} & 
\multicolumn{4}{c|}{\textbf{Lizard}} & 
\multicolumn{6}{c|}{\textbf{PMD}} &
\multicolumn{5}{c}{\textbf{SonarCloud}} \\
\cmidrule(lr){4-7} \cmidrule(lr){8-13} \cmidrule(l){14-18}
& & & \textbf{LoC} & \textbf{Tok} & \textbf{DR} & \textbf{CyC} & 
\textbf{Best Prac.} & \textbf{CS} & \textbf{Design} & \textbf{EP} & \textbf{MT} & \textbf{Perf.} &
\textbf{Sec} & \textbf{Rel} & \textbf{Main} & \textbf{CyC} & \textbf{CoC} \\
\midrule
\multirow{3}{*}{\textit{Qwen-0.5B}} 
& \MTqlora & 20.11\% & 1,933 & 12,750 & 96.70\% & 697 & 76 & 1,123 & 139 & 33 & 3 & 10 & 0 & 0 & 531 & 620 & 494 \\
& \MTqlora$_{9.3M}$ & \textbf{21.20\%} & 1,761 $\downarrow$ & 12,411 $\downarrow$ & \cellcolor{green!20}98.9\% & \cellcolor{blue!20}710 & \cellcolor{blue!20}85 & \cellcolor{blue!20}1,185 & \cellcolor{green!20}129 & \cellcolor{blue!20}34 & \cellcolor{blue!20}4 & \cellcolor{green!20}9 & 0 & \cellcolor{blue!20}3 & \cellcolor{blue!20}541 & \cellcolor{green!20}591 & \cellcolor{blue!20}512 \\
& \MTqlora$_{15M}$ & 20.65\% & 1,665 $\downarrow$ & 12,209 $\downarrow$ & \cellcolor{green!20}98.9\% & \cellcolor{green!20}613 & \cellcolor{yellow!20}74 & \cellcolor{blue!20}1,186 & \cellcolor{blue!20}163 & \cellcolor{green!20}29 & \cellcolor{yellow!20}3 & \cellcolor{green!20}9 & 0 & \cellcolor{blue!20}2 & \cellcolor{blue!20}545 & \cellcolor{green!20}594 & \cellcolor{blue!20}559 \\
\midrule
\multirow{2}{*}{\textit{Qwen-1.5B}} 
& \MTqlora & 19.02\% & 1,490 & 10,313 & 96.20\% & 589 & 75 & 1,183 & 127 & 31 & 5 & 11 & 0 & 2 & 530 & 544 & 442 \\
& \MTqlora$_{15M}$ & \textbf{27.17\%} & 1,621 $\uparrow$ & 11,478 $\uparrow$ & \cellcolor{green!20}99.5\% & \cellcolor{blue!20}625 & \cellcolor{blue!20}80 & \cellcolor{blue!20}1,336 & \cellcolor{yellow!20}128 & \cellcolor{blue!20}32 & \cellcolor{green!20}3 & \cellcolor{yellow!20}11 & 0 & \cellcolor{blue!20}3 & \cellcolor{blue!20}557 & \cellcolor{blue!20}618 & \cellcolor{blue!20}551 \\
\midrule
\multirow{2}{*}{\textit{Qwen-3B}} 
& \MTqlora & 32.07\% & 1,580 & 10,920 & 98.40\% & 558 & 86 & 1,184 & 128 & 32 & 4 & 7 & 0 & 2 & 541 & 554 & 469 \\
& \MTqlora$_{9.3M}$ & \textbf{34.78\%} & 1,573 $\downarrow$ & 10,793 $\downarrow$ & \cellcolor{green!20}99.5\% & \cellcolor{blue!20}570 & \cellcolor{green!20}80 & \cellcolor{green!20}1,176 & \cellcolor{blue!20}136 & \cellcolor{blue!20}42 & \cellcolor{yellow!20}4 & \cellcolor{blue!20}13 & 0 & \cellcolor{blue!20}3 & \cellcolor{blue!20}556 & \cellcolor{blue!20}564 & \cellcolor{blue!20}482 \\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/ext-cg-py.tex <==
\begin{table}[h]
\centering
\scriptsize
\caption{Capacity-matched configurations for Python code generation on CoderEval. \MTqlora$_{9.3M}$ and \MTqlora$_{15M}$ denote parameter-matched variants. Bold indicates best Pass@1 within each model size.}
\label{tab:extended_codegen_python}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{lc|c|cccc|cccc|ccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Method}} & 
\multirow{2}{*}{\textbf{Pass@1}} & 
\multicolumn{4}{c|}{\textbf{Lizard}} & 
\multicolumn{4}{c|}{\textbf{Pylint}} &
\multicolumn{5}{c}{\textbf{SonarCloud}} \\
\cmidrule(lr){4-7} \cmidrule(lr){8-11} \cmidrule(l){12-16}
& & & \textbf{LoC} & \textbf{Tok} & \textbf{DR} & \textbf{CyC} & 
\textbf{Err} & \textbf{Warn} & \textbf{Conv} & \textbf{Ref} &
\textbf{Sec} & \textbf{Rel} & \textbf{Main} & \textbf{CyC} & \textbf{CoC} \\
\midrule
\multirow{3}{*}{\textit{Qwen-0.5B}} 
& \MTqlora & 15.79\% & 1,952 & 13,327 & 100\% & 812 & 251 & 1,593 & 642 & 56 & 2 & 7 & 90 & 568 & 634 \\
& \MTqlora$_{9.3M}$ & \textbf{16.84\%} & 2,371 $\uparrow$ & 15,652 $\uparrow$ & \cellcolor{blue!20}98.9\% & \cellcolor{blue!20}913 & \cellcolor{green!20}249 & \cellcolor{green!20}1,538 & \cellcolor{green!20}604 & \cellcolor{blue!20}63 & \cellcolor{green!20}1 & \cellcolor{green!20}5 & \cellcolor{green!20}89 & \cellcolor{green!20}493 & \cellcolor{green!20}534 \\
& \MTqlora$_{15M}$ & 14.74\% & 2,467 $\uparrow$ & 15,486 $\uparrow$ & \cellcolor{blue!20}98.4\% & \cellcolor{blue!20}975 & \cellcolor{green!20}233 & \cellcolor{green!20}1,483 & \cellcolor{green!20}606 & \cellcolor{green!20}53 & 3 & \cellcolor{blue!20}12 & \cellcolor{blue!20}94 & \cellcolor{blue!20}590 & \cellcolor{blue!20}657 \\
\midrule
\multirow{2}{*}{\textit{Qwen-1.5B}} 
& \MTqlora & 18.95\% & 2,296 & 14,531 & 100\% & 882 & 315 & 1,767 & 677 & 76 & 1 & 5 & 72 & 638 & 771 \\
& \MTqlora$_{15M}$ & \textbf{18.95\%} & 2,100 $\downarrow$ & 13,568 $\downarrow$ & \cellcolor{yellow!20}100\% & \cellcolor{green!20}784 & \cellcolor{green!20}301 & \cellcolor{green!20}1,665 & \cellcolor{green!20}672 & \cellcolor{green!20}66 & \cellcolor{blue!20}4 & \cellcolor{green!20}1 & \cellcolor{green!20}52 & \cellcolor{green!20}585 & \cellcolor{green!20}674 \\
\midrule
\multirow{2}{*}{\textit{Qwen-3B}} 
& \MTqlora & \textbf{21.05\%} & 1,759 & 11,773 & 100\% & 677 & 269 & 1,521 & 673 & 56 & 2 & 5 & 106 & 537 & 549 \\
& \MTqlora$_{9.3M}$ & 20.53\% & 1,845 $\uparrow$ & 11,519 $\downarrow$ & \cellcolor{yellow!20}100\% & \cellcolor{yellow!20}677 & \cellcolor{green!20}266 & \cellcolor{blue!20}1,550 & \cellcolor{blue!20}688 & \cellcolor{blue!20}59 & 2 & \cellcolor{green!20}1 & \cellcolor{green!20}83 & \cellcolor{blue!20}558 & \cellcolor{blue!20}633 \\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/ext-cs.tex <==
\begin{table}[h]
\centering
\scriptsize
\caption{Capacity-matched configurations for code summarization on CoderEval. \MTqlora$_{9.3M}$ and \MTqlora15M$_{15M}$ denote parameter-matched variants. SIDE applies to \java only. Bold indicates best value within each model size and language.}
\label{tab:extended_codesum}
\resizebox{0.75\textwidth}{!}{%
\begin{tabular}{c|c|c|cccccc}
\toprule
\textbf{Lang} & \textbf{Model} & \textbf{Method} & \textbf{BLEU} & \textbf{METEOR} & \textbf{Rouge-L} & \textbf{chrF} & \textbf{BERTScore} & \textbf{SIDE} \\
\midrule
\multirow{7}{*}{Java}
& \multirow{3}{*}{\textit{Qwen-0.5B}} 
& \MTqlora & \textbf{1.25\%} & 11.69\% & \textbf{25.60\%} & \textbf{15.71\%} & \textbf{59.28\%} & 90.44\% \\
& & \MTqlora$_{9.3M}$ & 1.18\% & \textbf{11.81\%} & 24.46\% & 15.06\% & 58.57\% & 90.75\% \\
& & \MTqlora$_{15M}$ & 1.11\% & 11.31\% & 24.74\% & 15.46\% & 58.58\% & \textbf{91.99\%} \\
\cmidrule{2-9}
& \multirow{2}{*}{\textit{Qwen-1.5B}} 
& \MTqlora & 1.28\% & 11.57\% & 24.58\% & 15.90\% & 58.94\% & \textbf{92.21\%} \\
& & \MTqlora$_{15M}$ & \textbf{1.5\%} & \textbf{12.23\%} & \textbf{26.37\%} & \textbf{17.04\%} & \textbf{59.55\%} & 91.06\% \\
\cmidrule{2-9}
& \multirow{2}{*}{\textit{Qwen-3B}} 
& \MTqlora & \textbf{1.51\%} & \textbf{12.11\%} & 25.60\% & \textbf{16.37\%} & 59.20\% & 91.58\% \\
& & \MTqlora$_{9.3M}$ & 1.33\% & 12.04\% & \textbf{26.5\%} & 16.2\% & \textbf{59.25\%} & \textbf{92.06\%} \\
\midrule
\multirow{7}{*}{Python}
& \multirow{3}{*}{\textit{Qwen-0.5B}} 
& \MTqlora & \textbf{9.90\%} & \textbf{18.54\%} & \textbf{31.09\%} & \textbf{26.88\%} & \textbf{66.96\%} & -- \\
& & \MTqlora$_{9.3M}$ & 7.55\% & 15.58\% & 27.97\% & 23.49\% & 65.15\% & -- \\
& & \MTqlora$_{15M}$ & 7.78\% & 17.22\% & 29.42\% & 25.17\% & 66.25\% & -- \\
\cmidrule{2-9}
& \multirow{2}{*}{\textit{Qwen-1.5B}} 
& \MTqlora & 12.60\% & 21.28\% & 34.44\% & 28.98\% & 67.78\% & -- \\
& & \MTqlora$_{15M}$ & \textbf{13.99\%} & \textbf{22.52\%} & \textbf{36.23\%} & \textbf{30.3\%} & \textbf{68.66\%} & -- \\
\cmidrule{2-9}
& \multirow{2}{*}{\textit{Qwen-3B}} 
& \MTqlora & 24.33\% & \textbf{32.88\%} & 45.35\% & 40.98\% & 72.85\% & -- \\
& & \MTqlora$_{9.3M}$ & \textbf{25.13\%} & 32.52\% & \textbf{47.52\%} & \textbf{41.03\%} & \textbf{74.35\%} & -- \\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/ext-ct-java-csharp.tex <==
\begin{table}[h]
\centering
\scriptsize
\caption{Capacity-matched configurations for C\#$rightarrow$Java code translation on CodeXGLUE. \MTqlora$_{9.3M}$ and \MTqlora$_{15M}$
 denote parameter-matched variants. Bold indicates best CodeBLEU within each model size.}
\label{tab:extended_codetrans_java2csharp}
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{lc|c|cccc|cc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Method}} & 
\multirow{2}{*}{\textbf{CodeBLEU}} & 
\multicolumn{4}{c|}{\textbf{Lizard}} & 
\multicolumn{2}{c}{\textbf{Roslyn}} \\
\cmidrule(lr){4-7} \cmidrule(l){8-9}
& & & \textbf{LoC} & \textbf{Tok} & \textbf{DR} & \textbf{CyC} & 
\textbf{Syntax Errors} & \textbf{Maintainability} \\
\midrule
\multirow{3}{*}{\textit{Qwen-0.5B}} 
& \MTqlora & 68.92\% & 6,218 & 39,509 & 98.7\% & 1,515 & 256 & 835 \\
& \MTqlora$_{9.3M}$ & 60.98\% & 6,397 $\uparrow$ & 41,092 $\uparrow$ & \cellcolor{yellow!20}99\% & \cellcolor{blue!20}1,542 & \cellcolor{green!20}11 & \cellcolor{blue!20}1,476 \\
& \MTqlora$_{15M}$ & \textbf{71.79\%} & 5,965 $\downarrow$ & 37,927 $\downarrow$ & \cellcolor{blue!20}95.2\% & \cellcolor{green!20}1,429 & \cellcolor{green!20}239 & \cellcolor{green!20}790 \\
\midrule
\multirow{2}{*}{\textit{Qwen-1.5B}} 
& \MTqlora & \textbf{73.08\%} & 6,369 & 40,516 & 98.5\% & 1,563 & 313 & 592 \\
& \MTqlora$_{15M}$ & 71.77\% & 6,428 $\uparrow$ & 40,991 $\uparrow$ & \cellcolor{green!20}99.5\% & \cellcolor{blue!20}1,584 & \cellcolor{green!20}245 & \cellcolor{blue!20}621 \\
\midrule
\multirow{2}{*}{\textit{Qwen-3B}} 
& \MTqlora & \textbf{62.88\%} & 5,890 & 37,716 & 93.6\% & 1,455 & 126 & 3,061 \\
& \MTqlora$_{9.3M}$ & 59.97\% & 6,128 $\uparrow$ & 39,358 $\uparrow$ & \cellcolor{green!20}95.1\% & \cellcolor{blue!20}1,484 & \cellcolor{green!20}70 & \cellcolor{green!20}2,708 \\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/ext-ct-sharp-java.tex <==
\begin{table}[h]
\centering
\scriptsize
\caption{Capacity-matched configurations for Java$rightarrow$C\# code translation on CodeXGLUE. \MTqlora$_{9.3M}$ and \MTqlora$_{15M}$
 denote parameter-matched variants. Bold indicates best CodeBLEU within each model size.}
\label{tab:extended_codetrans_csharp2java}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{lc|c|cccc|cccccc|ccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Method}} & 
\multirow{2}{*}{\textbf{CodeBLEU}} & 
\multicolumn{4}{c|}{\textbf{Lizard}} & 
\multicolumn{6}{c|}{\textbf{PMD}} &
\multicolumn{5}{c}{\textbf{SonarCloud}} \\
\cmidrule(lr){4-7} \cmidrule(lr){8-13} \cmidrule(l){14-18}
& & & \textbf{LoC} & \textbf{Tok} & \textbf{DR} & \textbf{CyC} & 
\textbf{Best Prac.} & \textbf{CS} & \textbf{Design} & \textbf{EP} & \textbf{MT} & \textbf{Perf.} &
\textbf{Sec} & \textbf{Rel} & \textbf{Main} & \textbf{CyC} & \textbf{CoC} \\
\midrule
\multirow{3}{*}{\textit{Qwen-0.5B}} 
& \MTqlora & \textbf{68.37\%} & 5,807 & 35,170 & 99.6\% & 1,594 & 400 & 3,953 & 234 & 54 & 12 & 140 & 0 & 13 & 1,056 & 1,401 & 654 \\
& \MTqlora$_{9.3M}$ & 51.14\% & 6,378 $\uparrow$ & 41,329 $\uparrow$ & \cellcolor{yellow!20}99.6\% & \cellcolor{blue!20}1,596 & \cellcolor{green!20}13 & \cellcolor{green!20}776 & \cellcolor{green!20}121 & \cellcolor{green!20}15 & \textit{N/A} & \textit{N/A} & 0 & \cellcolor{green!20}1 & \cellcolor{green!20}262 & \cellcolor{green!20}139 & \cellcolor{green!20}16 \\
& \MTqlora$_{15M}$ & 59.45\% & 6,123 $\uparrow$ & 39,027 $\uparrow$ & \cellcolor{blue!20}97.9\% & \cellcolor{green!20}1,568 & \cellcolor{green!20}173 & \cellcolor{green!20}2,858 & \cellcolor{green!20}181 & \cellcolor{green!20}46 & \cellcolor{green!20}10 & \cellcolor{green!20}56 & 0 & \cellcolor{blue!20}17 & \cellcolor{green!20}724 & \cellcolor{green!20}1,020 & \cellcolor{green!20}571 \\
\midrule
\multirow{2}{*}{\textit{Qwen-1.5B}} 
& \MTqlora & \textbf{70.72\%} & 5,745 & 35,074 & 99.6\% & 1,566 & 400 & 3,939 & 213 & 61 & 22 & 163 & 0 & 19 & 1,088 & 1,428 & 678 \\
& \MTqlora$_{15M}$ & 69.38\% & 5,896 $\uparrow$ & 36,430 $\uparrow$ & \cellcolor{green!20}99.7\% & \cellcolor{blue!20}1,670 & \cellcolor{blue!20}404 & \cellcolor{yellow!20}3,939 & \cellcolor{blue!20}223 & \cellcolor{blue!20}68 & \cellcolor{green!20}21 & \cellcolor{blue!20}169 & 0 & \cellcolor{blue!20}24 & \cellcolor{blue!20}1,089 & \cellcolor{blue!20}1,449 & \cellcolor{blue!20}703 \\
\midrule
\multirow{2}{*}{\textit{Qwen-3B}} 
& \MTqlora & \textbf{71.22\%} & 5,742 & 34,862 & 99.5\% & 1,612 & 37 & 1,072 & 45 & 11 & 5 & 1 & 0 & 0 & 278 & 322 & 157 \\
& \MTqlora$_{9.3M}$ & 47.43\% & 4,360 & 25,278 & 78.6\% & 1,188 & 137 & 6 & \textit{N/A} & \textit{N/A} & \textit{N/A} & \textit{N/A} & 0 & 0 & 37 & 29 & 6 \\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/stat-tables/rq1-stat-cg.tex <==
% % ==================== PYTHON TABLE ====================
% \begin{table*}[t!]
% 	\centering
% 	\caption{RQ1: Statistical comparison of ST-QLoRA vs MT-QLoRA for Python code generation. Significance assessed using McNemar Test for Pass@1 and Wilcoxon Signed-Rank Test for quality metrics. Effect size measured by Odds Ratio (OR) for Pass@1 and Cliff's Delta (d) for quality metrics (N: negligible, S: small, M: medium, L: large). All p-values are Holm-Bonferroni corrected.}
% 	\label{tab:rq1-stat-python}
% 	\scriptsize
% 	\resizebox{\linewidth}{!}{
% 		\begin{tabular}{>{\centering\arraybackslash}m{1.8cm} | rr | rr rr rr | rr rr rr rr | rr rr rr rr}
% 			\toprule
% 			& \multicolumn{2}{c|}{\bf Pass@1} & \multicolumn{6}{c|}{\bf Lizard} & \multicolumn{8}{c|}{\bf Pylint} & \multicolumn{8}{c}{\bf SonarCloud} \\
% 			\cmidrule(lr){2-3} \cmidrule(lr){4-9} \cmidrule(lr){10-17} \cmidrule(lr){18-25}
			
% 			\bf Model
% 			& \multicolumn{2}{c|}{}
% 			& \multicolumn{2}{c}{\bf LoC} & \multicolumn{2}{c}{\bf Tok} & \multicolumn{2}{c|}{\bf CyC}
% 			& \multicolumn{2}{c}{\bf Err} & \multicolumn{2}{c}{\bf Warn} & \multicolumn{2}{c}{\bf Conv} & \multicolumn{2}{c|}{\bf Ref}
% 			& \multicolumn{2}{c}{\bf Rel} & \multicolumn{2}{c}{\bf Main} & \multicolumn{2}{c}{\bf CyC} & \multicolumn{2}{c}{\bf CoC} \\
			
% 			& \bf p-value & \bf OR 
% 			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d 
% 			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d 
% 			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d \\
% 			\midrule
			
% 			Qwen-0.5B & 1.00 & 1.000 & 1.00 & 0.003 (N) & 1.00 & -0.016 (N) & 1.00 & -0.009 (N) & 0.54 & -0.047 (N) & 1.00 & -0.005 (N) & 1.00 & 0.000 (N) & 1.00 & -0.004 (N) & 0.50 & -0.021 (N) & 1.00 & -0.039 (N) & 1.00 & -0.017 (N) & 1.00 & -0.004 (N) \\
% 			\cmidrule(lr){1-25}
% 			Qwen-1.5B & 1.00 & 0.579 & 1.00 & -0.033 (N) & 1.00 & -0.006 (N) & 1.00 & -0.029 (N) & 1.00 & -0.008 (N) & 1.00 & -0.045 (N) & 1.00 & -0.020 (N) & 1.00 & -0.015 (N) & 1.00 & 0.000 (N) & 0.16 & -0.074 (N) & 1.00 & -0.017 (N) & 0.94 & -0.051 (N) \\
% 			\cmidrule(lr){1-25}
% 			Qwen-3B   & 1.00 & 0.846 & 1.00 & 0.031 (N) & 1.00 & -0.015 (N) & 1.00 & -0.007 (N) & 0.16 & -0.061 (N) & 1.00 & 0.043 (N) & 1.00 & -0.036 (N) & 1.00 & -0.020 (N) & 0.25 & -0.026 (N) & 1.00 & 0.028 (N) & 1.00 & 0.012 (N) & 1.00 & 0.028 (N) \\
			
% 			\bottomrule
% 		\end{tabular}
% 	}
% 	\vspace{-0.2cm}
% \end{table*}

% % ==================== JAVA TABLE ====================
% \begin{table*}[t!]
% 	\centering
% 	\caption{RQ1: Statistical comparison of ST-QLoRA vs MT-QLoRA for Java code generation. Significance assessed using McNemar Test for Pass@1 and Wilcoxon Signed-Rank Test for quality metrics. Effect size measured by Odds Ratio (OR) for Pass@1 and Cliff's Delta (d) for quality metrics (N: negligible, S: small, M: medium, L: large). All p-values are Holm-Bonferroni corrected.}
% 	\label{tab:rq1-stat-java}
% 	\scriptsize
% 	\resizebox{\linewidth}{!}{
% 		\begin{tabular}{>{\centering\arraybackslash}m{1.8cm} | rr | rr rr rr | rr rr rr rr rr rr | rr rr rr rr}
% 			\toprule
% 			& \multicolumn{2}{c|}{\bf Pass@1} & \multicolumn{6}{c|}{\bf Lizard} & \multicolumn{12}{c|}{\bf PMD} & \multicolumn{8}{c}{\bf SonarCloud} \\
% 			\cmidrule(lr){2-3} \cmidrule(lr){4-9} \cmidrule(lr){10-21} \cmidrule(lr){22-29}
			
% 			\bf Model
% 			& \multicolumn{2}{c|}{}
% 			& \multicolumn{2}{c}{\bf LoC} & \multicolumn{2}{c}{\bf Tok} & \multicolumn{2}{c|}{\bf CyC}
% 			& \multicolumn{2}{c}{\bf BP} & \multicolumn{2}{c}{\bf CS} & \multicolumn{2}{c}{\bf Des} & \multicolumn{2}{c}{\bf EP} & \multicolumn{2}{c}{\bf MT} & \multicolumn{2}{c|}{\bf Perf}
% 			& \multicolumn{2}{c}{\bf Rel} & \multicolumn{2}{c}{\bf Main} & \multicolumn{2}{c}{\bf CyC} & \multicolumn{2}{c}{\bf CoC} \\
			
% 			& \bf p-value & \bf OR 
% 			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d 
% 			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d 
% 			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d \\
% 			\midrule
			
% 			Qwen-0.5B & 1.00 & 1.207 & 0.21 & -0.096 (N) & 1.00 & -0.003 (N) & 1.00 & -0.026 (N) & 1.00 & -0.009 (N) & 1.00 & 0.057 (N) & 1.00 & -0.019 (N) & 1.00 & -0.006 (N) & 1.00 & 0.000 (N) & 1.00 & 0.012 (N) & 1.00 & -0.005 (N) & 1.00 & -0.005 (N) & 1.00 & 0.000 (N) & 1.00 & -0.015 (N) \\
% 			\cmidrule(lr){1-29}
% 			Qwen-1.5B & 0.31 & 2.143 & 0.79 & 0.097 (N) & 0.79 & 0.100 (N) & 0.79 & 0.118 (N) & 1.00 & 0.027 (N) & 1.00 & 0.054 (N) & 1.00 & -0.017 (N) & 1.00 & 0.022 (N) & 1.00 & -0.005 (N) & 1.00 & 0.005 (N) & 1.00 & 0.000 (N) & 1.00 & 0.021 (N) & 1.00 & 0.101 (N) & 1.00 & 0.111 (N) \\
% 			\cmidrule(lr){1-29}
% 			Qwen-3B   & 1.00 & 0.704 & 1.00 & -0.016 (N) & 1.00 & 0.019 (N) & 1.00 & 0.049 (N) & 1.00 & -0.009 (N) & 1.00 & -0.004 (N) & 1.00 & 0.006 (N) & 1.00 & -0.013 (N) & 1.00 & -0.005 (N) & 1.00 & 0.022 (N) & 1.00 & 0.000 (N) & 1.00 & 0.034 (N) & 1.00 & 0.050 (N) & 1.00 & 0.030 (N) \\
			
% 			\bottomrule
% 		\end{tabular}
% 	}
% 	\vspace{-0.2cm}
% \end{table*}

% ==================== COMBINED RQ1 TABLE ====================
\begin{table*}[h]
	\centering
	\caption{Statistical comparison of ST-QLoRA vs MT-QLoRA for Python and Java code generation. Significance assessed using McNemar Test for Pass@1 and Wilcoxon Signed-Rank Test for quality metrics. Effect size measured by Odds Ratio (OR) for Pass@1 and Cliff's Delta (d) for quality metrics (N: negligible, S: small, M: medium, L: large). All p-values are Holm-Bonferroni corrected.}
	\label{tab:rq1-stat}
	%\scriptsize
    \small
	
	% ===== Python =====
	\resizebox{\linewidth}{!}{
		\begin{tabular}{>{\centering\arraybackslash}m{1.8cm} | rr | rr rr rr | rr rr rr rr | rr rr rr rr}
			\toprule
			\multicolumn{25}{c}{\textbf{Python}} \\
			\midrule
			& \multicolumn{2}{c|}{\bf Pass@1} & \multicolumn{6}{c|}{\bf Lizard} & \multicolumn{8}{c|}{\bf Pylint} & \multicolumn{8}{c}{\bf SonarCloud} \\
			\cmidrule(lr){2-3} \cmidrule(lr){4-9} \cmidrule(lr){10-17} \cmidrule(lr){18-25}
			
			\bf Model
			& \multicolumn{2}{c|}{}
			& \multicolumn{2}{c}{\bf LoC} & \multicolumn{2}{c}{\bf Tok} & \multicolumn{2}{c|}{\bf CyC}
			& \multicolumn{2}{c}{\bf Err} & \multicolumn{2}{c}{\bf Warn} & \multicolumn{2}{c}{\bf Conv} & \multicolumn{2}{c|}{\bf Ref}
			& \multicolumn{2}{c}{\bf Rel} & \multicolumn{2}{c}{\bf Main} & \multicolumn{2}{c}{\bf CyC} & \multicolumn{2}{c}{\bf CoC} \\
			
			& \bf p-value & \bf OR 
			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d 
			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d 
			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d \\
			\midrule
			
			Qwen-0.5B & 1.00 & 1.000 & 1.00 & 0.003 (N) & 1.00 & -0.016 (N) & 1.00 & -0.009 (N) & 0.54 & -0.047 (N) & 1.00 & -0.005 (N) & 1.00 & 0.000 (N) & 1.00 & -0.004 (N) & 0.50 & -0.021 (N) & 1.00 & -0.039 (N) & 1.00 & -0.017 (N) & 1.00 & -0.004 (N) \\
			Qwen-1.5B & 1.00 & 0.579 & 1.00 & -0.033 (N) & 1.00 & -0.006 (N) & 1.00 & -0.029 (N) & 1.00 & -0.008 (N) & 1.00 & -0.045 (N) & 1.00 & -0.020 (N) & 1.00 & -0.015 (N) & 1.00 & 0.000 (N) & 0.16 & -0.074 (N) & 1.00 & -0.017 (N) & 0.94 & -0.051 (N) \\
			Qwen-3B   & 1.00 & 0.846 & 1.00 & 0.031 (N) & 1.00 & -0.015 (N) & 1.00 & -0.007 (N) & 0.16 & -0.061 (N) & 1.00 & 0.043 (N) & 1.00 & -0.036 (N) & 1.00 & -0.020 (N) & 0.25 & -0.026 (N) & 1.00 & 0.028 (N) & 1.00 & 0.012 (N) & 1.00 & 0.028 (N) \\
			
			\bottomrule
		\end{tabular}
	}
	
	\vspace{0.3cm}
	
	% ===== Java =====
	\resizebox{\linewidth}{!}{
		\begin{tabular}{>{\centering\arraybackslash}m{1.8cm} | rr | rr rr rr | rr rr rr rr rr rr | rr rr rr rr}
			\toprule
			\multicolumn{29}{c}{\textbf{Java}} \\
			\midrule
			& \multicolumn{2}{c|}{\bf Pass@1} & \multicolumn{6}{c|}{\bf Lizard} & \multicolumn{12}{c|}{\bf PMD} & \multicolumn{8}{c}{\bf SonarCloud} \\
			\cmidrule(lr){2-3} \cmidrule(lr){4-9} \cmidrule(lr){10-21} \cmidrule(lr){22-29}
			
			\bf Model
			& \multicolumn{2}{c|}{}
			& \multicolumn{2}{c}{\bf LoC} & \multicolumn{2}{c}{\bf Tok} & \multicolumn{2}{c|}{\bf CyC}
			& \multicolumn{2}{c}{\bf BP} & \multicolumn{2}{c}{\bf CS} & \multicolumn{2}{c}{\bf Des} & \multicolumn{2}{c}{\bf EP} & \multicolumn{2}{c}{\bf MT} & \multicolumn{2}{c|}{\bf Perf}
			& \multicolumn{2}{c}{\bf Rel} & \multicolumn{2}{c}{\bf Main} & \multicolumn{2}{c}{\bf CyC} & \multicolumn{2}{c}{\bf CoC} \\
			
			& \bf p-value & \bf OR 
			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d 
			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d 
			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d \\
			\midrule
			
			Qwen-0.5B & 1.00 & 1.207 & 0.21 & -0.096 (N) & 1.00 & -0.003 (N) & 1.00 & -0.026 (N) & 1.00 & -0.009 (N) & 1.00 & 0.057 (N) & 1.00 & -0.019 (N) & 1.00 & -0.006 (N) & 1.00 & 0.000 (N) & 1.00 & 0.012 (N) & 1.00 & -0.005 (N) & 1.00 & -0.005 (N) & 1.00 & 0.000 (N) & 1.00 & -0.015 (N) \\
			Qwen-1.5B & 0.31 & 2.143 & 0.79 & 0.097 (N) & 0.79 & 0.100 (N) & 0.79 & 0.118 (N) & 1.00 & 0.027 (N) & 1.00 & 0.054 (N) & 1.00 & -0.017 (N) & 1.00 & 0.022 (N) & 1.00 & -0.005 (N) & 1.00 & 0.005 (N) & 1.00 & 0.000 (N) & 1.00 & 0.021 (N) & 1.00 & 0.101 (N) & 1.00 & 0.111 (N) \\
			Qwen-3B   & 1.00 & 0.704 & 1.00 & -0.016 (N) & 1.00 & 0.019 (N) & 1.00 & 0.049 (N) & 1.00 & -0.009 (N) & 1.00 & -0.004 (N) & 1.00 & 0.006 (N) & 1.00 & -0.013 (N) & 1.00 & -0.005 (N) & 1.00 & 0.022 (N) & 1.00 & 0.000 (N) & 1.00 & 0.034 (N) & 1.00 & 0.050 (N) & 1.00 & 0.030 (N) \\
			
			\bottomrule
		\end{tabular}
	}
	\vspace{-0.2cm}
\end{table*}

% % ==================== COMBINED RQ1 TABLE ====================
% \begin{table*}[h]
% 	\centering
% 	\caption{Statistical comparison of ST-QLoRA vs MT-QLoRA for Python and Java code generation. Significance assessed using McNemar Test for Pass@1 and Wilcoxon Signed-Rank Test for quality metrics. Effect size measured by Odds Ratio (OR) for Pass@1. All p-values are Holm-Bonferroni corrected.}
% 	\label{tab:rq1-stat}
% 	%\scriptsize
%     \small
	
% 	% ===== Python =====
% 	\resizebox{\linewidth}{!}{
% 		\begin{tabular}{>{\centering\arraybackslash}m{1.8cm} | r | r r r | r r r r | r r r r}
% 			\toprule
% 			\multicolumn{13}{c}{\textbf{Python}} \\
% 			\midrule
% 			& \multicolumn{1}{c|}{\bf Pass@1} & \multicolumn{3}{c|}{\bf Lizard} & \multicolumn{4}{c|}{\bf Pylint} & \multicolumn{4}{c}{\bf SonarCloud} \\
% 			\cmidrule(lr){2-2} \cmidrule(lr){3-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
			
% 			\bf Model
% 			& \multicolumn{1}{c|}{}
% 			& \multicolumn{1}{c}{\bf LoC} & \multicolumn{1}{c}{\bf Tok} & \multicolumn{1}{c|}{\bf CyC}
% 			& \multicolumn{1}{c}{\bf Err} & \multicolumn{1}{c}{\bf Warn} & \multicolumn{1}{c}{\bf Conv} & \multicolumn{1}{c|}{\bf Ref}
% 			& \multicolumn{1}{c}{\bf Rel} & \multicolumn{1}{c}{\bf Main} & \multicolumn{1}{c}{\bf CyC} & \multicolumn{1}{c}{\bf CoC} \\
			
% 			& \bf OR 
% 			& \bf p-value & \bf p-value & \bf p-value 
% 			& \bf p-value & \bf p-value & \bf p-value & \bf p-value 
% 			& \bf p-value & \bf p-value & \bf p-value & \bf p-value \\
% 			\midrule
			
% 			Qwen-0.5B & 1.000 & 1.00 & 1.00 & 1.00 & 0.54 & 1.00 & 1.00 & 1.00 & 0.50 & 1.00 & 1.00 & 1.00 \\
% 			Qwen-1.5B & 0.579 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 0.16 & 1.00 & 0.94 \\
% 			Qwen-3B   & 0.846 & 1.00 & 1.00 & 1.00 & 0.16 & 1.00 & 1.00 & 1.00 & 0.25 & 1.00 & 1.00 & 1.00 \\
			
% 			\bottomrule
% 		\end{tabular}
% 	}
	
% 	\vspace{0.3cm}
	
% 	% ===== Java =====
% 	\resizebox{\linewidth}{!}{
% 		\begin{tabular}{>{\centering\arraybackslash}m{1.8cm} | r | r r r | r r r r r r | r r r r}
% 			\toprule
% 			\multicolumn{15}{c}{\textbf{Java}} \\
% 			\midrule
% 			& \multicolumn{1}{c|}{\bf Pass@1} & \multicolumn{3}{c|}{\bf Lizard} & \multicolumn{6}{c|}{\bf PMD} & \multicolumn{4}{c}{\bf SonarCloud} \\
% 			\cmidrule(lr){2-2} \cmidrule(lr){3-5} \cmidrule(lr){6-11} \cmidrule(lr){12-15}
			
% 			\bf Model
% 			& \multicolumn{1}{c|}{}
% 			& \multicolumn{1}{c}{\bf LoC} & \multicolumn{1}{c}{\bf Tok} & \multicolumn{1}{c|}{\bf CyC}
% 			& \multicolumn{1}{c}{\bf BP} & \multicolumn{1}{c}{\bf CS} & \multicolumn{1}{c}{\bf Des} & \multicolumn{1}{c}{\bf EP} & \multicolumn{1}{c}{\bf MT} & \multicolumn{1}{c|}{\bf Perf}
% 			& \multicolumn{1}{c}{\bf Rel} & \multicolumn{1}{c}{\bf Main} & \multicolumn{1}{c}{\bf CyC} & \multicolumn{1}{c}{\bf CoC} \\
			
% 			& \bf OR 
% 			& \bf p-value & \bf p-value & \bf p-value 
% 			& \bf p-value & \bf p-value & \bf p-value & \bf p-value & \bf p-value & \bf p-value 
% 			& \bf p-value & \bf p-value & \bf p-value & \bf p-value \\
% 			\midrule
			
% 			Qwen-0.5B & 1.207 & 0.21 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
% 			Qwen-1.5B & 2.143 & 0.79 & 0.79 & 0.79 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
% 			Qwen-3B   & 0.704 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
			
% 			\bottomrule
% 		\end{tabular}
% 	}
% 	\vspace{-0.2cm}
% \end{table*}

==> tables/stat-tables/rq1-stat-cs-llm-judge.tex <==
% ==================== COMBINED RQ1 CODE SUMMARIZATION QUALITY TABLE ====================
\begin{table*}[t!]
	\centering
	\caption{RQ1: Statistical comparison of ST-QLoRA vs MT-QLoRA for code summarization quality (LLM Judge). Significance assessed using Wilcoxon Signed-Rank Test. Effect size measured by Cliff's Delta (d) (N: negligible, S: small, M: medium, L: large). All p-values are Holm-Bonferroni corrected.}
	\label{tab:rq1-stat-summarization-quality}
	\scriptsize
	
	% ===== Python =====
	\resizebox{0.7\linewidth}{!}{
		\begin{tabular}{>{\centering\arraybackslash}m{1.8cm} | rr rr rr}
			\toprule
			\multicolumn{7}{c}{\textbf{Python}} \\
			\midrule
			\bf Model
			& \multicolumn{2}{c}{\bf CA} & \multicolumn{2}{c}{\bf Conciseness} & \multicolumn{2}{c}{\bf Fluency} \\
			
			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d \\
			\midrule
			
			Qwen-0.5B & 0.10 & 0.089 (N) & 0.45 & 0.013 (N) & 0.20 & 0.070 (N) \\
			Qwen-1.5B & 0.67 & 0.012 (N) & 0.61 & -0.047 (N) & 0.94 & 0.004 (N) \\
			Qwen-3B   & 0.39 & -0.099 (N) & 1.00 & 0.054 (N) & 1.00 & -0.012 (N) \\
			
			\bottomrule
		\end{tabular}
	}
	
	\vspace{0.3cm}
	
	% ===== Java =====
	\resizebox{0.7\linewidth}{!}{
		\begin{tabular}{>{\centering\arraybackslash}m{1.8cm} | rr rr rr}
			\toprule
			\multicolumn{7}{c}{\textbf{Java}} \\
			\midrule
			\bf Model
			& \multicolumn{2}{c}{\bf CA} & \multicolumn{2}{c}{\bf Conciseness} & \multicolumn{2}{c}{\bf Fluency} \\
			
			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d \\
			\midrule
			
			Qwen-0.5B & 1.00 & 0.006 (N) & 1.00 & 0.001 (N) & 1.00 & -0.014 (N) \\
			Qwen-1.5B & 0.21 & 0.092 (N) & 0.94 & 0.000 (N) & 0.84 & 0.041 (N) \\
			Qwen-3B   & 1.00 & 0.003 (N) & 1.00 & 0.011 (N) & 1.00 & -0.003 (N) \\
			
			\bottomrule
		\end{tabular}
	}
	\vspace{-0.2cm}
\end{table*}

==> tables/stat-tables/rq1-stat-cs.tex <==
% ==================== COMBINED RQ1 CODE SUMMARIZATION TABLE ====================
\begin{table*}[h]
	\centering
	\caption{Statistical comparison of ST-QLoRA vs MT-QLoRA for code summarization. Significance assessed using Wilcoxon Signed-Rank Test. Effect size measured by Cliff's Delta (d) (N: negligible, S: small, M: medium, L: large). All p-values are Holm-Bonferroni corrected.}
	\label{tab:rq1-stat-summarization}
	%\scriptsize
    \small
	
	% ===== Java =====
	\resizebox{\linewidth}{!}{
		\begin{tabular}{>{\centering\arraybackslash}m{1.8cm} | rr rr rr rr rr rr}
			\toprule
			\multicolumn{13}{c}{\textbf{Java}} \\
			\midrule
			\bf Model
			& \multicolumn{2}{c}{\bf BLEU} & \multicolumn{2}{c}{\bf METEOR} & \multicolumn{2}{c}{\bf Rouge-L} & \multicolumn{2}{c}{\bf chrF} & \multicolumn{2}{c}{\bf BERTScore} & \multicolumn{2}{c}{\bf SIDE} \\
			
			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d \\
			\midrule
			
			Qwen-0.5B & 1.00 & 0.011 (N) & 1.00 & -0.010 (N) & 1.00 & -0.061 (N) & 1.00 & 0.026 (N) & 1.00 & 0.002 (N) & 1.00 & 0.045 (N) \\
			Qwen-1.5B & 0.33 & 0.025 (N) & 0.33 & 0.047 (N) & 0.33 & 0.071 (N) & 0.33 & 0.049 (N) & 0.33 & 0.053 (N) & 0.51 & -0.006 (N) \\
			Qwen-3B   & 0.16 & 0.061 (N) & 0.50 & 0.037 (N) & 0.50 & 0.030 (N) & 0.20 & 0.033 (N) & 0.50 & 0.030 (N) & 0.50 & 0.035 (N) \\
			
			\bottomrule
		\end{tabular}
	}
	
	\vspace{0.3cm}
	
	% ===== Python =====
	\resizebox{\linewidth}{!}{
		\begin{tabular}{>{\centering\arraybackslash}m{1.8cm} | rr rr rr rr rr}
			\toprule
			\multicolumn{11}{c}{\textbf{Python}} \\
			\midrule
			\bf Model
			& \multicolumn{2}{c}{\bf BLEU} & \multicolumn{2}{c}{\bf METEOR} & \multicolumn{2}{c}{\bf Rouge-L} & \multicolumn{2}{c}{\bf chrF} & \multicolumn{2}{c}{\bf BERTScore} \\
			
			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d \\
			\midrule
			
			Qwen-0.5B & 0.08 & -0.076 (N) & 0.08 & -0.055 (N) & 0.04 & -0.114 (N) & 0.06 & -0.099 (N) & 0.06 & -0.103 (N) \\
			Qwen-1.5B & $<$0.01 & -0.093 (N) & $<$0.01 & -0.106 (N) & $<$0.01 & -0.108 (N) & $<$0.01 & -0.105 (N) & $<$0.01 & -0.129 (N) \\
			Qwen-3B   & $<$0.01 & -0.196 (S) & $<$0.01 & -0.194 (S) & $<$0.01 & -0.188 (S) & $<$0.01 & -0.193 (S) & $<$0.01 & -0.170 (S) \\
			
			\bottomrule
		\end{tabular}
	}
	\vspace{-0.2cm}
\end{table*}

% % ==================== COMBINED RQ1 CODE SUMMARIZATION TABLE ====================
% \begin{table*}[h]
% 	\centering
% 	\caption{Statistical comparison of ST-QLoRA vs MT-QLoRA for code summarization. Significance assessed using Wilcoxon Signed-Rank Test. All p-values are Holm-Bonferroni corrected.}
% 	\label{tab:rq1-stat-summarization}
% 	%\scriptsize
%     \small
	
% 	% ===== Java =====
% 	\resizebox{\linewidth}{!}{
% 		\begin{tabular}{>{\centering\arraybackslash}m{1.8cm} | r r r r r r}
% 			\toprule
% 			\multicolumn{7}{c}{\textbf{Java}} \\
% 			\midrule
% 			\bf Model
% 			& \multicolumn{1}{c}{\bf BLEU} & \multicolumn{1}{c}{\bf METEOR} & \multicolumn{1}{c}{\bf Rouge-L} & \multicolumn{1}{c}{\bf chrF} & \multicolumn{1}{c}{\bf BERTScore} & \multicolumn{1}{c}{\bf SIDE} \\
			
% 			& \bf p-value & \bf p-value & \bf p-value & \bf p-value & \bf p-value & \bf p-value \\
% 			\midrule
			
% 			Qwen-0.5B & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
% 			Qwen-1.5B & 0.33 & 0.33 & 0.33 & 0.33 & 0.33 & 0.51 \\
% 			Qwen-3B   & 0.16 & 0.50 & 0.50 & 0.20 & 0.50 & 0.50 \\
			
% 			\bottomrule
% 		\end{tabular}
% 	}
	
% 	\vspace{0.3cm}
	
% 	% ===== Python =====
% 	\resizebox{\linewidth}{!}{
% 		\begin{tabular}{>{\centering\arraybackslash}m{1.8cm} | r r r r r}
% 			\toprule
% 			\multicolumn{6}{c}{\textbf{Python}} \\
% 			\midrule
% 			\bf Model
% 			& \multicolumn{1}{c}{\bf BLEU} & \multicolumn{1}{c}{\bf METEOR} & \multicolumn{1}{c}{\bf Rouge-L} & \multicolumn{1}{c}{\bf chrF} & \multicolumn{1}{c}{\bf BERTScore} \\
			
% 			& \bf p-value & \bf p-value & \bf p-value & \bf p-value & \bf p-value \\
% 			\midrule
			
% 			Qwen-0.5B & 0.08 & 0.08 & 0.04 & 0.06 & 0.06 \\
% 			Qwen-1.5B & $<$0.01 & $<$0.01 & $<$0.01 & $<$0.01 & $<$0.01 \\
% 			Qwen-3B   & $<$0.01 & $<$0.01 & $<$0.01 & $<$0.01 & $<$0.01 \\
			
% 			\bottomrule
% 		\end{tabular}
% 	}
% 	\vspace{-0.2cm}
% \end{table*}

==> tables/stat-tables/rq1-stat-ct.tex <==
% ==================== COMBINED RQ1 CODE TRANSLATION TABLE ====================
\begin{table*}[h]
	\centering
	\caption{Statistical comparison of ST-QLoRA vs MT-QLoRA for code translation. Significance assessed using Wilcoxon Signed-Rank Test. Effect size measured by Cliff's Delta (d) (N: negligible, S: small, M: medium, L: large). All p-values are Holm-Bonferroni corrected.}
	\label{tab:rq1-stat-translation}
	%\scriptsize
    \small
	
	% ===== Java to C# =====
	\resizebox{\linewidth}{!}{
		\begin{tabular}{>{\centering\arraybackslash}m{1.8cm} | rr | rr rr rr | rr rr}
			\toprule
			\multicolumn{13}{c}{\textbf{Java to C\#}} \\
			\midrule
			& \multicolumn{2}{c|}{\bf CodeBLEU} & \multicolumn{6}{c|}{\bf Lizard} & \multicolumn{4}{c}{\bf Roslyn} \\
			\cmidrule(lr){2-3} \cmidrule(lr){4-9} \cmidrule(lr){10-13}
			
			\bf Model
			& \multicolumn{2}{c|}{}
			& \multicolumn{2}{c}{\bf LoC} & \multicolumn{2}{c}{\bf Tok} & \multicolumn{2}{c|}{\bf CyC}
			& \multicolumn{2}{c}{\bf Syntax} & \multicolumn{2}{c}{\bf Main} \\
			
			& \bf p-value & \bf d 
			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d 
			& \bf p-value & \bf d & \bf p-value & \bf d \\
			\midrule
			
			Qwen-0.5B & $<$0.01 & 0.124 (N) & 1.00 & 0.008 (N) & 0.38 & 0.015 (N) & 1.00 & 0.003 (N) & 0.01 & 0.024 (N) & 1.00 & -0.004 (N) \\
			Qwen-1.5B & $<$0.01 & 0.045 (N) & 1.00 & 0.005 (N) & 1.00 & 0.010 (N) & 1.00 & -0.008 (N) & 1.00 & -0.010 (N) & $<$0.01 & 0.034 (N) \\
			Qwen-3B   & 0.03 & 0.054 (N) & $<$0.01 & 0.040 (N) & $<$0.01 & 0.046 (N) & 0.02 & 0.040 (N) & $<$0.01 & -0.048 (N) & $<$0.01 & -0.180 (S) \\
			
			\bottomrule
		\end{tabular}
	}
	
	\vspace{0.3cm}
	
	% ===== C# to Java =====
	\resizebox{\linewidth}{!}{
		\begin{tabular}{>{\centering\arraybackslash}m{1.8cm} | rr | rr rr rr | rr rr rr rr rr rr | rr rr rr rr}
			\toprule
			\multicolumn{29}{c}{\textbf{C\# to Java}} \\
			\midrule
			& \multicolumn{2}{c|}{\bf CodeBLEU} & \multicolumn{6}{c|}{\bf Lizard} & \multicolumn{12}{c|}{\bf PMD} & \multicolumn{8}{c}{\bf SonarCloud} \\
			\cmidrule(lr){2-3} \cmidrule(lr){4-9} \cmidrule(lr){10-21} \cmidrule(lr){22-29}
			
			\bf Model
			& \multicolumn{2}{c|}{}
			& \multicolumn{2}{c}{\bf LoC} & \multicolumn{2}{c}{\bf Tok} & \multicolumn{2}{c|}{\bf CyC}
			& \multicolumn{2}{c}{\bf BP} & \multicolumn{2}{c}{\bf CS} & \multicolumn{2}{c}{\bf Des} & \multicolumn{2}{c}{\bf EP} & \multicolumn{2}{c}{\bf MT} & \multicolumn{2}{c|}{\bf Perf}
			& \multicolumn{2}{c}{\bf Rel} & \multicolumn{2}{c}{\bf Main} & \multicolumn{2}{c}{\bf CyC} & \multicolumn{2}{c}{\bf CoC} \\
			
			& \bf p-value & \bf d 
			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d 
			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d 
			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d \\
			\midrule
			
			Qwen-0.5B & $<$0.01 & 0.132 (N) & 1.00 & -0.027 (N) & 1.00 & -0.024 (N) & 1.00 & -0.003 (N) & 1.00 & -0.009 (N) & 1.00 & 0.057 (N) & 1.00 & -0.019 (N) & 1.00 & -0.006 (N) & 1.00 & 0.000 (N) & 1.00 & 0.012 (N) & 1.00 & 0.007 (N) & 1.00 & 0.023 (N) & 1.00 & 0.022 (N) & 1.00 & -0.002 (N) \\
			Qwen-1.5B & 1.00 & -0.013 (N) & 1.00 & 0.000 (N) & 0.77 & 0.005 (N) & 0.77 & 0.010 (N) & 1.00 & 0.027 (N) & 1.00 & 0.054 (N) & 1.00 & -0.017 (N) & 1.00 & 0.022 (N) & 1.00 & -0.005 (N) & 1.00 & 0.005 (N) & 0.46 & -0.004 (N) & $<$0.01 & -0.052 (N) & 0.04 & -0.044 (N) & 1.00 & 0.000 (N) \\
			Qwen-3B   & 0.06 & -0.041 (N) & 1.00 & -0.007 (N) & 1.00 & -0.004 (N) & 1.00 & -0.006 (N) & 1.00 & -0.009 (N) & 1.00 & -0.004 (N) & 1.00 & 0.006 (N) & 1.00 & -0.013 (N) & 1.00 & -0.005 (N) & 1.00 & 0.022 (N) & 1.00 & -0.001 (N) & $<$0.01 & 0.034 (N) & 0.79 & 0.026 (N) & 1.00 & 0.016 (N) \\
			
			\bottomrule
		\end{tabular}
	}
	\vspace{-0.2cm}
\end{table*}

% % ==================== COMBINED RQ1 CODE TRANSLATION TABLE ====================
% \begin{table*}[h]
% 	\centering
% 	\caption{Statistical comparison of ST-QLoRA vs MT-QLoRA for code translation. Significance assessed using Wilcoxon Signed-Rank Test. All p-values are Holm-Bonferroni corrected.}
% 	\label{tab:rq1-stat-translation}
% 	%\scriptsize
%     \small
	
% 	% ===== Java to C# =====
% 	\resizebox{\linewidth}{!}{
% 		\begin{tabular}{>{\centering\arraybackslash}m{1.8cm} | r | r r r | r r}
% 			\toprule
% 			\multicolumn{7}{c}{\textbf{Java to C\#}} \\
% 			\midrule
% 			& \multicolumn{1}{c|}{\bf CodeBLEU} & \multicolumn{3}{c|}{\bf Lizard} & \multicolumn{2}{c}{\bf Roslyn} \\
% 			\cmidrule(lr){2-2} \cmidrule(lr){3-5} \cmidrule(lr){6-7}
			
% 			\bf Model
% 			& \multicolumn{1}{c|}{}
% 			& \multicolumn{1}{c}{\bf LoC} & \multicolumn{1}{c}{\bf Tok} & \multicolumn{1}{c|}{\bf CyC}
% 			& \multicolumn{1}{c}{\bf Syntax} & \multicolumn{1}{c}{\bf Main} \\
			
% 			& \bf p-value
% 			& \bf p-value & \bf p-value & \bf p-value
% 			& \bf p-value & \bf p-value \\
% 			\midrule
			
% 			Qwen-0.5B & $<$0.01 & 1.00 & 0.38 & 1.00 & 0.01 & 1.00 \\
% 			Qwen-1.5B & $<$0.01 & 1.00 & 1.00 & 1.00 & 1.00 & $<$0.01 \\
% 			Qwen-3B   & 0.03 & $<$0.01 & $<$0.01 & 0.02 & $<$0.01 & $<$0.01 \\
			
% 			\bottomrule
% 		\end{tabular}
% 	}
	
% 	\vspace{0.3cm}
	
% 	% ===== C# to Java =====
% 	\resizebox{\linewidth}{!}{
% 		\begin{tabular}{>{\centering\arraybackslash}m{1.8cm} | r | r r r | r r r r r r | r r r r}
% 			\toprule
% 			\multicolumn{15}{c}{\textbf{C\# to Java}} \\
% 			\midrule
% 			& \multicolumn{1}{c|}{\bf CodeBLEU} & \multicolumn{3}{c|}{\bf Lizard} & \multicolumn{6}{c|}{\bf PMD} & \multicolumn{4}{c}{\bf SonarCloud} \\
% 			\cmidrule(lr){2-2} \cmidrule(lr){3-5} \cmidrule(lr){6-11} \cmidrule(lr){12-15}
			
% 			\bf Model
% 			& \multicolumn{1}{c|}{}
% 			& \multicolumn{1}{c}{\bf LoC} & \multicolumn{1}{c}{\bf Tok} & \multicolumn{1}{c|}{\bf CyC}
% 			& \multicolumn{1}{c}{\bf BP} & \multicolumn{1}{c}{\bf CS} & \multicolumn{1}{c}{\bf Des} & \multicolumn{1}{c}{\bf EP} & \multicolumn{1}{c}{\bf MT} & \multicolumn{1}{c|}{\bf Perf}
% 			& \multicolumn{1}{c}{\bf Rel} & \multicolumn{1}{c}{\bf Main} & \multicolumn{1}{c}{\bf CyC} & \multicolumn{1}{c}{\bf CoC} \\
			
% 			& \bf p-value
% 			& \bf p-value & \bf p-value & \bf p-value
% 			& \bf p-value & \bf p-value & \bf p-value & \bf p-value & \bf p-value & \bf p-value
% 			& \bf p-value & \bf p-value & \bf p-value & \bf p-value \\
% 			\midrule
			
% 			Qwen-0.5B & $<$0.01 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
% 			Qwen-1.5B & 1.00 & 1.00 & 0.77 & 0.77 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 0.46 & $<$0.01 & 0.04 & 1.00 \\
% 			Qwen-3B   & 0.06 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & $<$0.01 & 0.79 & 1.00 \\
			
% 			\bottomrule
% 		\end{tabular}
% 	}
% 	\vspace{-0.2cm}
% \end{table*}

==> tables/stat-tables/rq2-stat-cg.tex <==
% % ==================== COMBINED RQ2 TABLE ====================
% \begin{table*}[h]
% 	\centering
% 	\caption{Statistical comparison of MT-QLoRA vs MT-FFT for Python and Java code generation. Significance assessed using McNemar Test for Pass@1 and Wilcoxon Signed-Rank Test for quality metrics. Effect size measured by Odds Ratio (OR) for Pass@1 and Cliff's Delta (d) for quality metrics (N: negligible, S: small, M: medium, L: large). All p-values are Holm-Bonferroni corrected.}
% 	\label{tab:rq2-stat}
% 	%\scriptsize
%     \small
	
% 	% ===== Python =====
% 	\resizebox{\linewidth}{!}{
% 		\begin{tabular}{>{\centering\arraybackslash}m{1.8cm} | rr | rr rr rr | rr rr rr rr | rr rr rr rr}
% 			\toprule
% 			\multicolumn{25}{c}{\textbf{Python}} \\
% 			\midrule
% 			& \multicolumn{2}{c|}{\bf Pass@1} & \multicolumn{6}{c|}{\bf Lizard} & \multicolumn{8}{c|}{\bf Pylint} & \multicolumn{8}{c}{\bf SonarCloud} \\
% 			\cmidrule(lr){2-3} \cmidrule(lr){4-9} \cmidrule(lr){10-17} \cmidrule(lr){18-25}
			
% 			\bf Model
% 			& \multicolumn{2}{c|}{}
% 			& \multicolumn{2}{c}{\bf LoC} & \multicolumn{2}{c}{\bf Tok} & \multicolumn{2}{c|}{\bf CyC}
% 			& \multicolumn{2}{c}{\bf Err} & \multicolumn{2}{c}{\bf Warn} & \multicolumn{2}{c}{\bf Conv} & \multicolumn{2}{c|}{\bf Ref}
% 			& \multicolumn{2}{c}{\bf Rel} & \multicolumn{2}{c}{\bf Main} & \multicolumn{2}{c}{\bf CyC} & \multicolumn{2}{c}{\bf CoC} \\
			
% 			& \bf p-value & \bf OR 
% 			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d 
% 			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d 
% 			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d \\
% 			\midrule
			
% 			Qwen-0.5B & 1.00 & 1.085 & 0.39 & -0.053 (N) & 0.39 & -0.067 (N) & 1.00 & 0.015 (N) & 1.00 & -0.040 (N) & 1.00 & 0.004 (N) & 1.00 & -0.013 (N) & 1.00 & -0.050 (N) & 1.00 & -0.006 (N) & 1.00 & -0.014 (N) & 0.23 & 0.140 (N) & 1.00 & 0.069 (N) \\
% 			Qwen-1.5B & 1.00 & 1.293 & 1.00 & -0.052 (N) & 1.00 & -0.064 (N) & 1.00 & -0.054 (N) & 1.00 & -0.042 (N) & 0.44 & 0.075 (N) & 1.00 & 0.070 (N) & 1.00 & 0.034 (N) & 1.00 & -0.005 (N) & 0.54 & 0.067 (N) & 1.00 & 0.035 (N) & 1.00 & -0.003 (N) \\
% 			Qwen-3B   & 0.27 & 5.667 & $<$0.01 & -0.137 (N) & $<$0.01 & -0.134 (N) & 0.01 & -0.077 (N) & 0.80 & -0.041 (N) & 0.91 & 0.000 (N) & $<$0.01 & 0.142 (N) & 0.28 & -0.055 (N) & 0.18 & 0.026 (N) & 0.28 & -0.055 (N) & 0.91 & 0.032 (N) & 0.91 & -0.002 (N) \\
			
% 			\bottomrule
% 		\end{tabular}
% 	}
	
% 	\vspace{0.3cm}
	
% 	% ===== Java =====
% 	\resizebox{\linewidth}{!}{
% 		\begin{tabular}{>{\centering\arraybackslash}m{1.8cm} | rr | rr rr rr | rr rr rr rr rr rr | rr rr rr rr}
% 			\toprule
% 			\multicolumn{29}{c}{\textbf{Java}} \\
% 			\midrule
% 			& \multicolumn{2}{c|}{\bf Pass@1} & \multicolumn{6}{c|}{\bf Lizard} & \multicolumn{12}{c|}{\bf PMD} & \multicolumn{8}{c}{\bf SonarCloud} \\
% 			\cmidrule(lr){2-3} \cmidrule(lr){4-9} \cmidrule(lr){10-21} \cmidrule(lr){22-29}
			
% 			\bf Model
% 			& \multicolumn{2}{c|}{}
% 			& \multicolumn{2}{c}{\bf LoC} & \multicolumn{2}{c}{\bf Tok} & \multicolumn{2}{c|}{\bf CyC}
% 			& \multicolumn{2}{c}{\bf BP} & \multicolumn{2}{c}{\bf CS} & \multicolumn{2}{c}{\bf Des} & \multicolumn{2}{c}{\bf EP} & \multicolumn{2}{c}{\bf MT} & \multicolumn{2}{c|}{\bf Perf}
% 			& \multicolumn{2}{c}{\bf Rel} & \multicolumn{2}{c}{\bf Main} & \multicolumn{2}{c}{\bf CyC} & \multicolumn{2}{c}{\bf CoC} \\
			
% 			& \bf p-value & \bf OR 
% 			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d 
% 			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d 
% 			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d \\
% 			\midrule
			
% 			Qwen-0.5B & 1.00 & 1.190 & $<$0.01 & -0.167 (S) & 0.10 & -0.116 (N) & 1.00 & -0.087 (N) & 0.54 & -0.054 (N) & 0.52 & -0.062 (N) & 1.00 & 0.024 (N) & 1.00 & -0.032 (N) & 1.00 & -0.005 (N) & 1.00 & -0.017 (N) & 1.00 & 0.000 (N) & 0.42 & -0.104 (N) & 0.65 & -0.111 (N) & 0.03 & -0.154 (S) \\
% 			Qwen-1.5B & 1.00 & 0.886 & $<$0.01 & -0.250 (S) & $<$0.01 & -0.257 (S) & $<$0.01 & -0.232 (S) & 0.17 & -0.075 (N) & 0.15 & -0.103 (N) & 1.00 & -0.014 (N) & 1.00 & -0.041 (N) & 0.78 & -0.016 (N) & 0.78 & -0.038 (N) & 1.00 & -0.005 (N) & 0.31 & -0.118 (N) & $<$0.01 & -0.252 (S) & $<$0.01 & -0.208 (S) \\
% 			Qwen-3B   & 0.39 & 2.176 & 0.36 & -0.094 (N) & 0.89 & -0.098 (N) & 1.00 & -0.043 (N) & 1.00 & 0.013 (N) & 1.00 & -0.013 (N) & 1.00 & -0.046 (N) & 1.00 & -0.007 (N) & 1.00 & 0.005 (N) & 0.06 & -0.055 (N) & 1.00 & 0.005 (N) & 1.00 & -0.065 (N) & 1.00 & -0.021 (N) & 1.00 & -0.018 (N) \\
			
% 			\bottomrule
% 		\end{tabular}
% 	}
% 	\vspace{-0.2cm}
% \end{table*}

% ==================== COMBINED RQ2 TABLE ====================
\begin{table*}[h]
	\centering
	\caption{Statistical comparison of MT-QLoRA vs MT-FFT for Python and Java code generation. Significance assessed using McNemar Test for Pass@1 and Wilcoxon Signed-Rank Test for quality metrics. Effect size measured by Odds Ratio (OR) for Pass@1 and Cliff's Delta (d) for quality metrics. All p-values are Holm-Bonferroni corrected. P-values are reported as ``x'' when $\geq$ 0.05 (not statistically significant) and as the actual value when $< 0.05$ (significant). Cliff's Delta effect sizes are provided for all comparisons with labels indicating magnitude: N (Negligible: $|\delta| < 0.147$), S (Small: $0.147 \leq |\delta| < 0.33$), M (Medium: $0.33 \leq |\delta| < 0.474$), L (Large: $|\delta| \geq 0.474$).}
	\label{tab:rq2-stat}
	%\scriptsize
    \small
	
	% ===== Python =====
	\resizebox{\linewidth}{!}{
		\begin{tabular}{>{\centering\arraybackslash}m{1.8cm} | rr | rr rr rr | rr rr rr rr | rr rr rr}
			\toprule
			\multicolumn{23}{c}{\textbf{Python}} \\
			\midrule
			& \multicolumn{2}{c|}{\bf Pass@1} & \multicolumn{6}{c|}{\bf Lizard} & \multicolumn{8}{c|}{\bf Pylint} & \multicolumn{6}{c}{\bf SonarCloud} \\
			\cmidrule(lr){2-3} \cmidrule(lr){4-9} \cmidrule(lr){10-17} \cmidrule(lr){18-23}
			
			\bf Model
			& \multicolumn{2}{c|}{}
			& \multicolumn{2}{c}{\bf LoC} & \multicolumn{2}{c}{\bf Tok} & \multicolumn{2}{c|}{\bf CyC}
			& \multicolumn{2}{c}{\bf Err} & \multicolumn{2}{c}{\bf Warn} & \multicolumn{2}{c}{\bf Conv} & \multicolumn{2}{c|}{\bf Ref}
			& \multicolumn{2}{c}{\bf Rel} & \multicolumn{2}{c}{\bf Main} & \multicolumn{2}{c}{\bf CoC} \\
			
			& \bf p-value & \bf OR 
			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d 
			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d 
			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d \\
			\midrule
			
			Qwen-0.5B & x & 1.085 & x & -0.053 (N) & x & -0.067 (N) & x & 0.015 (N) & x & -0.040 (N) & x & 0.004 (N) & x & -0.013 (N) & x & -0.050 (N) & x & -0.006 (N) & x & -0.014 (N) & x & 0.069 (N) \\
			Qwen-1.5B & x & 1.293 & x & -0.052 (N) & x & -0.064 (N) & x & -0.054 (N) & x & -0.042 (N) & x & 0.075 (N) & x & 0.070 (N) & x & 0.034 (N) & x & -0.005 (N) & x & 0.067 (N) & x & -0.003 (N) \\
			Qwen-3B   & x & 5.667 & $<$0.01 & -0.137 (N) & $<$0.01 & -0.134 (N) & 0.01 & -0.077 (N) & x & -0.041 (N) & x & 0.000 (N) & $<$0.01 & 0.142 (N) & x & -0.055 (N) & x & 0.026 (N) & x & -0.055 (N) & x & -0.002 (N) \\
			
			\bottomrule
		\end{tabular}
	}
	
	\vspace{0.3cm}
	
	% ===== Java =====
	\resizebox{\linewidth}{!}{
		\begin{tabular}{>{\centering\arraybackslash}m{1.8cm} | rr | rr rr rr | rr rr rr rr rr rr | rr rr rr}
			\toprule
			\multicolumn{27}{c}{\textbf{Java}} \\
			\midrule
			& \multicolumn{2}{c|}{\bf Pass@1} & \multicolumn{6}{c|}{\bf Lizard} & \multicolumn{12}{c|}{\bf PMD} & \multicolumn{6}{c}{\bf SonarCloud} \\
			\cmidrule(lr){2-3} \cmidrule(lr){4-9} \cmidrule(lr){10-21} \cmidrule(lr){22-27}
			
			\bf Model
			& \multicolumn{2}{c|}{}
			& \multicolumn{2}{c}{\bf LoC} & \multicolumn{2}{c}{\bf Tok} & \multicolumn{2}{c|}{\bf CyC}
			& \multicolumn{2}{c}{\bf BP} & \multicolumn{2}{c}{\bf CS} & \multicolumn{2}{c}{\bf Des} & \multicolumn{2}{c}{\bf EP} & \multicolumn{2}{c}{\bf MT} & \multicolumn{2}{c|}{\bf Perf}
			& \multicolumn{2}{c}{\bf Rel} & \multicolumn{2}{c}{\bf Main} & \multicolumn{2}{c}{\bf CoC} \\
			
			& \bf p-value & \bf OR 
			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d 
			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d 
			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d \\
			\midrule
			
			Qwen-0.5B & x & 1.190 & $<$0.01 & -0.167 (S) & x & -0.116 (N) & x & -0.087 (N) & x & -0.054 (N) & x & -0.062 (N) & x & 0.024 (N) & x & -0.032 (N) & x & -0.005 (N) & x & -0.017 (N) & x & 0.000 (N) & x & -0.104 (N) & 0.03 & -0.154 (S) \\
			Qwen-1.5B & x & 0.886 & $<$0.01 & -0.250 (S) & $<$0.01 & -0.257 (S) & $<$0.01 & -0.232 (S) & x & -0.075 (N) & x & -0.103 (N) & x & -0.014 (N) & x & -0.041 (N) & x & -0.016 (N) & x & -0.038 (N) & x & -0.005 (N) & x & -0.118 (N) & $<$0.01 & -0.208 (S) \\
			Qwen-3B   & x & 2.176 & x & -0.094 (N) & x & -0.098 (N) & x & -0.043 (N) & x & 0.013 (N) & x & -0.013 (N) & x & -0.046 (N) & x & -0.007 (N) & x & 0.005 (N) & x & -0.055 (N) & x & 0.005 (N) & x & -0.065 (N) & x & -0.018 (N) \\
			
			\bottomrule
		\end{tabular}
	}
	\vspace{-0.2cm}
\end{table*}

% % ==================== COMBINED RQ2 TABLE ====================
% \begin{table*}[h]
% 	\centering
% 	\caption{Statistical comparison of MT-QLoRA vs MT-FFT for Python and Java code generation. Significance assessed using McNemar Test for Pass@1 and Wilcoxon Signed-Rank Test for quality metrics. Effect size measured by Odds Ratio (OR) for Pass@1. All p-values are Holm-Bonferroni corrected.}
% 	\label{tab:rq2-stat}
% 	%\scriptsize
%     \small
	
% 	% ===== Python =====
% 	\resizebox{1\textwidth}{!}{%
% 		\begin{tabular}{>{\centering\arraybackslash}m{1.8cm} | r | r r r | r r r r | r r r r}
% 			\toprule
% 			\multicolumn{13}{c}{\textbf{Python}} \\
% 			\midrule
% 			& \multicolumn{1}{c|}{\bf Pass@1} & \multicolumn{3}{c|}{\bf Lizard} & \multicolumn{4}{c|}{\bf Pylint} & \multicolumn{4}{c}{\bf SonarCloud} \\
% 			\cmidrule(lr){2-2} \cmidrule(lr){3-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
			
% 			\bf Model
% 			& \multicolumn{1}{c|}{}
% 			& \multicolumn{1}{c}{\bf LoC} & \multicolumn{1}{c}{\bf Tok} & \multicolumn{1}{c|}{\bf CyC}
% 			& \multicolumn{1}{c}{\bf Err} & \multicolumn{1}{c}{\bf Warn} & \multicolumn{1}{c}{\bf Conv} & \multicolumn{1}{c|}{\bf Ref}
% 			& \multicolumn{1}{c}{\bf Rel} & \multicolumn{1}{c}{\bf Main} & \multicolumn{1}{c}{\bf CyC} & \multicolumn{1}{c}{\bf CoC} \\
			
% 			& \bf OR 
% 			& \bf p-value & \bf p-value & \bf p-value 
% 			& \bf p-value & \bf p-value & \bf p-value & \bf p-value 
% 			& \bf p-value & \bf p-value & \bf p-value & \bf p-value \\
% 			\midrule
			
% 			Qwen-0.5B & 1.085 & 0.39 & 0.39 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 0.23 & 1.00 \\
% 			Qwen-1.5B & 1.293 & 1.00 & 1.00 & 1.00 & 1.00 & 0.44 & 1.00 & 1.00 & 1.00 & 0.54 & 1.00 & 1.00 \\
% 			Qwen-3B   & 5.667 & $<$0.01 & $<$0.01 & 0.01 & 0.80 & 0.91 & $<$0.01 & 0.28 & 0.18 & 0.28 & 0.91 & 0.91 \\
			
% 			\bottomrule
% 		\end{tabular}
% 	}
	
% 	\vspace{0.3cm}
	
% 	% ===== Java =====
% 	\resizebox{1\textwidth}{!}{%
% 		\begin{tabular}{>{\centering\arraybackslash}m{1.8cm} | r | r r r | r r r r r r | r r r r}
% 			\toprule
% 			\multicolumn{15}{c}{\textbf{Java}} \\
% 			\midrule
% 			& \multicolumn{1}{c|}{\bf Pass@1} & \multicolumn{3}{c|}{\bf Lizard} & \multicolumn{6}{c|}{\bf PMD} & \multicolumn{4}{c}{\bf SonarCloud} \\
% 			\cmidrule(lr){2-2} \cmidrule(lr){3-5} \cmidrule(lr){6-11} \cmidrule(lr){12-15}
			
% 			\bf Model
% 			& \multicolumn{1}{c|}{}
% 			& \multicolumn{1}{c}{\bf LoC} & \multicolumn{1}{c}{\bf Tok} & \multicolumn{1}{c|}{\bf CyC}
% 			& \multicolumn{1}{c}{\bf BP} & \multicolumn{1}{c}{\bf CS} & \multicolumn{1}{c}{\bf Des} & \multicolumn{1}{c}{\bf EP} & \multicolumn{1}{c}{\bf MT} & \multicolumn{1}{c|}{\bf Perf}
% 			& \multicolumn{1}{c}{\bf Rel} & \multicolumn{1}{c}{\bf Main} & \multicolumn{1}{c}{\bf CyC} & \multicolumn{1}{c}{\bf CoC} \\
			
% 			& \bf OR 
% 			& \bf p-value & \bf p-value & \bf p-value 
% 			& \bf p-value & \bf p-value & \bf p-value & \bf p-value & \bf p-value & \bf p-value 
% 			& \bf p-value & \bf p-value & \bf p-value & \bf p-value \\
% 			\midrule
			
% 			Qwen-0.5B & 1.190 & $<$0.01 & 0.10 & 1.00 & 0.54 & 0.52 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 0.42 & 0.65 & 0.03 \\
% 			Qwen-1.5B & 0.886 & $<$0.01 & $<$0.01 & $<$0.01 & 0.17 & 0.15 & 1.00 & 1.00 & 0.78 & 0.78 & 1.00 & 0.31 & $<$0.01 & $<$0.01 \\
% 			Qwen-3B   & 2.176 & 0.36 & 0.89 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 0.06 & 1.00 & 1.00 & 1.00 & 1.00 \\
			
% 			\bottomrule
% 		\end{tabular}
% 	}
% 	\vspace{-0.2cm}
% \end{table*}

==> tables/stat-tables/rq2-stat-cs-llm-judge.tex <==
% ==================== COMBINED RQ2 CODE SUMMARIZATION QUALITY TABLE ====================
\begin{table*}[t!]
	\centering
	\caption{RQ2: Statistical comparison of MT-QLoRA vs MT-FFT for code summarization quality (LLM Judge). Significance assessed using Wilcoxon Signed-Rank Test. Effect size measured by Cliff's Delta (d) (N: negligible, S: small, M: medium, L: large). All p-values are Holm-Bonferroni corrected.}
	\label{tab:rq2-stat-summarization-quality}
	\scriptsize
	
	% ===== Python =====
	\resizebox{0.7\linewidth}{!}{
		\begin{tabular}{>{\centering\arraybackslash}m{1.8cm} | rr rr rr}
			\toprule
			\multicolumn{7}{c}{\textbf{Python}} \\
			\midrule
			\bf Model
			& \multicolumn{2}{c}{\bf CA} & \multicolumn{2}{c}{\bf Conciseness} & \multicolumn{2}{c}{\bf Fluency} \\
			
			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d \\
			\midrule
			
			Qwen-0.5B & 1.00 & 0.009 (N) & 1.00 & 0.005 (N) & 1.00 & -0.007 (N) \\
			Qwen-1.5B & 0.31 & -0.014 (N) & 0.09 & 0.077 (N) & 0.50 & -0.061 (N) \\
			Qwen-3B   & 1.00 & 0.042 (N) & 1.00 & -0.026 (N) & 1.00 & -0.003 (N) \\
			
			\bottomrule
		\end{tabular}
	}
	
	\vspace{0.3cm}
	
	% ===== Java =====
	\resizebox{0.7\linewidth}{!}{
		\begin{tabular}{>{\centering\arraybackslash}m{1.8cm} | rr rr rr}
			\toprule
			\multicolumn{7}{c}{\textbf{Java}} \\
			\midrule
			\bf Model
			& \multicolumn{2}{c}{\bf CA} & \multicolumn{2}{c}{\bf Conciseness} & \multicolumn{2}{c}{\bf Fluency} \\
			
			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d \\
			\midrule
			
			Qwen-0.5B & 1.00 & 0.001 (N) & 1.00 & 0.008 (N) & 1.00 & 0.036 (N) \\
			Qwen-1.5B & 0.71 & 0.046 (N) & 0.40 & 0.061 (N) & 0.40 & 0.087 (N) \\
			Qwen-3B   & 0.25 & 0.084 (N) & 0.25 & 0.033 (N) & 0.05 & 0.186 (S) \\
			
			\bottomrule
		\end{tabular}
	}
	\vspace{-0.2cm}
\end{table*}

==> tables/stat-tables/rq2-stat-cs.tex <==
% % ==================== COMBINED RQ2 CODE SUMMARIZATION TABLE ====================
% \begin{table*}[h]
% 	\centering
% 	\caption{Statistical comparison of MT-QLoRA vs MT-FFT for code summarization. Significance assessed using Wilcoxon Signed-Rank Test. Effect size measured by Cliff's Delta (d) (N: negligible, S: small, M: medium, L: large). All p-values are Holm-Bonferroni corrected.}
% 	\label{tab:rq2-stat-summarization}
% 	%\scriptsize
%     \small
	
% 	% ===== Java =====
% 	\resizebox{\linewidth}{!}{
% 		\begin{tabular}{>{\centering\arraybackslash}m{1.8cm} | rr rr rr rr rr rr}
% 			\toprule
% 			\multicolumn{13}{c}{\textbf{Java}} \\
% 			\midrule
% 			\bf Model
% 			& \multicolumn{2}{c}{\bf BLEU} & \multicolumn{2}{c}{\bf METEOR} & \multicolumn{2}{c}{\bf Rouge-L} & \multicolumn{2}{c}{\bf chrF} & \multicolumn{2}{c}{\bf BERTScore} & \multicolumn{2}{c}{\bf SIDE} \\
			
% 			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d \\
% 			\midrule
			
% 			Qwen-0.5B & 1.00 & -0.011 (N) & 0.62 & 0.035 (N) & 0.01 & 0.103 (N) & 1.00 & -0.018 (N) & 1.00 & 0.009 (N) & 0.12 & 0.097 (N) \\
% 			Qwen-1.5B & 1.00 & 0.008 (N) & 1.00 & 0.030 (N) & 1.00 & 0.017 (N) & 1.00 & 0.041 (N) & 1.00 & 0.026 (N) & 0.05 & 0.086 (N) \\
% 			Qwen-3B   & 1.00 & -0.055 (N) & 1.00 & 0.026 (N) & 0.56 & 0.036 (N) & 1.00 & 0.018 (N) & 1.00 & 0.008 (N) & 1.00 & 0.026 (N) \\
			
% 			\bottomrule
% 		\end{tabular}
% 	}
	
% 	\vspace{0.3cm}
	
% 	% ===== Python =====
% 	\resizebox{\linewidth}{!}{
% 		\begin{tabular}{>{\centering\arraybackslash}m{1.8cm} | rr rr rr rr rr}
% 			\toprule
% 			\multicolumn{11}{c}{\textbf{Python}} \\
% 			\midrule
% 			\bf Model
% 			& \multicolumn{2}{c}{\bf BLEU} & \multicolumn{2}{c}{\bf METEOR} & \multicolumn{2}{c}{\bf Rouge-L} & \multicolumn{2}{c}{\bf chrF} & \multicolumn{2}{c}{\bf BERTScore} \\
			
% 			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d \\
% 			\midrule
			
% 			Qwen-0.5B & $<$0.01 & 0.171 (S) & $<$0.01 & 0.175 (S) & $<$0.01 & 0.228 (S) & $<$0.01 & 0.223 (S) & $<$0.01 & 0.222 (S) \\
% 			Qwen-1.5B & $<$0.01 & 0.125 (N) & $<$0.01 & 0.139 (N) & $<$0.01 & 0.194 (S) & $<$0.01 & 0.156 (S) & $<$0.01 & 0.192 (S) \\
% 			Qwen-3B   & $<$0.01 & 0.189 (S) & $<$0.01 & 0.194 (S) & $<$0.01 & 0.215 (S) & $<$0.01 & 0.185 (S) & $<$0.01 & 0.170 (S) \\
			
% 			\bottomrule
% 		\end{tabular}
% 	}
% 	\vspace{-0.2cm}
% \end{table*}

% ==================== COMBINED RQ2 CODE SUMMARIZATION TABLE ====================
\begin{table*}[h]
	\centering
	\caption{Statistical comparison of MT-QLoRA vs MT-FFT for code summarization. Significance assessed using Wilcoxon Signed-Rank Test. All p-values are Holm-Bonferroni corrected. P-values are reported as ``x'' when $\geq$ 0.05 (not statistically significant) and as the actual value when $< 0.05$ (significant). Cliff's Delta effect sizes are provided for all comparisons with labels indicating magnitude: N (Negligible: $|\delta| < 0.147$), S (Small: $0.147 \leq |\delta| < 0.33$), M (Medium: $0.33 \leq |\delta| < 0.474$), L (Large: $|\delta| \geq 0.474$).}
	\label{tab:rq2-stat-summarization}
	%\scriptsize
    \small
	
	% ===== Java =====
	\resizebox{\linewidth}{!}{
		\begin{tabular}{>{\centering\arraybackslash}m{1.8cm} | rr rr rr rr rr rr}
			\toprule
			\multicolumn{13}{c}{\textbf{Java}} \\
			\midrule
			\bf Model
			& \multicolumn{2}{c}{\bf BLEU} & \multicolumn{2}{c}{\bf METEOR} & \multicolumn{2}{c}{\bf Rouge-L} & \multicolumn{2}{c}{\bf chrF} & \multicolumn{2}{c}{\bf BERTScore} & \multicolumn{2}{c}{\bf SIDE} \\
			
			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d \\
			\midrule
			
			Qwen-0.5B & x & -0.011 (N) & x & 0.035 (N) & 0.01 & 0.103 (N) & x & -0.018 (N) & x & 0.009 (N) & x & 0.097 (N) \\
			Qwen-1.5B & x & 0.008 (N) & x & 0.030 (N) & x & 0.017 (N) & x & 0.041 (N) & x & 0.026 (N) & x & 0.086 (N) \\
			Qwen-3B   & x & -0.055 (N) & x & 0.026 (N) & x & 0.036 (N) & x & 0.018 (N) & x & 0.008 (N) & x & 0.026 (N) \\
			
			\bottomrule
		\end{tabular}
	}
	
	\vspace{0.3cm}
	
	% ===== Python =====
	\resizebox{\linewidth}{!}{
		\begin{tabular}{>{\centering\arraybackslash}m{1.8cm} | rr rr rr rr rr}
			\toprule
			\multicolumn{11}{c}{\textbf{Python}} \\
			\midrule
			\bf Model
			& \multicolumn{2}{c}{\bf BLEU} & \multicolumn{2}{c}{\bf METEOR} & \multicolumn{2}{c}{\bf Rouge-L} & \multicolumn{2}{c}{\bf chrF} & \multicolumn{2}{c}{\bf BERTScore} \\
			
			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d \\
			\midrule
			
			Qwen-0.5B & $<$0.01 & 0.171 (S) & $<$0.01 & 0.175 (S) & $<$0.01 & 0.228 (S) & $<$0.01 & 0.223 (S) & $<$0.01 & 0.222 (S) \\
			Qwen-1.5B & $<$0.01 & 0.125 (N) & $<$0.01 & 0.139 (N) & $<$0.01 & 0.194 (S) & $<$0.01 & 0.156 (S) & $<$0.01 & 0.192 (S) \\
			Qwen-3B   & $<$0.01 & 0.189 (S) & $<$0.01 & 0.194 (S) & $<$0.01 & 0.215 (S) & $<$0.01 & 0.185 (S) & $<$0.01 & 0.170 (S) \\
			
			\bottomrule
		\end{tabular}
	}
	\vspace{-0.2cm}
\end{table*}

% % ==================== COMBINED RQ2 CODE SUMMARIZATION TABLE ====================
% \begin{table*}[h]
% 	\centering
% 	\caption{Statistical comparison of MT-QLoRA vs MT-FFT for code summarization. Significance assessed using Wilcoxon Signed-Rank Test. All p-values are Holm-Bonferroni corrected.}
% 	\label{tab:rq2-stat-summarization}
% 	%\scriptsize
%     \small
	
% 	% ===== Java =====
% 	\resizebox{0.75\textwidth}{!}{%
% 		\begin{tabular}{>{\centering\arraybackslash}m{1.8cm} | r r r r r r}
% 			\toprule
% 			\multicolumn{7}{c}{\textbf{Java}} \\
% 			\midrule
% 			\bf Model
% 			& \multicolumn{1}{c}{\bf BLEU} & \multicolumn{1}{c}{\bf METEOR} & \multicolumn{1}{c}{\bf Rouge-L} & \multicolumn{1}{c}{\bf chrF} & \multicolumn{1}{c}{\bf BERTScore} & \multicolumn{1}{c}{\bf SIDE} \\
			
% 			& \bf p-value & \bf p-value & \bf p-value & \bf p-value & \bf p-value & \bf p-value \\
% 			\midrule
			
% 			Qwen-0.5B & 1.00 & 0.62 & 0.01 & 1.00 & 1.00 & 0.12 \\
% 			Qwen-1.5B & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 0.05 \\
% 			Qwen-3B   & 1.00 & 1.00 & 0.56 & 1.00 & 1.00 & 1.00 \\
			
% 			\bottomrule
% 		\end{tabular}
% 	}
	
% 	\vspace{0.3cm}
	
% 	% ===== Python =====
% 	\resizebox{0.75\textwidth}{!}{%
% 		\begin{tabular}{>{\centering\arraybackslash}m{1.8cm} | r r r r r}
% 			\toprule
% 			\multicolumn{6}{c}{\textbf{Python}} \\
% 			\midrule
% 			\bf Model
% 			& \multicolumn{1}{c}{\bf BLEU} & \multicolumn{1}{c}{\bf METEOR} & \multicolumn{1}{c}{\bf Rouge-L} & \multicolumn{1}{c}{\bf chrF} & \multicolumn{1}{c}{\bf BERTScore} \\
			
% 			& \bf p-value & \bf p-value & \bf p-value & \bf p-value & \bf p-value \\
% 			\midrule
			
% 			Qwen-0.5B & $<$0.01 & $<$0.01 & $<$0.01 & $<$0.01 & $<$0.01 \\
% 			Qwen-1.5B & $<$0.01 & $<$0.01 & $<$0.01 & $<$0.01 & $<$0.01 \\
% 			Qwen-3B   & $<$0.01 & $<$0.01 & $<$0.01 & $<$0.01 & $<$0.01 \\
			
% 			\bottomrule
% 		\end{tabular}
% 	}
% 	\vspace{-0.2cm}
% \end{table*}

==> tables/stat-tables/rq2-stat-ct.tex <==
% % ==================== COMBINED RQ2 CODE TRANSLATION TABLE ====================
% \begin{table*}[h]
% 	\centering
% 	\caption{Statistical comparison of MT-QLoRA vs MT-FFT for code translation. Significance assessed using Wilcoxon Signed-Rank Test. Effect size measured by Cliff's Delta (d) (N: negligible, S: small, M: medium, L: large). All p-values are Holm-Bonferroni corrected.}
% 	\label{tab:rq2-stat-translation}
% 	%\scriptsize
%     \small
	
% 	% ===== Java to C# =====
% 	\resizebox{\linewidth}{!}{
% 		\begin{tabular}{>{\centering\arraybackslash}m{1.8cm} | rr | rr rr rr | rr rr}
% 			\toprule
% 			\multicolumn{13}{c}{\textbf{Java to C\#}} \\
% 			\midrule
% 			& \multicolumn{2}{c|}{\bf CodeBLEU} & \multicolumn{6}{c|}{\bf Lizard} & \multicolumn{4}{c}{\bf Roslyn} \\
% 			\cmidrule(lr){2-3} \cmidrule(lr){4-9} \cmidrule(lr){10-13}
			
% 			\bf Model
% 			& \multicolumn{2}{c|}{}
% 			& \multicolumn{2}{c}{\bf LoC} & \multicolumn{2}{c}{\bf Tok} & \multicolumn{2}{c|}{\bf CyC}
% 			& \multicolumn{2}{c}{\bf Syntax} & \multicolumn{2}{c}{\bf Main} \\
			
% 			& \bf p-value & \bf d 
% 			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d 
% 			& \bf p-value & \bf d & \bf p-value & \bf d \\
% 			\midrule
			
% 			Qwen-0.5B & $<$0.01 & -0.108 (N) & 1.00 & 0.016 (N) & 1.00 & 0.000 (N) & 0.60 & 0.010 (N) & 1.00 & 0.003 (N) & 1.00 & 0.007 (N) \\
% 			Qwen-1.5B & $<$0.01 & -0.138 (N) & $<$0.01 & -0.034 (N) & $<$0.01 & -0.035 (N) & $<$0.01 & -0.028 (N) & 0.24 & 0.009 (N) & 0.18 & 0.012 (N) \\
% 			Qwen-3B   & $<$0.01 & -0.131 (N) & 1.00 & -0.004 (N) & 1.00 & -0.011 (N) & 1.00 & -0.005 (N) & $<$0.01 & -0.107 (N) & $<$0.01 & 0.283 (S) \\
			
% 			\bottomrule
% 		\end{tabular}
% 	}
	
% 	\vspace{0.3cm}
	
% 	% ===== C# to Java =====
% 	\resizebox{\linewidth}{!}{
% 		\begin{tabular}{>{\centering\arraybackslash}m{1.8cm} | rr | rr rr rr | rr rr rr rr rr rr | rr rr rr rr}
% 			\toprule
% 			\multicolumn{29}{c}{\textbf{C\# to Java}} \\
% 			\midrule
% 			& \multicolumn{2}{c|}{\bf CodeBLEU} & \multicolumn{6}{c|}{\bf Lizard} & \multicolumn{12}{c|}{\bf PMD} & \multicolumn{8}{c}{\bf SonarCloud} \\
% 			\cmidrule(lr){2-3} \cmidrule(lr){4-9} \cmidrule(lr){10-21} \cmidrule(lr){22-29}
			
% 			\bf Model
% 			& \multicolumn{2}{c|}{}
% 			& \multicolumn{2}{c}{\bf LoC} & \multicolumn{2}{c}{\bf Tok} & \multicolumn{2}{c|}{\bf CyC}
% 			& \multicolumn{2}{c}{\bf BP} & \multicolumn{2}{c}{\bf CS} & \multicolumn{2}{c}{\bf Des} & \multicolumn{2}{c}{\bf EP} & \multicolumn{2}{c}{\bf MT} & \multicolumn{2}{c|}{\bf Perf}
% 			& \multicolumn{2}{c}{\bf Rel} & \multicolumn{2}{c}{\bf Main} & \multicolumn{2}{c}{\bf CyC} & \multicolumn{2}{c}{\bf CoC} \\
			
% 			& \bf p-value & \bf d 
% 			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d 
% 			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d 
% 			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d \\
% 			\midrule
			
% 			Qwen-0.5B & $<$0.01 & -0.104 (N) & $<$0.01 & 0.053 (N) & $<$0.01 & 0.047 (N) & 0.09 & 0.029 (N) & 0.54 & -0.054 (N) & 0.52 & -0.062 (N) & 1.00 & 0.024 (N) & 1.00 & -0.032 (N) & 1.00 & -0.005 (N) & 1.00 & -0.017 (N) & 1.00 & -0.006 (N) & 1.00 & -0.013 (N) & 1.00 & 0.001 (N) & 0.82 & 0.019 (N) \\
% 			Qwen-1.5B & 1.00 & -0.013 (N) & 0.33 & 0.011 (N) & 0.07 & 0.012 (N) & 1.00 & -0.008 (N) & 0.23 & -0.075 (N) & 0.22 & -0.103 (N) & 1.00 & -0.014 (N) & 1.00 & -0.041 (N) & 1.00 & -0.016 (N) & 1.00 & -0.038 (N) & 0.15 & 0.005 (N) & 0.22 & 0.028 (N) & 1.00 & 0.021 (N) & 0.50 & 0.006 (N) \\
% 			Qwen-3B   & $<$0.01 & -0.314 (S) & 1.00 & -0.018 (N) & 0.07 & -0.019 (N) & 1.00 & 0.000 (N) & 1.00 & 0.013 (N) & 1.00 & -0.013 (N) & 1.00 & -0.046 (N) & 1.00 & -0.007 (N) & 1.00 & 0.005 (N) & 0.04 & -0.055 (N) & 0.90 & -0.006 (N) & $<$0.01 & -0.435 (M) & $<$0.01 & -0.464 (M) & $<$0.01 & -0.146 (N) \\
			
% 			\bottomrule
% 		\end{tabular}
% 	}
% 	\vspace{-0.2cm}
% \end{table*}

% ==================== COMBINED RQ2 CODE TRANSLATION TABLE ====================
\begin{table*}[h]
	\centering
	\caption{Statistical comparison of MT-QLoRA vs MT-FFT for code translation. Significance assessed using Wilcoxon Signed-Rank Test. All p-values are Holm-Bonferroni corrected. P-values are reported as ``x'' when $\geq$ 0.05 (not statistically significant) and as the actual value when $< 0.05$ (significant). Cliff's Delta effect sizes are provided for all comparisons with labels indicating magnitude: N (Negligible: $|\delta| < 0.147$), S (Small: $0.147 \leq |\delta| < 0.33$), M (Medium: $0.33 \leq |\delta| < 0.474$), L (Large: $|\delta| \geq 0.474$).}
	\label{tab:rq2-stat-translation}
	%\scriptsize
    \small
	
	% ===== Java to C# =====
	\resizebox{\linewidth}{!}{
		\begin{tabular}{>{\centering\arraybackslash}m{1.8cm} | rr | rr rr rr | rr rr}
			\toprule
			\multicolumn{13}{c}{\textbf{Java to C\#}} \\
			\midrule
			& \multicolumn{2}{c|}{\bf CodeBLEU} & \multicolumn{6}{c|}{\bf Lizard} & \multicolumn{4}{c}{\bf Roslyn} \\
			\cmidrule(lr){2-3} \cmidrule(lr){4-9} \cmidrule(lr){10-13}
			
			\bf Model
			& \multicolumn{2}{c|}{}
			& \multicolumn{2}{c}{\bf LoC} & \multicolumn{2}{c}{\bf Tok} & \multicolumn{2}{c|}{\bf CyC}
			& \multicolumn{2}{c}{\bf Syntax} & \multicolumn{2}{c}{\bf Main} \\
			
			& \bf p-value & \bf d 
			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d 
			& \bf p-value & \bf d & \bf p-value & \bf d \\
			\midrule
			
			Qwen-0.5B & $<$0.01 & -0.108 (N) & x & 0.016 (N) & x & 0.000 (N) & x & 0.010 (N) & x & 0.003 (N) & x & 0.007 (N) \\
			Qwen-1.5B & $<$0.01 & -0.138 (N) & $<$0.01 & -0.034 (N) & $<$0.01 & -0.035 (N) & $<$0.01 & -0.028 (N) & x & 0.009 (N) & x & 0.012 (N) \\
			Qwen-3B   & $<$0.01 & -0.131 (N) & x & -0.004 (N) & x & -0.011 (N) & x & -0.005 (N) & $<$0.01 & -0.107 (N) & $<$0.01 & 0.283 (S) \\
			
			\bottomrule
		\end{tabular}
	}
	
	\vspace{0.3cm}
	
	% ===== C# to Java =====
	\resizebox{\linewidth}{!}{
		\begin{tabular}{>{\centering\arraybackslash}m{1.8cm} | rr | rr rr rr | rr rr rr rr rr rr | rr rr rr rr}
			\toprule
			\multicolumn{29}{c}{\textbf{C\# to Java}} \\
			\midrule
			& \multicolumn{2}{c|}{\bf CodeBLEU} & \multicolumn{6}{c|}{\bf Lizard} & \multicolumn{12}{c|}{\bf PMD} & \multicolumn{8}{c}{\bf SonarCloud} \\
			\cmidrule(lr){2-3} \cmidrule(lr){4-9} \cmidrule(lr){10-21} \cmidrule(lr){22-29}
			
			\bf Model
			& \multicolumn{2}{c|}{}
			& \multicolumn{2}{c}{\bf LoC} & \multicolumn{2}{c}{\bf Tok} & \multicolumn{2}{c|}{\bf CyC}
			& \multicolumn{2}{c}{\bf BP} & \multicolumn{2}{c}{\bf CS} & \multicolumn{2}{c}{\bf Des} & \multicolumn{2}{c}{\bf EP} & \multicolumn{2}{c}{\bf MT} & \multicolumn{2}{c|}{\bf Perf}
			& \multicolumn{2}{c}{\bf Rel} & \multicolumn{2}{c}{\bf Main} & \multicolumn{2}{c}{\bf CyC} & \multicolumn{2}{c}{\bf CoC} \\
			
			& \bf p-value & \bf d 
			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d 
			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d 
			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d \\
			\midrule
			
			Qwen-0.5B & $<$0.01 & -0.104 (N) & $<$0.01 & 0.053 (N) & $<$0.01 & 0.047 (N) & x & 0.029 (N) & x & -0.054 (N) & x & -0.062 (N) & x & 0.024 (N) & x & -0.032 (N) & x & -0.005 (N) & x & -0.017 (N) & x & -0.006 (N) & x & -0.013 (N) & x & 0.001 (N) & x & 0.019 (N) \\
			Qwen-1.5B & x & -0.013 (N) & x & 0.011 (N) & x & 0.012 (N) & x & -0.008 (N) & x & -0.075 (N) & x & -0.103 (N) & x & -0.014 (N) & x & -0.041 (N) & x & -0.016 (N) & x & -0.038 (N) & x & 0.005 (N) & x & 0.028 (N) & x & 0.021 (N) & x & 0.006 (N) \\
			Qwen-3B   & $<$0.01 & -0.314 (S) & x & -0.018 (N) & x & -0.019 (N) & x & 0.000 (N) & x & 0.013 (N) & x & -0.013 (N) & x & -0.046 (N) & x & -0.007 (N) & x & 0.005 (N) & 0.04 & -0.055 (N) & x & -0.006 (N) & $<$0.01 & -0.435 (M) & $<$0.01 & -0.464 (M) & $<$0.01 & -0.146 (N) \\
			
			\bottomrule
		\end{tabular}
	}
	\vspace{-0.2cm}
\end{table*}

% % ==================== COMBINED RQ2 CODE TRANSLATION TABLE ====================
% \begin{table*}[h]
% 	\centering
% 	\caption{Statistical comparison of MT-QLoRA vs MT-FFT for code translation. Significance assessed using Wilcoxon Signed-Rank Test. All p-values are Holm-Bonferroni corrected.}
% 	\label{tab:rq2-stat-translation}
% 	%\scriptsize
%     \small
	
% 	% ===== Java to C# =====
% 	\resizebox{0.75\textwidth}{!}{%
% 		\begin{tabular}{>{\centering\arraybackslash}m{1.8cm} | r | r r r | r r}
% 			\toprule
% 			\multicolumn{7}{c}{\textbf{Java to C\#}} \\
% 			\midrule
% 			& \multicolumn{1}{c|}{\bf CodeBLEU} & \multicolumn{3}{c|}{\bf Lizard} & \multicolumn{2}{c}{\bf Roslyn} \\
% 			\cmidrule(lr){2-2} \cmidrule(lr){3-5} \cmidrule(lr){6-7}
			
% 			\bf Model
% 			& \multicolumn{1}{c|}{}
% 			& \multicolumn{1}{c}{\bf LoC} & \multicolumn{1}{c}{\bf Tok} & \multicolumn{1}{c|}{\bf CyC}
% 			& \multicolumn{1}{c}{\bf Syntax} & \multicolumn{1}{c}{\bf Main} \\
			
% 			& \bf p-value
% 			& \bf p-value & \bf p-value & \bf p-value
% 			& \bf p-value & \bf p-value \\
% 			\midrule
			
% 			Qwen-0.5B & $<$0.01 & 1.00 & 1.00 & 0.60 & 1.00 & 1.00 \\
% 			Qwen-1.5B & $<$0.01 & $<$0.01 & $<$0.01 & $<$0.01 & 0.24 & 0.18 \\
% 			Qwen-3B   & $<$0.01 & 1.00 & 1.00 & 1.00 & $<$0.01 & $<$0.01 \\
			
% 			\bottomrule
% 		\end{tabular}
% 	}
	
% 	\vspace{0.3cm}
	
% 	% ===== C# to Java =====
% 	\resizebox{1\textwidth}{!}{%
% 		\begin{tabular}{>{\centering\arraybackslash}m{1.8cm} | r | r r r | r r r r r r | r r r r}
% 			\toprule
% 			\multicolumn{15}{c}{\textbf{C\# to Java}} \\
% 			\midrule
% 			& \multicolumn{1}{c|}{\bf CodeBLEU} & \multicolumn{3}{c|}{\bf Lizard} & \multicolumn{6}{c|}{\bf PMD} & \multicolumn{4}{c}{\bf SonarCloud} \\
% 			\cmidrule(lr){2-2} \cmidrule(lr){3-5} \cmidrule(lr){6-11} \cmidrule(lr){12-15}
			
% 			\bf Model
% 			& \multicolumn{1}{c|}{}
% 			& \multicolumn{1}{c}{\bf LoC} & \multicolumn{1}{c}{\bf Tok} & \multicolumn{1}{c|}{\bf CyC}
% 			& \multicolumn{1}{c}{\bf BP} & \multicolumn{1}{c}{\bf CS} & \multicolumn{1}{c}{\bf Des} & \multicolumn{1}{c}{\bf EP} & \multicolumn{1}{c}{\bf MT} & \multicolumn{1}{c|}{\bf Perf}
% 			& \multicolumn{1}{c}{\bf Rel} & \multicolumn{1}{c}{\bf Main} & \multicolumn{1}{c}{\bf CyC} & \multicolumn{1}{c}{\bf CoC} \\
			
% 			& \bf p-value
% 			& \bf p-value & \bf p-value & \bf p-value
% 			& \bf p-value & \bf p-value & \bf p-value & \bf p-value & \bf p-value & \bf p-value
% 			& \bf p-value & \bf p-value & \bf p-value & \bf p-value \\
% 			\midrule
			
% 			Qwen-0.5B & $<$0.01 & $<$0.01 & $<$0.01 & 0.09 & 0.54 & 0.52 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 0.82 \\
% 			Qwen-1.5B & 1.00 & 0.33 & 0.07 & 1.00 & 0.23 & 0.22 & 1.00 & 1.00 & 1.00 & 1.00 & 0.15 & 0.22 & 1.00 & 0.50 \\
% 			Qwen-3B   & $<$0.01 & 1.00 & 0.07 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 0.04 & 0.90 & $<$0.01 & $<$0.01 & $<$0.01 \\
			
% 			\bottomrule
% 		\end{tabular}
% 	}
% 	\vspace{-0.2cm}
% \end{table*}

==> tables/stat-tables/rq3-stat-cg.tex <==
% % ==================== COMBINED RQ3 TABLE ====================
% \begin{table*}[h]
% 	\centering
% 	\caption{Statistical comparison of 3-task MT-QLoRA vs 2-task MT-QLoRA (Qwen 3B) for Python and Java code generation. Significance assessed using McNemar Test for Pass@1 and Wilcoxon Signed-Rank Test for quality metrics. Effect size measured by Odds Ratio (OR) for Pass@1 and Cliff's Delta (d) for quality metrics (N: negligible, S: small, M: medium, L: large). All p-values are Holm-Bonferroni corrected.}
% 	\label{tab:rq3-stat}
% 	%\scriptsize
% 	\small
% 	% ===== Python =====
% 	\resizebox{\linewidth}{!}{
% 		\begin{tabular}{>{\centering\arraybackslash}m{2.5cm} | rr | rr rr rr | rr rr rr rr | rr rr rr rr}
% 			\toprule
% 			\multicolumn{25}{c}{\textbf{Python}} \\
% 			\midrule
% 			& \multicolumn{2}{c|}{\bf Pass@1} & \multicolumn{6}{c|}{\bf Lizard} & \multicolumn{8}{c|}{\bf Pylint} & \multicolumn{8}{c}{\bf SonarCloud} \\
% 			\cmidrule(lr){2-3} \cmidrule(lr){4-9} \cmidrule(lr){10-17} \cmidrule(lr){18-25}
			
% 			\bf Comparison
% 			& \multicolumn{2}{c|}{}
% 			& \multicolumn{2}{c}{\bf LoC} & \multicolumn{2}{c}{\bf Tok} & \multicolumn{2}{c|}{\bf CyC}
% 			& \multicolumn{2}{c}{\bf Err} & \multicolumn{2}{c}{\bf Warn} & \multicolumn{2}{c}{\bf Conv} & \multicolumn{2}{c|}{\bf Ref}
% 			& \multicolumn{2}{c}{\bf Rel} & \multicolumn{2}{c}{\bf Main} & \multicolumn{2}{c}{\bf CyC} & \multicolumn{2}{c}{\bf CoC} \\
			
% 			& \bf p-value & \bf OR 
% 			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d 
% 			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d 
% 			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d \\
% 			\midrule
			
% 			3-task vs CG+CS & 1.00 & 1.118 & 0.02 & 0.070 (N) & $<$0.01 & 0.087 (N) & 0.22 & 0.076 (N) & 0.56 & 0.038 (N) & $<$0.01 & 0.101 (N) & 1.00 & 0.016 (N) & 1.00 & -0.004 (N) & 0.72 & 0.016 (N) & 1.00 & 0.011 (N) & 0.68 & 0.056 (N) & 0.56 & 0.057 (N) \\
% 			3-task vs CG+CT & 1.00 & 1.000 & 1.00 & -0.006 (N) & 1.00 & 0.013 (N) & 1.00 & 0.032 (N) & 0.07 & 0.058 (N) & 1.00 & 0.023 (N) & 1.00 & 0.015 (N) & 1.00 & 0.025 (N) & 1.00 & 0.016 (N) & 1.00 & 0.017 (N) & 1.00 & 0.015 (N) & 1.00 & 0.013 (N) \\
			
% 			\bottomrule
% 		\end{tabular}
% 	}
	
% 	\vspace{0.3cm}
	
% 	% ===== Java =====
% 	\resizebox{\linewidth}{!}{
% 		\begin{tabular}{>{\centering\arraybackslash}m{2.5cm} | rr | rr rr rr | rr rr rr rr rr rr | rr rr rr rr}
% 			\toprule
% 			\multicolumn{29}{c}{\textbf{Java}} \\
% 			\midrule
% 			& \multicolumn{2}{c|}{\bf Pass@1} & \multicolumn{6}{c|}{\bf Lizard} & \multicolumn{12}{c|}{\bf PMD} & \multicolumn{8}{c}{\bf SonarCloud} \\
% 			\cmidrule(lr){2-3} \cmidrule(lr){4-9} \cmidrule(lr){10-21} \cmidrule(lr){22-29}
			
% 			\bf Comparison
% 			& \multicolumn{2}{c|}{}
% 			& \multicolumn{2}{c}{\bf LoC} & \multicolumn{2}{c}{\bf Tok} & \multicolumn{2}{c|}{\bf CyC}
% 			& \multicolumn{2}{c}{\bf BP} & \multicolumn{2}{c}{\bf CS} & \multicolumn{2}{c}{\bf Des} & \multicolumn{2}{c}{\bf EP} & \multicolumn{2}{c}{\bf MT} & \multicolumn{2}{c|}{\bf Perf}
% 			& \multicolumn{2}{c}{\bf Rel} & \multicolumn{2}{c}{\bf Main} & \multicolumn{2}{c}{\bf CyC} & \multicolumn{2}{c}{\bf CoC} \\
			
% 			& \bf p-value & \bf OR 
% 			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d 
% 			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d 
% 			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d \\
% 			\midrule
			
% 			3-task vs CG+CS & 1.00 & 0.704 & 1.00 & 0.049 (N) & 1.00 & -0.025 (N) & 1.00 & -0.033 (N) & 1.00 & 0.023 (N) & 0.05 & -0.088 (N) & 1.00 & -0.007 (N) & 1.00 & -0.012 (N) & 1.00 & 0.000 (N) & 1.00 & -0.017 (N) & 1.00 & 0.000 (N) & 1.00 & -0.051 (N) & 1.00 & -0.031 (N) & 1.00 & -0.036 (N) \\
% 			3-task vs CG+CT & 0.68 & 0.543 & 1.00 & -0.002 (N) & 1.00 & -0.028 (N) & 1.00 & -0.058 (N) & 1.00 & 0.004 (N) & 1.00 & -0.050 (N) & 1.00 & -0.009 (N) & 0.51 & -0.055 (N) & 1.00 & 0.000 (N) & 1.00 & -0.017 (N) & 1.00 & -0.011 (N) & 1.00 & -0.040 (N) & 1.00 & -0.057 (N) & 1.00 & -0.085 (N) \\
			
% 			\bottomrule
% 		\end{tabular}
% 	}
% 	\vspace{-10pt}
% \end{table*}


% ==================== COMBINED RQ3 TABLE ====================
\begin{table*}[h]
	\centering
	\caption{Statistical comparison of 3-task MT-QLoRA vs 2-task MT-QLoRA (Qwen 3B) for Python and Java code generation. Significance assessed using McNemar Test for Pass@1 and Wilcoxon Signed-Rank Test for quality metrics. Effect size measured by Odds Ratio (OR) for Pass@1. All p-values are Holm-Bonferroni corrected.}
	\label{tab:rq3-stat}
	%\scriptsize
	\small
	% ===== Python =====
	\resizebox{1\textwidth}{!}{%
		\begin{tabular}{>{\centering\arraybackslash}m{2.5cm} | r | r r r | r r r r | r r r r}
			\toprule
			\multicolumn{13}{c}{\textbf{Python}} \\
			\midrule
			& \multicolumn{1}{c|}{\bf Pass@1} & \multicolumn{3}{c|}{\bf Lizard} & \multicolumn{4}{c|}{\bf Pylint} & \multicolumn{4}{c}{\bf SonarCloud} \\
			\cmidrule(lr){2-2} \cmidrule(lr){3-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
			
			\bf Comparison
			& \multicolumn{1}{c|}{}
			& \multicolumn{1}{c}{\bf LoC} & \multicolumn{1}{c}{\bf Tok} & \multicolumn{1}{c|}{\bf CyC}
			& \multicolumn{1}{c}{\bf Err} & \multicolumn{1}{c}{\bf Warn} & \multicolumn{1}{c}{\bf Conv} & \multicolumn{1}{c|}{\bf Ref}
			& \multicolumn{1}{c}{\bf Rel} & \multicolumn{1}{c}{\bf Main} & \multicolumn{1}{c}{\bf CyC} & \multicolumn{1}{c}{\bf CoC} \\
			
			& \bf OR 
			& \bf p-value & \bf p-value & \bf p-value 
			& \bf p-value & \bf p-value & \bf p-value & \bf p-value 
			& \bf p-value & \bf p-value & \bf p-value & \bf p-value \\
			\midrule
			
			3-task vs CG+CS & 1.118 & 0.02 & $<$0.01 & 0.22 & 0.56 & $<$0.01 & 1.00 & 1.00 & 0.72 & 1.00 & 0.68 & 0.56 \\
			3-task vs CG+CT & 1.000 & 1.00 & 1.00 & 1.00 & 0.07 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
			
			\bottomrule
		\end{tabular}
	}
	
	\vspace{0.3cm}
	
	% ===== Java =====
	\resizebox{1\textwidth}{!}{%
		\begin{tabular}{>{\centering\arraybackslash}m{2.5cm} | r | r r r | r r r r r r | r r r r}
			\toprule
			\multicolumn{15}{c}{\textbf{Java}} \\
			\midrule
			& \multicolumn{1}{c|}{\bf Pass@1} & \multicolumn{3}{c|}{\bf Lizard} & \multicolumn{6}{c|}{\bf PMD} & \multicolumn{4}{c}{\bf SonarCloud} \\
			\cmidrule(lr){2-2} \cmidrule(lr){3-5} \cmidrule(lr){6-11} \cmidrule(lr){12-15}
			
			\bf Comparison
			& \multicolumn{1}{c|}{}
			& \multicolumn{1}{c}{\bf LoC} & \multicolumn{1}{c}{\bf Tok} & \multicolumn{1}{c|}{\bf CyC}
			& \multicolumn{1}{c}{\bf BP} & \multicolumn{1}{c}{\bf CS} & \multicolumn{1}{c}{\bf Des} & \multicolumn{1}{c}{\bf EP} & \multicolumn{1}{c}{\bf MT} & \multicolumn{1}{c|}{\bf Perf}
			& \multicolumn{1}{c}{\bf Rel} & \multicolumn{1}{c}{\bf Main} & \multicolumn{1}{c}{\bf CyC} & \multicolumn{1}{c}{\bf CoC} \\
			
			& \bf OR 
			& \bf p-value & \bf p-value & \bf p-value 
			& \bf p-value & \bf p-value & \bf p-value & \bf p-value & \bf p-value & \bf p-value 
			& \bf p-value & \bf p-value & \bf p-value & \bf p-value \\
			\midrule
			
			3-task vs CG+CS & 0.704 & 1.00 & 1.00 & 1.00 & 1.00 & 0.05 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
			3-task vs CG+CT & 0.543 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 0.51 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
			
			\bottomrule
		\end{tabular}
	}
	\vspace{-10pt}
\end{table*}

==> tables/stat-tables/rq3-stat-cs.tex <==
% % ==================== COMBINED RQ3 CODE SUMMARIZATION TABLE ====================
% \begin{table*}[h]
% 	\centering
% 	\caption{Statistical comparison of 3-task MT-QLoRA vs 2-task MT-QLoRA (Qwen 3B) for code summarization. Significance assessed using Wilcoxon Signed-Rank Test. Effect size measured by Cliff's Delta (d) (N: negligible, S: small, M: medium, L: large). All p-values are Holm-Bonferroni corrected.}
% 	\label{tab:rq3-stat-summarization}
% 	%\scriptsize
%     \small
	
% 	% ===== Java =====
% 	\resizebox{\linewidth}{!}{
% 		\begin{tabular}{>{\centering\arraybackslash}m{2.5cm} | rr rr rr rr rr rr}
% 			\toprule
% 			\multicolumn{13}{c}{\textbf{Java}} \\
% 			\midrule
% 			\bf Comparison
% 			& \multicolumn{2}{c}{\bf BLEU} & \multicolumn{2}{c}{\bf METEOR} & \multicolumn{2}{c}{\bf Rouge-L} & \multicolumn{2}{c}{\bf chrF} & \multicolumn{2}{c}{\bf BERTScore} & \multicolumn{2}{c}{\bf SIDE} \\
			
% 			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d \\
% 			\midrule
			
% 			3-task vs CG+CS & 1.00 & -0.006 (N) & 1.00 & -0.007 (N) & 1.00 & -0.018 (N) & 1.00 & 0.013 (N) & 1.00 & -0.008 (N) & 1.00 & -0.019 (N) \\
% 			3-task vs CS+CT & 0.37 & -0.058 (N) & 1.00 & -0.018 (N) & 1.00 & 0.007 (N) & 1.00 & 0.000 (N) & 1.00 & -0.016 (N) & 1.00 & -0.039 (N) \\
			
% 			\bottomrule
% 		\end{tabular}
% 	}
	
% 	\vspace{0.3cm}
	
% 	% ===== Python =====
% 	\resizebox{\linewidth}{!}{
% 		\begin{tabular}{>{\centering\arraybackslash}m{2.5cm} | rr rr rr rr rr}
% 			\toprule
% 			\multicolumn{11}{c}{\textbf{Python}} \\
% 			\midrule
% 			\bf Comparison
% 			& \multicolumn{2}{c}{\bf BLEU} & \multicolumn{2}{c}{\bf METEOR} & \multicolumn{2}{c}{\bf Rouge-L} & \multicolumn{2}{c}{\bf chrF} & \multicolumn{2}{c}{\bf BERTScore} \\
			
% 			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d \\
% 			\midrule
			
% 			3-task vs CG+CS & 1.00 & 0.005 (N) & 1.00 & 0.002 (N) & 1.00 & -0.011 (N) & 1.00 & 0.008 (N) & 0.80 & -0.032 (N) \\
% 			3-task vs CS+CT & $<$0.01 & 0.208 (S) & $<$0.01 & 0.227 (S) & $<$0.01 & 0.229 (S) & $<$0.01 & 0.219 (S) & $<$0.01 & 0.214 (S) \\
			
% 			\bottomrule
% 		\end{tabular}
% 	}
% 	\vspace{-0.2cm}
% \end{table*}

% ==================== COMBINED RQ3 CODE SUMMARIZATION TABLE ====================
\begin{table*}[h]
	\centering
	\caption{Statistical comparison of 3-task MT-QLoRA vs 2-task MT-QLoRA (Qwen 3B) for code summarization. Significance assessed using Wilcoxon Signed-Rank Test. All p-values are Holm-Bonferroni corrected.}
	\label{tab:rq3-stat-summarization}
	%\scriptsize
    \small
	
	% ===== Java =====
	\resizebox{0.75\textwidth}{!}{%
		\begin{tabular}{>{\centering\arraybackslash}m{2.5cm} | r r r r r r}
			\toprule
			\multicolumn{7}{c}{\textbf{Java}} \\
			\midrule
			\bf Comparison
			& \multicolumn{1}{c}{\bf BLEU} & \multicolumn{1}{c}{\bf METEOR} & \multicolumn{1}{c}{\bf Rouge-L} & \multicolumn{1}{c}{\bf chrF} & \multicolumn{1}{c}{\bf BERTScore} & \multicolumn{1}{c}{\bf SIDE} \\
			
			& \bf p-value & \bf p-value & \bf p-value & \bf p-value & \bf p-value & \bf p-value \\
			\midrule
			
			3-task vs CG+CS & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
			3-task vs CS+CT & 0.37 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
			
			\bottomrule
		\end{tabular}
	}
	
	\vspace{0.3cm}
	
	% ===== Python =====
	\resizebox{0.75\textwidth}{!}{%
		\begin{tabular}{>{\centering\arraybackslash}m{2.5cm} | r r r r r}
			\toprule
			\multicolumn{6}{c}{\textbf{Python}} \\
			\midrule
			\bf Comparison
			& \multicolumn{1}{c}{\bf BLEU} & \multicolumn{1}{c}{\bf METEOR} & \multicolumn{1}{c}{\bf Rouge-L} & \multicolumn{1}{c}{\bf chrF} & \multicolumn{1}{c}{\bf BERTScore} \\
			
			& \bf p-value & \bf p-value & \bf p-value & \bf p-value & \bf p-value \\
			\midrule
			
			3-task vs CG+CS & 1.00 & 1.00 & 1.00 & 1.00 & 0.80 \\
			3-task vs CS+CT & $<$0.01 & $<$0.01 & $<$0.01 & $<$0.01 & $<$0.01 \\
			
			\bottomrule
		\end{tabular}
	}
	\vspace{-0.2cm}
\end{table*}

==> tables/stat-tables/rq3-stat-ct.tex <==
% % ==================== COMBINED RQ3 CODE TRANSLATION TABLE ====================
% \begin{table*}[h]
% 	\centering
% 	\caption{Statistical comparison of 3-task MT-QLoRA vs 2-task MT-QLoRA (Qwen 3B) for code translation. Significance assessed using Wilcoxon Signed-Rank Test. Effect size measured by Cliff's Delta (d) (N: negligible, S: small, M: medium, L: large). All p-values are Holm-Bonferroni corrected.}
% 	\label{tab:rq3-stat-translation}
% 	%\scriptsize
%     \small
	
% 	% ===== Java to C# =====
% 	\resizebox{\linewidth}{!}{
% 		\begin{tabular}{>{\centering\arraybackslash}m{2.5cm} | rr | rr rr rr | rr rr}
% 			\toprule
% 			\multicolumn{13}{c}{\textbf{Java to C\#}} \\
% 			\midrule
% 			& \multicolumn{2}{c|}{\bf CodeBLEU} & \multicolumn{6}{c|}{\bf Lizard} & \multicolumn{4}{c}{\bf Roslyn} \\
% 			\cmidrule(lr){2-3} \cmidrule(lr){4-9} \cmidrule(lr){10-13}
			
% 			\bf Comparison
% 			& \multicolumn{2}{c|}{}
% 			& \multicolumn{2}{c}{\bf LoC} & \multicolumn{2}{c}{\bf Tok} & \multicolumn{2}{c|}{\bf CyC}
% 			& \multicolumn{2}{c}{\bf Syntax} & \multicolumn{2}{c}{\bf Main} \\
			
% 			& \bf p-value & \bf d 
% 			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d 
% 			& \bf p-value & \bf d & \bf p-value & \bf d \\
% 			\midrule
			
% 			3-task vs CG+CT & $<$0.01 & -0.271 (S) & $<$0.01 & -0.058 (N) & $<$0.01 & -0.057 (N) & $<$0.01 & -0.059 (N) & $<$0.01 & -0.177 (S) & $<$0.01 & 0.566 (L) \\
% 			3-task vs CS+CT & $<$0.01 & 0.688 (L) & $<$0.01 & 0.816 (L) & $<$0.01 & 0.831 (L) & $<$0.01 & 0.758 (L) & $<$0.01 & 0.059 (N) & $<$0.01 & 0.424 (M) \\
			
% 			\bottomrule
% 		\end{tabular}
% 	}
	
% 	\vspace{0.3cm}
	
% 	% ===== C# to Java =====
% 	\resizebox{\linewidth}{!}{
% 		\begin{tabular}{>{\centering\arraybackslash}m{2.5cm} | rr | rr rr rr | rr rr rr rr rr rr | rr rr rr rr}
% 			\toprule
% 			\multicolumn{29}{c}{\textbf{C\# to Java}} \\
% 			\midrule
% 			& \multicolumn{2}{c|}{\bf CodeBLEU} & \multicolumn{6}{c|}{\bf Lizard} & \multicolumn{12}{c|}{\bf PMD} & \multicolumn{8}{c}{\bf SonarCloud} \\
% 			\cmidrule(lr){2-3} \cmidrule(lr){4-9} \cmidrule(lr){10-21} \cmidrule(lr){22-29}
			
% 			\bf Comparison
% 			& \multicolumn{2}{c|}{}
% 			& \multicolumn{2}{c}{\bf LoC} & \multicolumn{2}{c}{\bf Tok} & \multicolumn{2}{c|}{\bf CyC}
% 			& \multicolumn{2}{c}{\bf BP} & \multicolumn{2}{c}{\bf CS} & \multicolumn{2}{c}{\bf Des} & \multicolumn{2}{c}{\bf EP} & \multicolumn{2}{c}{\bf MT} & \multicolumn{2}{c|}{\bf Perf}
% 			& \multicolumn{2}{c}{\bf Rel} & \multicolumn{2}{c}{\bf Main} & \multicolumn{2}{c}{\bf CyC} & \multicolumn{2}{c}{\bf CoC} \\
			
% 			& \bf p-value & \bf d 
% 			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d 
% 			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d 
% 			& \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d & \bf p-value & \bf d \\
% 			\midrule
			
% 			3-task vs CG+CT & $<$0.01 & -0.118 (N) & 1.00 & -0.004 (N) & 1.00 & -0.006 (N) & 0.62 & 0.009 (N) & 1.00 & 0.004 (N) & 1.00 & -0.050 (N) & 1.00 & -0.009 (N) & 0.40 & -0.055 (N) & 1.00 & 0.000 (N) & 1.00 & -0.017 (N) & 0.40 & -0.008 (N) & $<$0.01 & -0.300 (S) & $<$0.01 & -0.319 (S) & $<$0.01 & -0.091 (N) \\
% 			3-task vs CS+CT & $<$0.01 & 0.760 (L) & $<$0.01 & 0.853 (L) & $<$0.01 & 0.846 (L) & $<$0.01 & 0.809 (L) & 0.35 & 0.023 (N) & 0.03 & -0.088 (N) & 0.74 & -0.007 (N) & 0.74 & -0.012 (N) & 1.00 & 0.000 (N) & 0.74 & -0.017 (N) & 0.10 & 0.006 (N) & $<$0.01 & -0.561 (L) & $<$0.01 & 0.202 (S) & $<$0.01 & 0.052 (N) \\
			
% 			\bottomrule
% 		\end{tabular}
% 	}
% 	\vspace{-0.2cm}
% \end{table*}

% ==================== COMBINED RQ3 CODE TRANSLATION TABLE ====================
\begin{table*}[h]
	\centering
	\caption{Statistical comparison of 3-task MT-QLoRA vs 2-task MT-QLoRA (Qwen 3B) for code translation. Significance assessed using Wilcoxon Signed-Rank Test. All p-values are Holm-Bonferroni corrected.}
	\label{tab:rq3-stat-translation}
    \resizebox{0.75\textwidth}{!}{%
	%\scriptsize
	
	% ===== Java to C# =====
		\begin{tabular}{>{\centering\arraybackslash}m{2.5cm} | r | r r r | r r}
			\toprule
			\multicolumn{7}{c}{\textbf{Java to C\#}} \\
			\midrule
			& \multicolumn{1}{c|}{\bf CodeBLEU} & \multicolumn{3}{c|}{\bf Lizard} & \multicolumn{2}{c}{\bf Roslyn} \\
			\cmidrule(lr){2-2} \cmidrule(lr){3-5} \cmidrule(lr){6-7}
			
			\bf Comparison
			& \multicolumn{1}{c|}{}
			& \multicolumn{1}{c}{\bf LoC} & \multicolumn{1}{c}{\bf Tok} & \multicolumn{1}{c|}{\bf CyC}
			& \multicolumn{1}{c}{\bf Syntax} & \multicolumn{1}{c}{\bf Main} \\
			
			& \bf p-value
			& \bf p-value & \bf p-value & \bf p-value
			& \bf p-value & \bf p-value \\
			\midrule
			
			3-task vs CG+CT & $<$0.01 & $<$0.01 & $<$0.01 & $<$0.01 & $<$0.01 & $<$0.01 \\
			3-task vs CS+CT & $<$0.01 & $<$0.01 & $<$0.01 & $<$0.01 & $<$0.01 & $<$0.01 \\
			
			\bottomrule
		\end{tabular}
    }
	
	\vspace{0.3cm}
	
	% ===== C# to Java =====
	\resizebox{1\textwidth}{!}{%
		\begin{tabular}{>{\centering\arraybackslash}m{2.5cm} | r | r r r | r r r r r r | r r r r}
			\toprule
			\multicolumn{15}{c}{\textbf{C\# to Java}} \\
			\midrule
			& \multicolumn{1}{c|}{\bf CodeBLEU} & \multicolumn{3}{c|}{\bf Lizard} & \multicolumn{6}{c|}{\bf PMD} & \multicolumn{4}{c}{\bf SonarCloud} \\
			\cmidrule(lr){2-2} \cmidrule(lr){3-5} \cmidrule(lr){6-11} \cmidrule(lr){12-15}
			
			\bf Comparison
			& \multicolumn{1}{c|}{}
			& \multicolumn{1}{c}{\bf LoC} & \multicolumn{1}{c}{\bf Tok} & \multicolumn{1}{c|}{\bf CyC}
			& \multicolumn{1}{c}{\bf BP} & \multicolumn{1}{c}{\bf CS} & \multicolumn{1}{c}{\bf Des} & \multicolumn{1}{c}{\bf EP} & \multicolumn{1}{c}{\bf MT} & \multicolumn{1}{c|}{\bf Perf}
			& \multicolumn{1}{c}{\bf Rel} & \multicolumn{1}{c}{\bf Main} & \multicolumn{1}{c}{\bf CyC} & \multicolumn{1}{c}{\bf CoC} \\
			
			& \bf p-value
			& \bf p-value & \bf p-value & \bf p-value
			& \bf p-value & \bf p-value & \bf p-value & \bf p-value & \bf p-value & \bf p-value
			& \bf p-value & \bf p-value & \bf p-value & \bf p-value \\
			\midrule
			
			3-task vs CG+CT & $<$0.01 & 1.00 & 1.00 & 0.62 & 1.00 & 1.00 & 1.00 & 0.40 & 1.00 & 1.00 & 0.40 & $<$0.01 & $<$0.01 & $<$0.01 \\
			3-task vs CS+CT & $<$0.01 & $<$0.01 & $<$0.01 & $<$0.01 & 0.35 & 0.03 & 0.74 & 0.74 & 1.00 & 0.74 & 0.10 & $<$0.01 & $<$0.01 & $<$0.01 \\
			
			\bottomrule
		\end{tabular}
	}
	\vspace{-0.2cm}
\end{table*}
